Compact and Optimal Deep Learning with Recurrent Parameter Generators

Deep learning has achieved tremendous success by training increasingly large models, which are then compressed for practical deployment. We propose a drastically different approach to compact and optimal deep learning: We decouple the Degrees of freedom (DoF) and the actual number of parameters of a model, optimize a small DoF with predefined random linear constraints for a large model of arbitrary architecture, in one-stage end-to-end learning. Specifically, we create a recurrent parameter generator (RPG), which repeatedly fetches parameters from a ring and unpacks them onto a large model with random permutation and sign flipping to promote parameter decorrelation. We show that gradient descent can automatically find the best model under constraints with faster convergence. Our extensive experimentation reveals a log-linear relationship between model DoF and accuracy. Our RPG demonstrates remarkable DoF reduction and can be further pruned and quantized for additional run-time performance gain. For example, in terms of top-1 accuracy on ImageNet, RPG achieves $96\%$ of ResNet18's performance with only $18\%$ DoF (the equivalent of one convolutional layer) and $52\%$ of ResNet34's performance with only $0.25\%$ DoF! Our work shows a significant potential of constrained neural optimization in compact and optimal deep learning.

==> 2107 (1)/Recurrent layers/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> 2107 (1)/Recurrent layers/sections/0abstract.tex <==
\begin{abstract}
Deep learning has achieved tremendous success 
by training increasingly large models, which are then compressed for practical deployment.  We propose a drastically different approach to compact and optimal deep learning:   
 We decouple the Degrees of freedom (DoF) and the actual number of parameters of a model, optimize a small DoF with predefined random linear constraints for a large model of an arbitrary architecture, in one-stage end-to-end learning.
 
Specifically, we create a recurrent parameter generator (RPG), which repeatedly fetches parameters from a ring  and unpacks them onto a large model with random permutation and sign flipping to promote parameter decorrelation.  We show that gradient descent can automatically find the best model under constraints with in fact faster convergence.

Our extensive experimentation reveals a log-linear relationship between model DoF and accuracy.  Our
 RPG demonstrates remarkable DoF reduction, 
and can be further pruned and quantized for additional  run-time performance gain.
For example, in terms of top-1 accuracy on ImageNet,
RPG achieves 96\% of ResNet18's performance with only 18\% DoF (the equivalent of one convolutional layer) and 52\% of ResNet34's performance with only 0.25\% DoF!
Our work shows significant potential of constrained neural optimization in compact and optimal deep learning.
\end{abstract}

==> 2107 (1)/Recurrent layers/sections/1intro.tex <==
%\textcolor{red}{To add: RPG is similar to weight clustering. Model file can be diminished - thus, there is smaller storage space and faster transfer rate.}

\def\figModelRing#1{
\begin{figure}[#1]\centering
\vspace{-1.5em}
\includegraphics[width=0.92\columnwidth]{figures/modelRing.pdf}
\caption{ \small We propose a recurrent parameter generator (RPG) that shares a fixed set of parameters in a ring and use them to generate parameters of different parts of a neural network, %simply by permutations and sign flipping, 
whereas in the standard neural network, all the parameters are independent of each other, so the model gets bigger as it gets deeper. \textbf{Left}: The \textcolor{orange}{third} section of the model starts to overlap with the \textcolor{red}{first} section in the model ring, and all later layers 
 share generating parameters for possibly multiple times.
 \textbf{Right:} Employing the Recurrent Parameter Generator (RPG) for ResNet could reduce the model parameters to any size. Specifically, with only half ResNet34 backbone parameters, we achieve the same ImageNet top-1 accuracy. 
 We also outperform model compression methods such as Knapsack \cite{aflalo2020knapsack}.% and PruneNet \cite{khetan2020prunenet}.
}
\vspace{-1.5em}
\label{fig:modelRing}
\end{figure}
}

\def\figtasks#1{
\vspace{-1.5em}
\begin{figure*}[#1]\centering
\includegraphics[width=0.9\textwidth]{figures/tasks_v2.pdf}
\vspace{-1em}
\caption{ \small  We demonstrate the effectiveness of RPG on various applications including image classification (\textbf{Left}), human pose estimation (\textbf{Middle}), and multitask regression (\textbf{Right}). RPGs are shared at multiple scales: a network can either have a global RPG or multiple local RPGs that are shared within blocks or sub-networks.
}
\vspace{-1.5em}
\label{fig:tasks}
\end{figure*}
}

\section{Introduction}

\begin{figure}[t]
    \centering
 \includegraphics[width=\columnwidth]{figures/teaser.pdf}
   \caption{ \small 
   We propose a novel approach to compact and optimal deep learning by decoupling model DoF and model parameters.
   {\bf a}) Existing methods first finds the optimal in a large model space and then compress it for practical deployment.  
   {\bf b})  We propose to start with a small (DoF) model of free parameters, use 
   recurrent parameter generator (RPG) to unpack them onto a large model with predefined random linear projections. 
   {\bf c}) Gradient descent finds the optimal model of a small DoF under these linear constraints with faster converge than training the large unpacked model itself (Fig.\ref{fig:combo2}{\bf b}). 
   If the DoF is too small, the optimal large model may fall out of the constrained subpsace.  However, at a sufficiently large DoF,  RPG gets rid of redundancy and often finds a model with little loss in accuracy. 
   %Large models are known to have high redundancy and low degree of freedom (DoF), for which they could be pruned to small models, e.g. high filter similarity of different layers in VGG16 is observed ({\bf c}).
    {\bf d}) RPG reveals a log-linear relationship between model DoF and accuracy.
   {\bf e}) RPG achieves the same ImageNet accuracy with half of the ResNet-vanilla DoF. RPG also outperforms other state-of-the-art compression approaches.
   }  %\captionof{figure}{A figure}
  \label{fig:teaser}
  \vspace{-1.5em}
\end{figure}

%TODO: (on reduce redundancy) Cite OCNN, lean block;
% Mention we do not compress FLOPs

% points: 1) decouple; 2) DoF; 3) practical use (reduce flops)

Deep neural networks as general optimization tools have achieved great success with increasingly more training data, deeper and larger neural networks:  A recently developed NLP model, GPT-3 \cite{brown2020language}, has astonishing 175 billion parameters!  
While the model performance generally scales with the number of parameters \cite{henighan2020scaling}, with parameters outnumbering training data, the model is significantly over-parameterized. 

%(Fig.\ref{fig:combo1}{\bf a}), 
Many approaches have been proposed to remove redundancy in trained large models: neural network pruning \cite{lecun1990optimal, han2015deep, liu2018rethinking}, efficient network design spaces \cite{howard2017mobilenets, iandola2016squeezenet, sandler2018mobilenetv2}, parameter regularization \cite{wan2013regularization, wang2020orthogonal, srivastava2014dropout, NowlanH92simplifying}, model quantization \cite{hubara2017quantized, rastegari2016xnor, louizos2018relaxed}, neural architecture search \cite{zoph2016neural, cai2018proxylessnas, wan2020fbnetv2}, recurrent models \cite{bai2019deep, bai2020multiscale, wei2016convolutional}, multi-task feature encoding \cite{ramamonjisoa2019sharpnet, hao2020multi}, etc. 
Pruning-based model compression dates back to the late 80s \cite{mozer1989using, lecun1990optimal} and has enjoyed recent resurgence \cite{han2015deep, blalock2020state}. They remove unimportant parameters from a pre-trained model and can achieve significant model compression.


 %\figModelRing{tp}
 \begin{figure}[t]
    \centering
 \includegraphics[width=\columnwidth]{figures/genweight.pdf}
   \vspace{-1em}
   \caption{ \small
   {\bf Upper:} Networks are optimized with a linear constraint $\hat{\mathbf{W}} = \boldsymbol{G} \mathbf{W}$, where the constrained parameter $\hat{\mathbf{W}}$ of each network layer was generated by the generating matrix $\boldsymbol{G}$ from the free parameter $\mathbf{W}$, which is directly optimized. $\hat{\mathbf{W}}$ is unpacked large model parameter while the size of $\mathbf{W}$ is the model DoF.
   {\bf Lower:} This paper discusses a specific format of parameter generation, 
  recurrent parameter generator (RPG).
   RPG shares a fixed set of parameters in a ring and uses them to generate parameters of different parts of a neural network,
whereas in the standard neural network, all the parameters are independent of each other, so the model gets bigger as it gets deeper. The \textcolor{orange}{third} section of the model starts to overlap with the \textcolor{red}{first} section in the model ring, and all later layers 
 share generating parameters for possibly multiple times.
   }  %\captionof{figure}{A figure}
  \label{fig:modelring_}
  \vspace{-1.5em}
\end{figure}

%Though sharing a similar motivation to reduce the parameter redundancy, 
Our work is a departure from mainstream approaches towards model optimization and parameter reduction: rather than compressing a large model, we directly optimize a lean model with a small set of free parameters (number of free parameters equal to degree of freedom of the model, or DoF), which can be linearly unpacked to a large model. Training the large model can be viewed as solving a neural optimization with a set of predefined linear constraints. One benefit of constrained neural optimization we observe is that it leads to a faster convergence rate (Section \ref{sec:general}).
% The optimization parameters of the large model are linearly constrained by the small DoF.
%We explore an entirely different territory of model DoF reduction: rather than compressing a large model, we define an arbitrarily large model based on a fixed set of parameters to maximize the model capacity. 
Specifically, we define different layers in a neural network based on a fixed amount of DoF, which we call \textit{recurrent parameter generator} (RPG).
That is, we differentiate the number of model parameters and DoF.
Traditionally, model parameters are treated independently of each other; the total number of parameters equals DoF. However, by tapping into how a core set of free parameters can be assigned to the neural network model, we can develop a large model of many parameters, which are linearly constrained by the small set of free parameters.
%We show that the excess parameter capacity can be exploited with almost no assumptions of how the parameters are assigned to the neural network architecture.

There is excess capacity in neural networks independent of how and where the parameters are used in the network, even at the level of individual scalar values.
% , parameters can be reused in another arbitrary location of the deep network architecture without significantly impacting model performance.
Surprisingly, backpropagation training of a deep network is able to cope with that the same parameter can be assigned to multiple random locations in the network without significantly impacting model performance. Our extensive experiments show that a large neural network does not need to be over-parameterized to achieve competitive performance. Particularly, a ResNet18 can be implemented with DoF equivalent to one convolution layer in a ResNet18-vanilla ($4.72\times$ DoF reduction) and still achieves $67.2\%$ ImageNet top-1 accuracy. The proposed method is also extremely flexible in reducing model DoF. In some sense, the proposed RPG method can be viewed as an automatic model DoF reduction technique, which explores the optimal accuracy-parameter trade-off. When we reduce the model DoF, RPG demonstrates graceful performance degradation, and its compression results are frequently on par with the SOTA pruning methods besides the flexibility. Even if we reduce the Res18 backbone DoF to $36$K, which is about $300\times$ reduction, ResNet18 can still achieve $40\%$ ImageNet top-1 accuracy. Further, we show RPG can be quantized and pruned to improve FLOPs and runtime with relatively
mild accuracy drops. 

To summarize, we make three contributions:
%\vspace{-0.5em}
\begin{enumerate*}
%\setlength{\itemsep}{-0em}
    \item We provide a new perspective towards automatic model size reduction: we define a neural network with certain DoF with random linear constraints. We discover that gradient descent can automatically solve constrained optimization for the best model with a faster convergence rate. This constrained neural optimization perspective is likely to benefit many other applications. % under the desired constraint.
    
    \item We propose the recurrent parameter generator (RPG), which decouples the network architecture and the network DoF. We can flexibly choose any desired DoF to construct the network given a specific neural network architecture. 

    \item By separating network architectures from parameters, RPG becomes a tool to understand the relationship between the model DoF and the network performance.  We observe an empirical log-linear DoF-Accuracy relationship.
    %\textcolor{red}{By factoring out network architecture, RPG could be considered as a tool to understand relationships between parameter size and network performance. We show a log-linear relationship between them.} %Given a compression ratio, RPG achieves on-par performance compared to the state-of-the-art model pruning methods. This may provide an entirely new perspective for model compression.
    
    %\item With destructive weight sharing, RPG achieves competitive performance compared to several recurrent weight-sharing models. This makes RPG a strong baseline for probing the representation sharing for recurrent models.
\end{enumerate*}
\figtasks{t}

% This makes RPG a strong and practical baseline for probing whether there is nontrivial representation sharing within any recurrent network.

%\textcolor{red}{This needs to be moved to later part of the paper.} Notably, we choose a destructive parameter sharing method \cite{CheungPSP19} for RPG in this work, which discourages potential representation sharing from layer to layer. Compared to other weight-sharing methods, e.g., convolutional pose machine (CPM) and multi-scale deep equilibrium models (MDEQ), our method achieves competitive  performance on various benchmarks. 


% A more relevant result was shown in model superposition \cite{cheung2019superposition} that many different models based on the same neural network can be stored into one set of parameters with minimal performance interference to each other. Inspired by the result, we generalize the concept and propose to define many different layer in a deep neural network based on a fixed amount of parameters. we show that the excess capacity can be exploited with almost no assumptions of how the parameters are assigned into architecture of the neural network. In other words, there is excess capacity in neural network models independent of how and where the parameters are used in the network. Even at the level of individual scalar values, parameters can be reused in another arbitrary location of the deep network architecture without significantly impacting model performance. Surprisingly, back propagation training of a deep network is able to cope with that the same parameter can be assigned to multiple random locations in the network without significantly impacting model performance. Through thorough experiments, we show that a large neural network does not need to be over overparameterized to achieve competitive performance. Particularly, a Resnet18 model can be implemented with the number of weights equivalent to one convolution layer in a conventional Resnet ($4.72\times$ parameter reduction) and still achieve $67.2\%$ ImageNet top-1 accuracy. The propose method is also extremely flexible in reducing the model parameters. Even if we reduce the backbone parameters to $36K$, which is about $300\times$ reduction, Resnet18 can still achieve $40.0\%$ ImageNet top-1 accuracy.

% Notably, a destructive parameter sharing method is used in this work, which discourages any potential representation sharing from layer to layer. Compared to other recurrent weight-sharing methods, e.g. convolutional pose machine (CPM) or multi-scale deep equilibrium models (MDEQ), our method achieves competitive or even better performance on a variety benchmarks. This makes our work a strong baseline for probing whether there is nontrivial representation sharing within any recurrent network.




% The number of parameters in deep networks often outnumber the datapoints they are trained on indicating that these models are significantly overparameterized. 
% This has led to many types of network compression algorithms and pruning methods to reduce the redundancies after training. But what is the source of this excess capacity?


%\textcolor{red}{ Call it ``parameter generator ring'', dub as parameter ring.}
% Contributions:
% \begin{itemize}
% \item Generic method to construct an arbitrarily convolutional neural network with a fixed set of parameters. Show competitive performance.
% \item Strong baseline for probing if there is any representation sharing in recurrent models.
% \end{itemize}


  


==> 2107 (1)/Recurrent layers/sections/2relatedworks.tex <==
\vspace{-0.5em}
\section{Related Work}
\vspace{-0.5em}
%There are many important efforts to compress  neural networks or to reduce the redundancy in neural network parameters.
Many works study model DoF reduction or compression.
We discuss each one and its relationship to our work.

\noindent \textbf{Model Pruning, Neural Architecture Search, and Quantization.}
%As we discussed earlier, 
Model pruning seeks to remove unimportant parameters in a trained model. Recently, it's proposed to use neural architecture search as coarse-grained model pruning \cite{yu2018slimmable, dong2019network}. Another related effort is  network quantization \cite{hubara2017quantized, rastegari2016xnor, louizos2018relaxed}, which seeks to reduce the bits used for each parameter and can frequently reduce the model size by $4\times$ with minimal accuracy drop. More recently, \cite{dollar2021fast} presents a framework for analyzing model scaling strategies that consider network properties such as FLOPs and activations.

\noindent \textbf{Parameter Regularization and Priors}. 
%Another highly related direction is parameter regularization.  %Another highly related direction to this work is parameter regularization. 
Regularization has been widely used to reduce model redundancy \cite{krogh1992simple, NowlanH92simplifying}, alleviate overfitting \cite{srivastava2014dropout, wan2013regularization}, and ensure desired mathematical regularity \cite{wang2020orthogonal}. RPG can be viewed as a parameter regularization in the sense that weight sharing poses many equality constraints to  weights and regularizes  weights to a low-dimensional space. HyperNeat \cite{stanley2009hypercube} and CPPNs \cite{stanley2007compositional} use networks to determine the weight between two neurons as a function of their positions. \cite{karaletsos2018probabilistic, KaraletsosB20} introduced a similar idea by providing a hierarchical prior for network parameters.

% Given a network design, another way to improve performance and model capacity is via a regularizer on model parameters. Regularizers include weight decay \cite{krogh1992simple}, dropout\cite{srivastava2014dropout}, and orthogonal regularizer \cite{wang2020orthogonal}.
% %Weight decay. OCNN \cite{wang2020orthogonal}, dropout\cite{srivastava2014dropout}, DropConnect\cite{wan2013regularization}
% %Researchers \cite{wang2020orthogonal} demonstrate adding additional regularizer improves model capacity.

% \textbf{Recurrent Models.}
%add Convolutional Sparse Coding.

%ResNext use group convolution as efficient processing. A related work?


\noindent \textbf{Recurrent Networks and Deep Equilibrium Models.} Recurrence and feedback have been shown in psychology and neuroscience to act as modulators or competitive inhibitors to aid feature grouping \cite{gilbert2007brain}, figure-ground segregation \cite{hupe1998cortical} and object recognition \cite{wyatte2012limits}. Recurrence-inspired mechanisms also achieve success in feed-forward models. There are two main types of employing recurrence based on if weights are shared across recurrent modules. ResNet \cite{he2016deep}, a representative of reusing similar structures without weight sharing, introduces parallel residual connections and achieves better performance by going deeper in networks. Similarly, some works \cite{szegedy2015going,srivastava2015highway} also suggest iteratively injecting thus-far representations to the feed-forward network useful. Stacked inference methods \cite{ramakrishna2014pose,wolpert1992stacked,weiss2010structured} are also related while they consider each output in isolation. Some find sharing weights across recurrent modules valuable. They demonstrate applications in temporal modelling \cite{weiss2010structured,shi2015convolutional,karpathy2015deep}, spatial attention \cite{mnih2014recurrent,butko2009optimal}, pose estimation \cite{wei2016convolutional,carreira2016human}, and so on \cite{li2016iterative,zamir2017feedback}. Such methods usually shine in modeling long-term dependencies. In this work, we recurrently share weights across different layers of a feedback network to reduce network redundancy. 

% \textbf{Deep Equilibrium Models.}
%DEQ, MDEQ. Application in detection.
%Improve efficiency: Fixed Point Networks:
%Implicit Depth Models with Jacobian-Free Backprop
Given stacking weight-shared modules improve the performance, researchers consider running even infinite depth of such modules by making the sequential modules converge to a fixed point \cite{lecun1988theoretical,bai2019deep}. Employing such \textit{equilibrium} models to existing networks, they show improved performance in many natural language processing \cite{bai2019deep} and computer vision tasks \cite{bai2020multiscale,wang2020implicit}. One issue with deep equilibrium models is that the forward and backward propagation usually takes much more iterations than explicit feed-forward networks. Some work \cite{fung2021fixed} improves the efficiency by making the backward propagation Jacobian free. Another issue is that \textit{infinite} depth and fixed point may not be necessary or even too strict for some tasks. 
Instead of achieving infinite depth, our model shares parameters to a certain level. We empirically compare with equilibrium models in Section \ref{sec:exp}.


\noindent \textbf{Efficient Network Space and Matrix Factorization.}
Convolution is an efficient and structured matrix-vector multiplication. Arguably, the most fundamental idea in building efficient linear systems is matrix factorization. Given the redundancy in deep convolutional neural network parameters, one can leverage the matrix factorization concept, e.g., factorized convolutions, and design more efficient network classes \cite{howard2017mobilenets, iandola2016squeezenet, tan2019efficientnet, sandler2018mobilenetv2}.


% \textbf{Deep Network Redundancy.}
% %+ Review once-for-all (arxiv 1908.09791)
% Deep neural networks are over-parameterized and have significant redundancy \cite{jaderberg2014speeding}. Towards reduce network redundancy and efficient deep learning, different works propose solutions including model compression \cite{han2015deep,han2015learning},  efficient network structures \cite{iandola2016squeezenet,sandler2018mobilenetv2}, training techniques \cite{wang2020orthogonal}, and hardware-aware neural architecture search \cite{wu2019fbnet,tan2019mnasnet}. These works demonstrate reduced network redundancy and improved efficiency for a specific tasks. Recent works \cite{cai2019once,cheung2019superposition} further show that parameters of a base model can be shared and used for multiple tasks, which further improves the model efficiency. We explore sharing parameters across different layers of a model.

==> 2107 (1)/Recurrent layers/sections/3methods.tex <==
%\vspace{-0.5em}
\section{Recurrent Parameter Generator}
%\vspace{-0.5em}

\label{sec:method:ls}

%\textcolor{red}{To add: linear constraint theory}
%\textcolor{red}{matrix from the general orthogonal group also leads to similar results but this implementation has better efficiency.}

\noindent {\bf Linearly Constrained Neural Optimization.} 
% Parameter generator can be considered  as optimizing neural networks with linear constraints.
Consider optimizing a network with input data $\mathbf{X}$, parameters $\hat{\mathbf{W}}$ and loss function $L$. The optimization can be written as: 
\begin{align}
    \min L(\mathbf{X}; \hat{\mathbf{W}} )\ \ \text{s.t.}\  \mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W} (\text{or equally} \ \boldsymbol{R}\mathbf{\hat{\mathbf{W}}} = 0)
\end{align}
where $\mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W}$ refers to a set of linear constraints, where $\boldsymbol{G}\in \Re^{N\times M}$ is a full-rank tall matrix (i.e. $N\ge M$). Here we refer to $\hat{\mathbf{W}}$ as the constrained parameters and $\mathbf{W}$ as the free parameters. This constraint is a change of variable, i.e., the constrained parameter $\hat{\mathbf{W}}$ is linearly generated from the free parameter $\mathbf{W}$ by generating matrix $\boldsymbol{G}$. We can consider $\mathbf{W}$ as a compressed model, which is unpacked into $\hat{\mathbf{W}}$ to construct the large neural network. $\mathbf{W}$ is directly optimized via gradient descent and free to update. In this linearly constrained neural optimization, the model DoF is equivalent to $M$, which is the dimension of $\mathbf{W}$. An equivalent form of the constraint $\mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W}$ is $\boldsymbol{R}\mathbf{\hat{\mathbf{W}}} = 0$, where $\boldsymbol{R}\in\Re^{(N-M)\times N}$ can be derived from SVD of $\boldsymbol{G}$. 

% We also discuss the even sampling and batch normalization technique that are beneficial for training with RPG.


\noindent {\bf Recurrent Parameter Generator.} Let's assume that we construct a deep convolutional neural network containing $L$ different convolution layers. Let $\mathbf{K}_1,\mathbf{K}_2,\dots, \mathbf{K}_L$ be the corresponding $L$ convolutional kernels\footnote{A kernel contains all the filters of one layer. In this paper, we treat each convolutional kernel as a vector. When the kernel is used to do the convolution, it will be reshaped into the corresponding shape.}. 
Rather than using separate sets of parameters for different convolution layers, we create a single set of parameters $\mathbf{W}\in\Re^M$ and use it to generate the corresponding parameters $\hat{\mathbf{W}} = \left[\mathbf{K}_1^T,\mathbf{K}_2^T,\dots, \mathbf{K}_L^T\right]^T \in \Re^N$ for each convolution layer:
%Rather than using a different set of parameters for each different layer, we reuse a single set of parameters $W\in\Re^N$ in the following fashion:
\begin{equation}
\mathbf{K}_i = \boldsymbol{G}_i\cdot \mathbf{W}, i \in \{1,\dots,L\}
\label{eq:k}
\end{equation}
where $\boldsymbol{G}_i$ is a fixed predefined generating matrix, which is used to generate $\mathbf{K}_i$ from $\mathbf{W}$.
We call $\boldsymbol{G} = \left[\boldsymbol{G}_1^T,\dots,\boldsymbol{G}_L^T\right]^T$ and $\mathbf{W}$ the \textit{recurrent parameter generator} (RPG). In this work, we always assume that the size of $\mathbf{W}$ is not larger than the total parameters of the model, i.e., $|\mathbf{W}|\leq\sum_{i}{|\mathbf{K}_i|}$. This means an element of $\mathbf{W}$ will generally be used in more than one layer of a neural network. Additionally, the gradient of $\mathbf{W}$ is a linear superposition of the gradients from each convolution layer.
During the neural network training, let's assume convolution kernel $\mathbf{K}_i$ receives gradient $\frac{\partial \ell}{\partial \mathbf{K}_i}$, where $\ell$ is the loss function. Based on the chain rule, it is clear that the gradient of $\mathbf{W}$ is:
\begin{equation}
\frac{\partial \ell}{\partial \mathbf{W}} = \sum_{i=1}^{L}{\boldsymbol{G}^T_i\cdot \frac{\partial \ell}{\partial \mathbf{K}_i}}
\label{eq:grad_w}
\end{equation}
% {\bf Recurrent Parameter Generator.} We focus on a special case where $W$ is reused when generating convolutional kernels. In this case, the size of $W$ is smaller than the total parameters of the model, and elements of $W$ are recurrently used. $\{R_i\}$ and $W$ together is considered as a \textit{recurrent parameter generator}. Additionally, the gradient of $W$ is a linear superposition of the gradients from each convolution layer.
%{\bf Model Rings.} As we can see, the gradient of $W$ is a linear superposition of the gradients from each convolution layer. We call $W$ as the \emph{model ring} since it can be effectively seen as a superposition of many different convolutional kernels.
\noindent {\bf Generating Matrices and Destructive Weight Sharing.} There are various ways to create the generating matrices $\{\boldsymbol{G}_i\}$. While in general $\boldsymbol{G}$ can be any full-rank tall matrix, this paper focuses on the destructive generating matrices, which are random orthogonal matrices and could prevent different kernels from sharing the representation during weight sharing. Random generating matrices empirically improve the model capacity when the model DoF is fixed. We provide an intuitive theoretical explanation of how random orthogonal matrices prevent representation sharing as follows.

% Let's assume $\{\boldsymbol{G}_i\}$ are random orthogonal matrices and $\boldsymbol{G}_i = \left[A_1,\dots,A_\right]$

For easier discussion, let us consider a special case, where all of the convolutional kernels have the same size and are used in the same shape in the corresponding convolution layers. The dimension of $\mathbf{W}$ is equal to that of one convolutional layer kernel. In other words, $\{\boldsymbol{G}_i\}$ are square matrices, and the spatial sizes of all of the convolutional kernels have the same size, $d_{in}\times d_{out}\times w\times h$, and the input channel dimension $d_{in}$ is always equal to the output channel dimension $d_{out}$. In this case, a filter $\mathbf{f}$ in a kernel can be treated as a vector in $\Re^{dwh}$. Further, we choose $\boldsymbol{G}_i$ to be a block-diagonal matrix $\boldsymbol{G}_i=\text{diag}\{\boldsymbol{A}_i,\boldsymbol{A}_i,\dots,\boldsymbol{A}_i\}$, where $\boldsymbol{A}_i\in O(dwh)$ is an orthogonal matrix that generates each filter of the kernel $\mathbf{K}_i$ from $\mathbf{W}$, and $O(\cdot)$ denotes the orthogonal group. Similar to the Proposition~2 in \cite{CheungPSP19}, we show in the Appendix \ref{sec:supp2} that: if $\boldsymbol{A}_i$, $\boldsymbol{A}_j$ are sampled from the $O(dwh)$ Haar distribution and $\mathbf{f}_i$, $\mathbf{f}_j$ are the corresponding filters (generated by $\boldsymbol{G}_i$, $\boldsymbol{G}_j$ respectively from the same set of entries of $\mathbf{W}$) from $\mathbf{K}_i$, $\mathbf{K}_j$ respectively, then we have $\E\left[\langle \mathbf{f}_i,\mathbf{f}_j \rangle\right] = 0$ and $\E \left[\langle \frac{\mathbf{f}_i}{\|\mathbf{f}_i\|},\frac{\mathbf{f}_j}{\|\mathbf{f}_j\|}\rangle^2 \right]=\frac{1}{dwh}$. Since $dwh$ is usually large, the corresponding filters from $\mathbf{K}_i$, $\mathbf{K}_j$ are close to orthogonal and generally dissimilar. This shows that even when $\{\mathbf{K}_i\}$ are generated from the same entries of $\mathbf{W}$, they are prevented from sharing the representation.

Though $\{\boldsymbol{G}_i\}$ are not updated during training, the size of $\boldsymbol{G}_i$ can be quite large in general, which can create additional computation and storage overhead. In practice, we can use permutation and element-wise random sign reflection to construct a subset of the orthogonal group as permutations and sign reflections could be implemented with high simplicity and negligible cost. A simple demonstration of $\{\boldsymbol{G}_i\}$ is demonstrated in Fig.\ref{fig:modelring_}{\bf U}\footnote{Permutations and element-wise random sign reflection conceptually are subgroups from the orthogonal group, but we shall never use them in the matrix form for the obvious efficiency purpose.}. Since pseudo-random numbers are used, it takes only two random seeds to store a random permutation and an element-wise random sign reflection.


% In practice, we can use permutation $p\in P(M)$ and element-wise random sign reflection $b\in B(M)$ to construct a subset of the orthogonal group $O(M)$, i.e. we choose $\boldsymbol{A}_i \in \{b\circ p|\ b\in B(M), p\in P(M)\}$.\footnote{Permutations and element-wise random sign reflection conceptually are subgroups from the orthogonal group, but we shall never use them in the matrix form for the obvious efficiency purpose.} Since pseudo-random numbers are used, it takes only two random seeds to store a random permutation and an element-wise random sign reflection. 

% This paper requires that $R$ can only have three values $1, 0, -1$. In general, $R$ is a random matrix, but we show that this implementation has better efficiency.



% In this work, we generalize the usage of $\boldsymbol{G}_i$ beyond the block-diagonal generating matrices described above. $\{\mathbf{K}_i\}$ may have different sizes, which can be chosen even larger than the size of $\mathbf{W}$. When $\mathbf{K}_i\in \Re^{N_i}$ is larger than $\mathbf{W}\in\Re^{N}$, the corresponding generating matrix $\boldsymbol{G}_i$ is a tall matrix. There are many ways to efficiently create the generating matrices. We use random permutations $P(N_i)$ and element-wise random sign reflections $B(N_i)$ to create $\boldsymbol{G}_i$:
% \begin{equation}
% \label{eq:generating_matrix}
% \boldsymbol{G}_i\in \{b\circ p|\ b\in B(N_i), p\in P(N_i)\},\ i = 1,\dots,L
% \end{equation}
% $\{\boldsymbol{G}_i\}$ tend to lead to destructive weight sharing and lead to better utilization of the parameter capacity. Permutations and sign reflections could be implemented with high simplicity and negligible cost.

% The opposite of destructive generating matrices would be the identity matrix.




% Add destructive proposition.

%\textbf{Super-Parameter.}

% \textbf{Permutation and Random Rotation.}

\noindent \textbf{Even Parameter Sampling and Model Ring.}
% For better parameter capacity, we introduce an even sampling strategy. We illustrate the general parameter generator in Fig.\ref{fig:modelring_}{\bf L} and RPG in Fig.\ref{fig:modelring_}{\bf R}.
While it is easy to randomly sample elements from $\mathbf{W}$ when generating parameters for each layer, it may not be optimal as some elements in $\mathbf{W}$ may not be evenly used, and some elements in $\mathbf{W}$ used at all due to sampling fluctuation. 
A simple equalization technique can be used to guarantee all elements of $\mathbf{W}$ are evenly sampled.
Suppose the size of $\mathbf{W}$ is $M$, and the size of parameter $\mathbf{\hat{\mathbf{W}}}$  of the model to be generated is $N$, $N>M$. As we mentioned earlier, there are $L$ layers and they require $\{\|K_1\|,\dots,\|K_L\|\}$ parameters respectively. As $N>M$, we can use $W$ as a ring: we first draw the first $\|K_1\|$ parameters from $\mathbf{\hat{\mathbf{W}}}$ followed by a pre-generated random permutation $p_1$ and a  pre-generated random element-wise sign flipping $b_1$ to construct layer-1 kernel $\mathbf{K}_1$. Then we draw the next $\|K_2\|$ parameters from $\mathbf{\hat{\mathbf{W}}}$ followed by pre-generated random permutation $p_2$ and a pre-generated random element-wise sign flipping $b_2$. We continue this process and wrap around when there is not enough entries left from $\mathbf{\hat{\mathbf{W}}}$. We refer to $\mathbf{\hat{\mathbf{W}}}$ together with this sampling strategy as \textit{model rings} since the free parameters are recurrently used in a loop. We illustrate the general parameter generator in Fig.\ref{fig:modelring_}{\bf U} and RPG in Fig.\ref{fig:modelring_}{\bf L}. This For data saving efficiency, we just need to save several random seed numbers instead of saving the pre-generated permutations $\{p_1,\dots,p_L\}$ and sign flipping operations $\{b_1,\dots,b_L\}$.


% We first generate $\floor{\frac{N}{M} }$ arrays $\{x|x=1,..,M\}$ and concatenate them with $(N \mod M)$ elements randomly sampled from array $\{x|x=1,..,M\}$. We call the concatenated array index array $u \in \Re^N$.
% When initializing each layer's parameter, we sequentially get indices of chosen elements $u_i$ from $u$, and randomly shuffle $u_i$.
%In this way, each layer's parameters are randomly and evenly sampled from $\mathbf{W}$.
% We refer to $\mathbf{W}$ as \textit{model rings} since elements are recurrently used in a loop.
% For data saving efficiency, we just need to save two random seed numbers (one for sampling $(M \mod N)$ elements and one for shuffling) instead of saving the large index array $u$.

\noindent \textbf{Batch Normalization.} Model performance is relatively sensitive to the batch normalization parameters. For better performance, each convolution layer needs to have its own batch normalization parameters. In general, however, the size of batch normalization is relatively negligible. Yet when $\mathbf{W}$ is extremely small (e.g., $36$K parameters), the size of batch normalization should be considered.

\iffalse
\begin{figure}[t]
    \centering
 \includegraphics[width=1\columnwidth]{figures/MSparam.pdf}
   \vspace{-1em}
   \caption{ \small Recurrent parameter generators at multiple scales. \textbf{Upper:} A global RPG is used for generating convolution kernels for the entire ResNet18. \textbf{Lower }: Four local RPGs are each responsible for generating convolution kernels within each corresponding building block of the ResNet18.}  %\captionof{figure}{A figure}
  \label{fig:msparam}
  \vspace{-1.5em}
\end{figure}
\fi

 % \vspace{-1em}
\section{RPG at Multiple Scales}
 % \vspace{-1em}

We discuss the general idea of parameter generators where only one RPG is shared globally across all layers previously. 
We could also create several local RPGs, each of which is shared at certain scales, such as blocks and sub-networks. Such RPGs may be useful for certain applications such as recurrent modeling. %Experimental results are reported in Section \ref{sec:cifar_exp}.

\label{sec:extension}
\noindent \textbf{RPGs at Block-Level.}
Many existing network architectures reuse the same design of network blocks multiple times for higher learning capacity, as discussed in the related work. 
Instead of using one global RPG for the entire network, we could alternatively create several RPGs that are shared within certain network blocks.
We take Res18 \cite{he2016deep} as a concrete example.% (Fig.\ref{fig:msparam}). 
Res18 has four building blocks. Every block has 2 residual convolution modules. %Each block has multiple residual convolution modules and outputs feature maps at different spatial sizes. 
%Specifically, ResNet18 has $2,2,2,2$ residual modules for each building block, while ResNet34 has  $3,4,6,3$ residual modules for each building block.
%To superpose ResNet18 at block scale, 
We create four local RPGs for Res18.
Each RPG is shared within the corresponding building block, where the size of the RPG is flexible and can be determined by users. Fig.\ref{fig:tasks}{\bf M}) illustrates how RPGs can be shared at the block-level.

\noindent \textbf{RPGs at Sub-Network-Level.} 
Reusing sub-networks, or recurrent networks, has achieved success in many tasks as they iteratively refine and improve the prediction.
Parameters are often shared when reusing the sub-networks.
This may not be optimal as sub-networks at different stages iteratively improve the prediction, and shared parameters may limit the learning capacity at different stages.
However, not sharing parameters at all greatly increases the model size.
RPG can be created for each sub-network. Such design leads to a much smaller DoF, while parameters of different sub-networks are orthogonal by undergoing destructive changes.% instead of directly copy-paste.
%We superpose different sub-networks with one or more RPGs. Superposition sub-networks could have a much smaller model size, while parameters for different sub-networks undergo destructive changes instead of directly copy-paste.
%We show we can also create model rings that are used for recurrent networks. At each recurrence, the weights for recurrent networks are under destructive changes. 
We show applications of sub-network-level RPGs for pose estimation and multitask regression (Section \ref{sec:pose} and \ref{sec:multi}). Fig.\ref{fig:tasks}{\bf R}) illustrates sub-network-level RPGs.% with two different ways of network superposition.


==> 2107 (1)/Recurrent layers/sections/4results.tex <==
%\vspace{-1em}
\section{Experimental Results}

\label{sec:exp}
We evaluate the performance of RPG with various tasks illustrated in Fig.\ref{fig:tasks}. %\textcolor{red}{ We refer to model DoF as \textit{number of parameters} or \textit{parameter size} for convenience, although their differences have been discussed in Introduction.}
For classification, RPG was used for the entire network except for the last fully-connected layer. We discuss performance with regard to \textit{backbone DoF}, the actual number of parameters of the backbone. For example, Res18 has $11$M backbone parameters and $512$K fc parameters, and RPG was applied to reduce $11$M backbone DoF only.
%We conduct 3 sets of experiments to evaluate the proposed superposition method (with tasks illustrated in Fig.\ref{fig:tasks}). The first set benchmarks the performance of RPG networks on image classification datasets including CIFAR100 and ImageNet. %Specifically, 
%We compare with deep equilibrium models, a strong baseline on exploiting model capacity with limited model size. 
%The second set benchmarks the performance of RPG at block and sub-network level on human pose estimation and multi-task regression datasets. We compare with recurrent models as baselines.
%The last set provide additional analysis and ablation studies of RPG networks.
%Experiments are conducted on NVIDIA GeForce GTX 2080Ti GPUs.

%\vspace{-1em}
\subsection{CIFAR Classification}
%\vspace{-0.5em}

\label{sec:cifar_exp}
%We benchmark the performance of the proposed RPG network on CIFAR10 and CIFAR100 datasets. 

\noindent \textbf{Implementation Details}. CIFAR experiments use 128 batch size, 5e-4 weight decay,  initial learning rate of 0.1 with gamma of 0.1 at epoch 60, 120 and 160. We use Kaiming initialization \cite{he2015delving} with adaptive scaling. Shared parameters are initialized with a particular variance and scale the parameters for each layer to make it match the Kaiming initialization.

\begin{table}[b]
\vspace{-1em}
\parbox{\linewidth}{
\vspace{-0.03in}
\caption{ \small RPG compared with multiscale deep equilibrium models (MDEQ) \cite{bai2020multiscale} on CIFAR10 and CIFAR100 classification. At the same number of model DoF, RPG achieves 3\% - 6\% performance gain with 15 - 25x less inference time. Inference time is measured by milliseconds per image.}
\label{tab:cifar-deq}
\centering
%\LARGE
\vspace{-0.7em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
%\rowcolor{LightCyan}
                          &  & \multicolumn{3}{c}{ {\bf Our RPG (same DoF)} }    \\\cline{3-5} 
  \multirow{-2}{*}{ {\bf Accuracy} (\%)}  &   \multirow{-2}{*}{\bf MDEQ}                & {\bf 2x MS blk} & {\bf 3x MS blk} & {\bf 4x MS blk} \\ \hline
{\bf CIFAR10 }   & 85.1                  & 88.5         & 90.1         & \textbf{90.9}         \\ \hline
{\bf CIFAR100}   & 59.8                  & 62.8         & 64.7         & \textbf{65.7}         \\ \hline\hline
{\bf Inference time (ms)} & 3.15                 & \textbf{0.12}         & 0.18         & 0.22         \\ \hline
\end{tabular}}
}
\vfill
\vspace{0.5em}
\parbox{\linewidth}{
\centering
%\LARGE
\caption{  \small ResNet-RPG outperforms existing DoF reduction methods \cite{han2015deep,chen2015compressing,yang2019legonet} on CIFAR100.
Additionally, a global RPG outperforms block-wise local RPGs.
%At the same number of backbone DoF on CIFAR100, using local RPGs at block-level improves accuracy. Using a global RPG further improves the accuracy. RPG also outperforms baseline methods.
}
\label{tab:cifar-block}
\vspace{-0.7em}
\resizebox{0.7\linewidth}{!}{\begin{tabular}{l|c|c}
\hline  & {\bf DoF} & {\bf Acc. (\%)} \\ \hline
{\bf R18-vanilla}             & 11M               & 77.5      \\ \hline
{\bf R34-RPG.blk} & 11M               & 78.5      \\ \hline
{\bf R34-RPG}            & 11M               & \textbf{78.9}      \\ \hline \hline
{\bf R34-random weight share}& 11M               & 74.9     \\\hline
{\bf R34-DeepCompression} \cite{han2015deep}& 11M               & 72.2    \\\hline
{\bf R34-Hash} \cite{chen2015compressing}& 11M               & 75.6     \\\hline
{\bf R34-Lego} \cite{yang2019legonet}& 11M               & 78.4     \\\hline\hline
{\bf R34-vanilla}              & 21M% 21,258,240 
& \textbf{79.1}      \\ \hline
\end{tabular}
}
}
\end{table}

\noindent \textbf{Compared to Deep Equilibrium Models}. As a representative of implicit models, deep equilibrium models \cite{bai2019deep}  reduce model DoF by finding fix points via additional optimizations. We compare the image classification accuracy on CIFAR10 and CIFAR100, as well as the inference time on CIFAR100 (Table \ref{tab:cifar-deq}). Following the settings of MDEQ \cite{bai2020multiscale}, an image was sequentially fed into the initial convolutional block, the multi-scale deep equilibrium block (dubbed as \textit{MS} block), and the classification head. 
MDEQ \cite{bai2020multiscale} achieves \textit{infinite} MS blocks by finding the fixed point of the MS block.  We reuse the MS block two to four times without increasing the model DoF. RPG achieves 3\% - 6\% gain on CIFAR10 and 3\% - 6\% gain on CIFAR100. RPG inference time is 15 - 25 times smaller than MDEQ since MDEQ needs additional time to solve equilibrium during training.

%CIFAR10: MDEQ 85.1\%; ours loop twice 88.53\%, loop 3 times 90.1\%, loop 4 times 90.87\%.

%CIFAR100: MDEQ 59.75\%; ours loop twice 62.83\%, loop 3 times 64.74\%, loop 4 times 65.74\%.

%%Time (ms/per image): MDEQ: 804.7504425048828/128; ours loop twice 14.95671272277832/128, loop 3 times 22.687673568725586/128, loop 4 times 28.149127960205078/128.
%Time (ms/per image): MDEQ: 6.29; ours loop twice 0.12, loop 3 times 0.18, loop 4 times 0.22


\begin{figure}
    \centering
   \includegraphics[width=\columnwidth]{figures/combo1.pdf}
    \caption{\small {\bf a)} Large models are known to have high redundancy and low degree of freedom (DoF). They could be pruned to small models, e.g. high filter similarity of different layers in VGG16 is observed. {\bf b)} Ablation studies of permutation and sign reflection of Res34-RPG. Having both matrices gives the highest performance.}
    \label{fig:combo1}
      \vspace{-1.5em}
\end{figure}

\iffalse
\begin{figure*}[t!]
\centering
\resizebox{0.29\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
   % \vspace{-1em}
 \includegraphics[width=0.8\columnwidth]{figures/filter_sim.pdf}
\caption{ \small Large models are known to have high redundancy and low degree of freedom (DoF). They could be pruned to small models, e.g. high filter similarity of different layers in VGG16 is observed.}
\label{fig:filter_sim}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
    \vspace{-1em}
 \includegraphics[width=\columnwidth]{figures/cifar_nparam.pdf}
\caption{ \small Log-linear DoF-accuracy relationship of CIFAR100 accuracy and model DoF on CIFAR100. 
%CIFAR100 accuracy versus the backbone DoF for ResNet-vanilla and RPG.
RPG achieves the same accuracy as vanilla ResNet with 50\% DoF.}
\label{fig:cifar-nparam}
\end{minipage}}
\hfill
\resizebox{0.35\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=0.95\columnwidth]{figures/ablation.pdf}
   \caption{  \small Ablation studies of permutation and sign reflection of Res34-RPG. Having both matrices gives the highest performance.}
   \label{fig:ablation}
     \vspace{-2em}

\end{minipage}}
\vspace{-1.2em}
\end{figure*}
\fi

\noindent \textbf{Global RPG with Varying Model DoF.} 
We create one global RPG to generate parameters for convolution layers of ResNet and refer to it as \textit{ResNet-RPG}.
We report CIFAR100 top-1 accuracy of ResNet-RPG18 and ResNet-RPG34 at different model DoF (Table \ref{tab:imagenet} and Fig.\ref{fig:cifar-nparam} in Appendix \ref{sec:cifar_supp}).
Compared to ResNet, ResNet-RPG achieves higher accuracy at the same model DoF. Specifically, we achieve 36\% CIFAR100 accuracy with only 8K backbone DoF. Further, ResNet34-RPG achieves higher accuracy than ResNet18-RPG, indicating increasing time complexity gives performance gain. We observe log-linear DoF-accuracy relationship, with details in \textit{Power Law} of the following subsection.

\noindent \textbf{Local RPGs at the Block-Level}. 
In the previous Res-RPG experiments, we use one global RPG for the entire network. %(Fig.\ref{fig:msparam}-\textbf{Upper}).%the equalization technique (mentioned in Section \ref{sec:method:ls}) so that parameters of different convolutional layers are evenly sampled from the model ring. 
We also evaluate the performance when RPGs are shared locally at a block level, as discussed in Section \ref{sec:multi}.
In Table \ref{tab:cifar-block}, compared to plain ResNet18 at the same DoF, our block-level RPG network gives 1.0\% gain. In contrast, our ResNet-RPG (parameters are evenly distributed) gives a 1.4\% gain.
Using one global RPG where parameters of each layer are evenly distributed is 0.4\% higher than multiple RPGs. %The gain comes from the equalization technique.
%We compare using one model ring shared by all layers versus parameters shared by corresponding blocks (Table \ref{tab:cifar-block}). Using a model ring shared by all layers leads to 0.4\% higher accuracy.
%CIFAR10: resnet18 baseline: 95.49\%, resnet18 extend to 34: 95.52\%, resnet34 baseline: 95.57\%

%%% CIFAR100: resnet18 baseline: 77.57\%, resnet18 extend to 34 (block reuse): 78.2\%, resnet18 extend to 34 (superparam): 78.6\% , resnet34 baseline: 79.10\%.

\noindent \textbf{Comparison to Baselines.} Table \ref{tab:cifar-block} compares RPG and other model DoF reduction methods including random weight sharing, weight sharing with the deep compression \cite{han2015deep}, hashing trick \cite{chen2015compressing} and weight sharing with Lego filters \cite{yang2019legonet}. We also compare with HyperNetworks \cite{ha2016hypernetworks} in Appendix \ref{sec:hypernet}. At the same model DoF, RPG outperforms all other baselines, demonstrating the effectiveness of the proposed method. 

\noindent \textbf{RPG for Transformers.} We apply RPG for a vision transformer ViT \cite{dosovitskiy2020image} and report results in %Table \ref{tab:vit} and
Fig.\ref{fig:combo2}{\bf a}. Specifically, the ViT-tiny model with 6 transformer layers, 4 attention heads and 64 embedding dimensions, is used as a baseline. A log-linear relationship is also identified in ViT-RPG.


\subsection{ImageNet Classification}
\vspace{-0.5em}

\noindent \textbf{Implementation Details}. All ImageNet experiments use batchsize of 256, weight decay of 3e-5, and an initial learning rate of 0.3 with gamma of 0.1 every 75 epochs and 225 epochs in total. Our schedule is different from the standard schedule as the weight-sharing mechanism requires different training dynamics. We tried a few settings and found this one to be the best for RPG.

\noindent \textbf{RPG with Varying Model DoF.} We use RPG with different DoF for ResNet and report the top-1 accuracy (Table \ref{tab:imagenet} and Fig.\ref{fig:teaser}\textbf{e})). ResNet-RPGs consistently achieve higher performance than ResNets under the same model DoF. Specifically, ResNet-RPG34 achieves the same accuracy 73.4\% as ResNet34 with only half of ResNet34 backbone DoF. ResNet-RPG18 also achieves the same accuracy as ResNet18 with only half of ResNet18 backbone DoF. Further, RPG networks have higher generalizability (Section \ref{sec:general}).

\begin{table}[t!]
\centering
\LARGE
\caption{ \small ResNet-RPG consistently achieves higher performance at the same model DoF. We report ImageNet and CIFAR100 top-1 accuracy and backbone DoF for ResNet-vanilla and ResNet-RPG. }
\vspace{-0.3em}
\label{tab:imagenet}
%\vspace{0.2in}
\setlength{\tabcolsep}{20pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
         {\bf Acc. (\%)}      & \multicolumn{3}{c|}{ \bf R18-RPG} &  {\bf R18-vanilla} & \multicolumn{3}{c|}{ \bf R34-RPG} & {\bf R34-vanilla} \\ \hline

{\bf ImageNet }            & 40.0             & 67.2 & 70.5   & 70.5          & 41.6       & 69.1      & \textbf{73.4}   & \textbf{73.4}   \\ \hline
{\bf CIFAR100  }        &60.2              & 75.6& 77.6    & 77.6        & 61.7       & 76.5      & \textbf{78.9}   &\textbf{79.1}   \\ \hline\hline
{\bf Model DoF }          & 45K              & 2M        & 5.5M   & 11M    & 45K         & 2M        & 11M    & 21M     \\ \hline 
\end{tabular}}
\vspace{-1.5em}

\end{table}

\noindent \textbf{Power Law.} Empirically, accuracy and model DoF follow a power law, when RPG DoF is lower than 50\% ResNet-vanilla DoF (Fig.\ref{fig:teaser}{\bf d}).
The exponents of the power laws are the same for ResNet18-RPG and ResNet34-RPG on ImageNet.
The scaling law may be useful for estimating the network accuracy without training the network.
Similarly, \cite{henighan2020scaling} also identifies a power law for accuracy and model DoF of transformers.
The proposed RPG enables {\it under-parameterized} models for large-scale datasets such as ImageNet, which may unleash more new studies and findings.

%\textbf{Compared to MDEQ}. MDEQ \cite{bai2020multiscale} achieves 75.2\% top-1 accuracy on ImageNet. We use our model ring at the same number of model parameters and lower inference time and achieves \textcolor{red}{XXX}.
%MDEQ baseline: 75.2\%. ours: 74.3\%.


\iffalse
\textbf{ResNet Experiment logs}.

\begin{itemize}
    % \item Resnet18 (modified to 34) IMAGENET: Top1 val acc: $70.94 \%$ , Top5 val acc: $90.00 \%$
    \item Resnet18 (baseline) IMAGENET: Top1 val acc: $69.80 \%$, Top5 val acc $89.18 \%$:
    \item Resnet34 (baseline) IMAGENET: Top1 val acc: $73.4 \%$, Top5 val acc: $91.4 \%$
    
    \item ResNet-rpg18 (512x512x3x3) IMAGENET: 3E-5 wd, 0.3*0.1**(ep/75.) for 250 epochs learning schedule, new initialization, final accuracy on validation set: Acc@1 67.2\% Acc@5 87.4\%
    
    \item ResNet-rpg34 (512x512x3x3) IMAGENET: ResNet-rpg34, 5E-5 wd, 0.3*0.1**(ep/75.) for 250 epochs learning schedule, final accuracy on validation set:  Acc@1 69.1\% Acc@5 88.7\%
    
    \item ResNet-rpg34 (11.16M, 512x3x3x2422) IMAGENET: Acc@1: 73.4\%, Acc@5 91.2\%
    
\end{itemize}
\fi

\vspace{-0.5em}
\subsection{Pose Estimation}
\vspace{-0.5em}

\label{sec:pose}



\begin{table}[b]
\parbox{\linewidth}{

\centering
\LARGE
\caption{ \small RPG outperforms CPM \cite{wei2016convolutional} at the same DoF. We report pose estimation performance (model DoF) on MPII human pose compared with CPM \cite{wei2016convolutional}. The metric is PCKh@0.5. }
\label{tab:pck}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c|c}
\hline
    {\bf Acc. (DoF)}  & {\bf CPM} \cite{wei2016convolutional}  & {\bf RPG}   & {\bf No shared w.} \\ \hline
{\bf 1x sub-net}  & \multicolumn{3}{c}{84.7 (3.3M)}         \\ \hline
{\bf 2x sub-nets} & 86.1 (3.3M) & 86.5 (3.3M) & 87.1 (6.7M)  \\ \hline
{\bf 4x sub-nets} & 86.5 (3.3M) & 87.3 (3.3M) & 88.0 (13.3M) \\ \hline
\end{tabular}}

}
\vfill
\vspace{0.3em}
\parbox{\linewidth}{
\centering
\LARGE
\caption{ \small RPG achieves the best accuracy without sharing batch normalize parameters and with permutation and sign reflection. We report multitask regression errors on S3DIS with sub-net architecture as  \cite{ramamonjisoa2019sharpnet}. % \cite{armeni2017joint}.
Lower is better. All methods share the same DoF. Sub-net is reused once.}
\label{tab:multitask}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c}
\hline
    {\bf RMSE} (\%) & {\bf Depth} & {\bf Normal} \\ \hline
{\bf Vanilla model} & 25.5     & 41.0      \\ \hline
{\bf RPG with shared BN}                                & 24.7     & 40.3      \\ \hline
{\bf Reuse \& new BN}                           & 24.0     & 39.4     \\ \hline
{\bf Reuse \& new BN \& perm. and reflect.} & \textbf{22.8}     & \textbf{39.1}      \\ \hline
\end{tabular}}
}
\end{table}
\noindent \textbf{Implementation Details.}
We superpose sub-networks for pose estimation with a globally shared RPG. %(Fig.\ref{fig:pose}).
Hourglass networks \cite{newell2016stacked} are used as the backbone.
An input image is first fed to an initial convolution block to obtain a feature map, which is then fed to multiple stacked pose estimation sub-networks. Each sub-network outputs a pose estimation prediction, which is penalized by the pose estimation loss. 
Convolutional pose machine (CPM) \cite{wei2016convolutional} share all sub-networks weights. 
We create one global RPG to generate parameters for each sub-network. Our model size is set to the same as CPM. We also compare with larger models where parameters of sub-networks are not shared.

We evaluate on MPII Human Pose dataset \cite{andriluka20142d}, a benchmark for articulated human pose estimation, which consists of over 28K training samples over 40K people with annotated body joints. We use the hourglass network \cite{newell2016stacked} as backbone and follow all their settings. 

\noindent \textbf{Results and Analysis.} We report the Percentage of Correct Key-points at 50\% threshold (PCK@0.5) of different methods in Table \ref{tab:pck}. 
CPM \cite{wei2016convolutional} share all parameters for different sub-networks. We use one RPG that is shared globally at the same size as CPM. For reference, we also compare with the no-sharing model as the performance ceiling.
Adding the number of recurrences leads to performance gain for all methods. 
At the same model size, RPG achieves higher PCK@0.5 compared to CPM. Increasing the number of parameters by not sharing sub-network parameters also leads to some performance gain.

%metric: PCKh@0.5\\
%- 1 model (3.3M) 84.7\\
%- 2 models: cpm (3.3M) 86.1, our super (3.3M) 86.5, different weight (6.7M) 87.1\\
%- 4 models: cpm (3.3M) 86.5, our super (3.3M) 87.3, different weight (13.3M) 88.0
\iffalse
\begin{figure}[t]\centering
  \vspace{-0.12in}
    \includegraphics[width=0.62\columnwidth]{figures/subnet_pose.pdf}
\caption{ Pose estimation  with sub-network RPG.
   An input image is fed to an initial convolutional block and $N$ stacked pose estimation networks. Each sub-network predicts the pose that are penalized by corresponding loss. Parameters of each sub-network are generated from a global RPG.}
\label{fig:pose}
\end{figure}
\fi

\begin{figure*}
    \centering
   \includegraphics[width=\textwidth]{figures/combo2.pdf}
    \caption{\small {\bf a)} A log-linear DoF-accuracy relationship exists for RPGs applied to vision transformer ViT \cite{dosovitskiy2020image}. {\bf b)} RPG converges faster than the vanilla model. We plot the CIFAR10 accuracy (smoothed by moving average) versus training iterations for Res18-vanilla and Res18-RPG. RPG converges at 1k iterations while the vanilla model converges at 1.7k. {\bf c)} RPG consistently converges faster. The reduction becomes substantial with the increasing batchsize, e.g., at batchsize 1024, RPG takes $41\%$ less iterations to converge. Denote final accuracy as $P_f$, the convergence iteration is defined when current smoothed accuracy (by moving average) is within 5\% range of $P_f$.}
    \label{fig:combo2}
\end{figure*}

\iffalse
\begin{figure*}[t!]
\centering
\resizebox{0.33\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
    \vspace{-1em}
 \includegraphics[width=0.9\columnwidth]{figures/vit_nparam.pdf}
\caption{ \small A log-linear DoF-accuracy relationship exists for RPGs applied on vision transformer ViT \cite{dosovitskiy2020image}.
%The model accuracy and DoF plot of ViT-RPGs. The accuracy-DoF relationship also follows a log-linear relationship.
}
\label{fig:vit}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=\columnwidth]{figures/converge.pdf}
   \caption{  \small RPG converges faster than the vanilla model. We plot the CIFAR10 accuracy (smoothed by moving average) versus training iterations for Res18-vanilla and Res18-RPG. RPG converges at 1k iterations while vanilla model converges at 1.7k.
   }
   \label{fig:converge1}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=\columnwidth]{figures/batchsize.pdf}
   \caption{  \small RPG consistently converges faster than the vanilla R18. The reduction becomes substantial with the increasing batchsize, e.g. at batchsize 1024, RPG takes $41\%$ less iterations to converge. Denote final accuracy as $P_f$, the convergence iteration is defined when current smoothed accuracy (by moving average) is within 5\% range of $P_f$.}
   \label{fig:converge2}
\end{minipage}}
\vspace{-2em}
\end{figure*}
\fi
\vspace{-0.5em}
\subsection{Multi-Task Regression}
\vspace{-0.5em}

\label{sec:multi}

\iffalse
\begin{figure}
    \centering
 \includegraphics[width=\columnwidth]{figures/subnet_multi.pdf}
   \caption{\small Multi-task regression  with (sub-)network RPG. 
   An input image is fed to an initial network $G$ and $N$ stacked network $F_i$. Each network outputs depth and normal maps which are penalized by corresponding loss.
   We use multiple RPGs that are shared at corresponding building blocks of the network $F_i$.
   Note that network $G$ and $F_i$ do not share parameters as they take different inputs.}  %\captionof{figure}{A figure}
  \label{fig:multitask}
\end{figure}
\fi

\noindent \textbf{Implementation Details.} We superpose sub-networks for multi-task regression with multiple RPGs at the building-block level.
We  focus on predicting depth and normal maps from a given image. We stack multiple SharpNet \cite{ramamonjisoa2019sharpnet}, a network for monocular depth and normal estimation. 
Specifically, we create multiple RPGs at the SharpNet building-block level. That is, parameters of corresponding blocks of different sub-networks are generated from the same RPG.

We evaluate the monocular depth and normal prediction performance on a 3D indoor scene dataset \cite{armeni2017joint}, which contains over 70K images with corresponding depths and normals covering over 6,000 $\text{m}^2$ indoor area.
We follow all settings of SharpNet \cite{ramamonjisoa2019sharpnet}, a SOTA monocular depth and normal estimation method.

\noindent \textbf{Results and Analysis.} We report the mean square errors for depth and normal estimation in Table \ref{tab:multitask}. Compared to one-time inference without recurrence, our RPG network gives 3\% and 2\% gain for depth and normal estimation, respectively. Directly sharing weights but using new batch normalization layers decrease the performance by 1.2\% and 0.3\% for depth and normal. Sharing weights and normalization layers further decrease the performance by 0.7\% and 0.9\% for depth and normal.

%	Depth RMSE,	Normal RMSE\\
%shared \& mask\& change BN,	22.79\%,	39.05\%\\
%shared \& no mask nor permute\& change BN,	24.0\%,	39.4\%\\
%shared \& no mask nor permute\& no change BN,	24.7\%,	40.3\%\\
%one time baseline, 25.5\%,	41.0\%

%\textcolor{red}{Figure: visualizations of different methods}
\vspace{-0.5em}
\subsection{Pruning RPG}
\vspace{-0.5em}


\begin{table}[t]
\parbox{\linewidth}{
\vspace{-0.03in}
\caption{ \small RPG achieves higher post-pruning CIFAR10 accuracy and similar post-pruning accuracy drops as SOTA fine-grained pruning approach IMP \cite{frankle2019stabilizing}. Fine-grained pruning is used for reducing DoF.
%Comparison with fine-grained pruning for reducing model size. Compared with IMP \cite{frankle2019stabilizing} on CIFAR10, RPG achieves higher pruned accuracy and similar accuracy drops.
}
\label{tab:fprune}
\centering
\LARGE
\vspace{-0.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline

                           & {\bf acc before} & {\bf acc after ↓ DoF} & {\bf acc drop} & {\bf model DoF} \\ \hline
{\bf R18-IMP} \cite{frankle2019stabilizing} & 92.3       & 90.5               & 1.8      & 274k      \\ \hline
{\bf R18-RPG} & 95.0       & 93.0               & 2.0      & 274k      \\ \hline
\end{tabular}}
}
\vfill
\vspace{0.5em}
\parbox{\linewidth}{
\centering
\LARGE
\caption{ \small RPG achieves similar post-pruning ImageNet performance as SOTA coarse-grained apporach Knapsack \cite{aflalo2020knapsack} at the same FLOPs. Coarse-grained pruning is used for reducing RPG FLOPs.
%Comparison with coarse-grained pruning for reducing FLOPs and inference speed.RPG achieves similar performance as Knapsack \cite{aflalo2020knapsack} on ImageNet classification.
}
\label{tab:cprune}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c|c} \hline
   & {\bf DoF before pruning} & {\bf Pruned acc.} & {\bf FLOPs}  \\ \hline
{\bf R18-Knapsack}   & 11.2M                    & 69.35\%     & 1.09e9 \\ \hline
{\bf Pruned R18-RPG} & 5.6M                     & 69.10\%     & 1.09e9 \\ \hline
\end{tabular}
}
}
\vspace{-1em}
\end{table}

\noindent \textbf{Fine-Grained Pruning}. 
Fine-grained pruning methods aim to reduce the model DoF by sparsifying weight matrices.
Such methods usually do not reduce the inference speed, although custom algorithms \cite{sgk_sc2020} may improve the speed.
%Fine-grained pruning methods aim at reducing the model parameters, and generally cannot reduce the inference speed in practice. 
%RPG models can be directly compared to such methods as they share the same goal of reducing the number of parameters. 
At the same model DoF, RPG outperforms state-of-the-art fine-grained pruning method IMP \cite{frankle2019stabilizing}. Accuracy drops of RPG and IMP are similar, both around 2\% (Table \ref{tab:fprune}).
It is worth noting that although IMP has no run time improvement in regular settings,
it could save inference time with customized sparse GPU kernels \cite{sgk_sc2020}.

\noindent \textbf{Coarse-Grained Pruning}. While RPG is not designed to reduce FLOPs, it can be combined with coarse-grained pruning to reduce FLOPs. We prune RPG filters with the lowest $\ell_1$ norms. Table \ref{tab:cprune} shows that the pruned RPG achieves on-par performance as state-of-the-art coarse-grained pruning method Knapsack \cite{aflalo2020knapsack} at the same FLOPs.



\vspace{-0.5em}
\subsection{Analysis} 
\vspace{-0.5em}

\label{sec:general}


\begin{table*}[t]
%\vspace{-1em}
    \caption{ \small RPG increases the model generalizability. \textbf{(a)} ResNet-RPG has lower training-validation accuracy gap on ImageNet classification. The metric is training accuracy minus validation accuracy. Lower is better. \textbf{(b)} Using RPG for pose estimation also decreases the training and validation performance GAP.  The metric is training PCK@0.5 minus validation PCK@0.5. Lower is better. \textbf{(c)} ResNet with RPG has higher performance on out-of-distribution dataset ObjectNet \cite{barbu2019objectnet}. The model is trained on ImageNet only and directly evaluated on ObjectNet. }
        \vspace{-1em}

\label{tab:general}
    \begin{subtable}{.24\linewidth}
      \centering
        \caption{IN train-val gap}
\resizebox{\textwidth}{!}{\begin{tabular}{l|c|c}
\hline
{\bf Acc gap (\%)} & {\bf vanilla} & {\bf RPG} \\ \hline
{\bf R18} & -0.7   & {\bf -2.7}        \\ \hline
{\bf R34} & 1.1    & {\bf -2.3}        \\ \hline
\end{tabular}}
    \end{subtable}%
    \hfill
    \begin{subtable}{.38\linewidth}
      \centering
        \caption{Pose train-val gap}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
{\bf Acc gap (\%)} & {\bf no shared w} & {\bf shared w}  & {\bf RPG} \\ \hline
{\bf 2x sub-nets} & 1.15       & 1.13    & {\bf 0.64}      \\ \hline
{\bf 4x sub-nets} & 1.98       & 1.70    & {\bf 1.15}      \\ \hline
\end{tabular}}
    \end{subtable} 
    \hfill
    \begin{subtable}{.3\linewidth}
      \centering
        \caption{OOD on ObjectNet}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
 & {\bf R18} & {\bf R34-RPG} & {\bf R34} \\ \hline
{\bf DoF} & 11M   & 11M        & 21M   \\ \hline
{\bf Acc.} (\%) & 13.4  & {\bf 16.5}       & 16.0  \\ \hline
\end{tabular}}
    \end{subtable}
    \vspace{-1em}
\end{table*}


\noindent \textbf{Convergence rate.} Compared with the vanilla model, RPG optimizes in a parameter subspace $\hat{\mathbf{W}} =\boldsymbol{G} \mathbf{W}$ with fewer DoF. Would such constrained optimization lead to a faster convergence rate? We analyze the convergence rate of Res18-vanilla and Res18-RPG (DoF is 5.5M, 50\% of the vanilla model) with different batchsizes. All models are trained with multi-step SGD optimizer and they all reach $>94.1\%$ final CIFAR10 accuracy. For simplicity, we analyze the first optimization stage where learning rate has not decayed.

Fig.\ref{fig:combo2}{\bf b} plots the accuracy (smoothed with moving averages) v.s. training iterations with batchsize 1024. RPG has a faster convergence rate than vanilla models. We also analyze the smoothed accuracy and identify the convergence iteration versus batchsize in Fig.\ref{fig:combo2}{\bf c}. RPG consistently converges faster than the vanilla model, and the reduction becomes substantial with the increasing batchsize. %RPG consistently has lower convergence iteration than the vanilla model, and the gap is larger beyond batchsize 256. As RPG optimizes in small model space, batchsize needs to be large enough to ensure the model updates in a correct direction every iteration for a fast convergence.


\noindent \textbf{Comparison to Model Compression Methods}. 
 We report ResNet-RPG performance with different model DoF and existing compression methods on ImageNet (Fig.\ref{fig:teaser}\textbf{e}).
  RPG networks outperform SOTA methods such as \cite{aflalo2020knapsack,dong2019network,he2019filter,he2018soft,dong2017more,khetan2020prunenet}. For example, at the same model DoF, our RPG network has 0.6\% gain over the knapsack pruning \cite{aflalo2020knapsack}, a SOTA method of ImageNet pruning. 


\noindent \textbf{Storage.} RPG models only need to save the effective parameter $\mathbf{W}$, which has the size of the model DoF, since the generation matrix $G$ is saved as a random seed at no cost. The storage space of the model file can be diminished to satisfy a smaller storage limit for inference and a faster model file transfer. Empirically on PyTorch platform, ResNet18-vanilla model file is 45MB. With no accuracy loss, ResNet18-RPG model save file size is 23MB ($ \downarrow  49\%$). With 2 percentage point accuracy loss, RPG save file size is 9.5MB  ($ \downarrow  79\%$).
%Empirically on PyTorch platform for ResNet18, RPG model file achieves 

\noindent \textbf{Generalizability}. 
%To understand generalizability of proposed RPG networks, 
We report the performance gap between training and validation set on ImageNet (Table \ref{tab:general}(a)) and MPII pose estimation (Table \ref{tab:general}(b)). CPM \cite{wei2016convolutional} serves as the baseline pose estimation method. RPG models consistently achieve lower gaps between training and validation sets, indicating the RPG model suffers less from over-fitting.

We also report the out-of-distribution performance of RPG models. ObjectNet \cite{barbu2019objectnet} contains 50k images with 113 classes overlapping with ImageNet. Existing models are reported to have a large performance drop on ObjectNet. 
We directly evaluate the performance of ImageNet-trained model on ObjectNet without any fine-tuning (Table \ref{tab:general}(c)).
With the same backbone DoF, R18-RPG achieves a 3\% gain compared to R18-vanilla.
With the same network architecture design, R34-RPG achieves 0.5\% gain compared to R34.
This indicates RPG networks have higher out-of-distribution performance even with smaller model DoF.

%\textbf{Filter Similarity}.
%\textcolor{red}{TODO}

%\textbf{Filters Visualization}.
%\textcolor{red}{TODO}

\iffalse
\textbf{Feature Similarity}. 
RPG networks are small in DoF, are they still possible to prune?
Some work \cite{wang2019cop} achieves satisfactory pruning results by calculating the correlation matrix of a feature map from the network, and prune channels with high correlations. 
Following their settings, we report feature similarity of ResNet34-RPG after residual building block 3 (Fig.\ref{fig:featuresim}). From our small ResNet34-RPG with 45k backbone DoF to plain ResNet34 with 21M backbone DoF, the feature similarity gradually increases. 
This indicates our RPG networks can still be pruned, and the FLOPs and run time can be further reduced. We provide empirical pruning results in Appendix \ref{sec:supp1}.
\fi

\noindent \textbf{Quantization.} Network quantization can reduce model size with minimal accuracy drop. It is of interest to study if RPG models, whose parameters have been shrunk, can be quantized. After 8-bit quantization, the accuracy of ResNet18-RPG (5.6M DoF) only drop 0.1 percentage point on ImageNet, indicating RPG can be quantized for further model size reduction. Details are in Appendix \ref{sec:quantize}. 

\noindent \textbf{Security}. Permutation matrices generated by the random seed can be considered as security keys to decode the model. Further, only random seeds to generate generating matrix $G$ need to be saved and transferred at negligible cost.%, which is efficient in terms of size.

%\vspace{-1em}
\subsection{Ablation Studies}
\vspace{-0.5em}

\label{sec:ablation}
We conduct ablation studies on CIFAR100 to analyze functions of permutation and reflection matrices (Fig.\ref{fig:combo1}{\bf b}. 
We evaluate ResNet-RPG34 with 2M backbone DoF. Permutation and sign reflection together achieves 76.5\% accuracy, while permutation only achieves 75.8\%, and sign reflection only achieves 71.1\%. Training with neither permutation nor reflection matrices achieves 70.7\%. This suggests permutation and sign reflection matrices increase RPG performance.

%\textbf{Functions of Permutation and Reflection Matrices.}


%CIFAR100, resnet34, 2M: no perm nor mask: 70.7 \% ;no perm: 71.1\%; no mask: 75.8\%; with perm and mask: 76.5\%.
%CIFAR100, resnet18: no perm nor mask: 77.8\% ;no perm: 77.8\%; no mask: 78.3\%; with perm and mask: 78.2\%.
%\textbf{Number Parameters vs Accuracy}

==> 2107 (1)/Recurrent layers/sections/5summary.tex <==
%\vspace{-1em}

\section{Discussion}
\vspace{-0.5em}

 The common practice in neural network compression is to prune weights from a trained large model with many parameters or degrees of freedom (DoF).
 Our key insight is that a direct and drastically different approach might work faster and better: We start from a lean model with a small DoF, which can be linearly unpacked into a large model with many parameters. Then we can let the gradient descent automatically find the best model under the linear constraints. Our work is a departure from mainstream approaches towards model optimization and parameter reduction. We show how the model DoF and actual parameter size can be decoupled: we can define an arbitrary network of an arbitrary DoF.% (number of parameters). 

%Our RPG achieves on-par performance with SOTA fine-grained pruning methods. Another interesting finding is that the model accuracy shows a log-linear dependency on DoF (Section A of the supplementary). In other words, as the DoF is reduced by a factor of 2, the accuracy drop is only linear. RPG also provides a very strong baseline for parameter sharing methods.

We limit our scope to optimization with random linear constraints, termed destructive weight sharing. %for different convolutional layers. 
However, in general, there might also exist nonlinear RPGs and efficient nonlinear generation functions to create convolutional kernels from a shared model ring $\mathbf{W}$. 
Further, although RPG focuses on reducing model DoF, it can be quantized and pruned to further reduce the FLOPs and runtime.
%Additionally, although we focus on reducing model parameters, results in Fig.\ref{fig:featuresim} indicate RPG networks are compressible, and it is possible to further reduce the FLOPs and run time.

%(filter similarity: it is possible to compress other runtime efficient networks)

To sum up, we develop an efficient approach to build an arbitrarily complex neural network with any amount of DoF via a recurrent parameter generator.
On a wide range of applications, including classification, pose estimation and multitask regression, we show RPG consistently achieves higher performance at the same model DoF. Further, we show  such networks converge faster, are less likely to overfit and have higher performance on out-of-distribution data.

RPG can be added to any existing network flexibly with any amount of DoF at the user's discretion. It provides new perspectives for recurrent models, equilibrium models, and model compression. It also serves as a tool for understanding relationships between network properties and network DoF by factoring out the network architecture.
%The superposition method is general and can be applied to any given convolutional neural network for limiting model size for lower model redundancy.
%The model size is flexible and can be tailored at the user's discretion.

%{\small  \textbf{Reproducibility:} We provide our code in the supplementary.}

==> 2107 (1)/Recurrent layers/sections/old0abstract.tex <==
\begin{abstract}
Deep neural networks have achieved tremendous success as general optimization tools. To achieve higher accuracy, one has to frequently use a larger model with more parameters or degrees of freedom (DoF). A common practice of neural network compression is to prune weights from a trained large model. In this work, we explore a drastically different way of model DoF reduction. We start from a lean model with a small DoF, which can be linearly unpacked into a large model with many parameters. This can be viewed as constrained neural optimization, where the parameters have many predefined random linear constraints. We show that gradient descent can automatically find the best model under constraints with a faster convergence rate.
% The common practice in machine learning is to search for the best model in large model space with many parameters or degrees of freedom (DoF), and then shrink the optimal model for deployment. We start from a lean model with a small DoF, which can be unpacked into a large model with many parameters. We can then let the gradient descent automatically find the best model under the DoF constraint.
%The size of deep network parameters has been growing rapidly for higher performance, yet the relationship between network degree of freedom (DoF) and performance has been rarely studied. Model architecture becomes a factor for the study as it is coupled with DoF and hard to factorize. 
%We present a generic method for recurrently using the same parameters for  different layers of a deep network that decouples model architecture and DoF. 
Specifically, we create a recurrent parameter generator (RPG), from which the parameters of each layer are linearly generated. We demonstrate how to build a one-layer-size neural network to achieve similar performance as existing CNNs on various applications. For example, ResNet18 achieves $70\%$ ImageNet accuracy, while the RPG network built for it with the number of weights equivalent to one convolutional layer (or $18\%$ of the vanilla model size) achieves $67\%$ ImageNet top-1 accuracy. 
% We achieve significant performance gain compared to existing works. 
%Though using recurrent models to build a deep convolutional neural network (CNN) is not entirely new, our method achieves significant performance gain compared to the existing works. 
% We demonstrate how to build a one-layer-size neural network to achieve similar performance as other traditional CNNs on various applications.% and datasets.
%Furthermore, we demonstrate the RPG can be applied at different scales, such as layers, blocks, or even sub-networks. 
%Additionally, 
% For example, our RPG network built for ResNet18 with the number of weights equivalent to one convolutional layer of a vanilla ResNet achieves $67.2\%$ ImageNet top-1 accuracy. 
%We use the RPG to build a ResNet18 network with the number of weights equivalent to one convolutional layer of a conventional ResNet and show this model can achieve $67.2\%$ ImageNet top-1 accuracy. 
RPG allows us to build an arbitrarily complex neural network with any amount of parameters. For example, we build a ResNet34 with model DoF reduced by more than $400$ times, which still achieves $42\%$ ImageNet top-1 accuracy.
Furthermore, RPG can be further pruned and quantized for better run-time performance in addition to reducing DoF.
We provide a new tool to study the degree of freedom of a neural network and identify a log-linear relationship between model DoF and accuracy. Arguably most importantly, the discovery, supported by extensive experimental results, shows that constrained neural optimization has a significant potential for many applications.
% We also provide a new perspective for model compression.
% Rather than shrinking parameters from a large model, RPG sets a certain parameter-size constraint and 
% uses the gradient descent algorithm to automatically find the best model under the constraint. Extensive experimental results demonstrate the power of RPG.

%\keywords{ constrained neural optimization, parameter generator, degree of freedom, convergence rate}


%   The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
%   both the left- and right-hand margins. Use 10~point type, with a vertical
%   spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
%   bold, and in point size 12. Two line spaces precede the abstract. The abstract
%   must be limited to one paragraph.
\end{abstract}

==> 2107 (1)/Recurrent layers/sections/scratch_points.tex <==
\begin{table}[ht]
\begin{minipage}[b]{0.5\columnwidth}
\centering
\resizebox{0.55\textwidth}{!}{\begin{tabular}{>{\columncolor[gray]{0.95}}l|c|c}
\hline \rowcolor{LightCyan} & DoF  & Acc. (\%) \\ \hline
ViT-vanilla & 590k & 89.1          \\ \hline
ViT-1/2     & 295k & 89.0          \\ \hline
ViT-1/4     & 148k & 88.4          \\ \hline
ViT-1/8     & 74k  & 86.0          \\ \hline
ViT-1/16    & 37k  & 83.1          \\ \hline
ViT-1/32    & 18k  & 80.0          \\ \hline
ViT-1/64    & 9k   & 76.5          \\ \hline
\end{tabular}}
    \caption{\small ViT with RPG to achieve different model DoF and CIFAR10 classification accuracy.}
       \label{tab:vit}
    \label{table:student}
\end{minipage}\hfill
\begin{minipage}[b]{0.48\linewidth}
\centering
   \includegraphics[width=\columnwidth]{figures/vit_nparam.pdf}
\captionof{figure}{\small The model accuracy and DoF plot of ViT-RPGs. The accuracy-DoF relationship also follows a log-linear relationship. }
   \label{fig:vit}
\label{fig:image}
\end{minipage}
\end{table}

\textbf{Points to make}   
   
Limit model redundancy.
0) Inverse to model compression. 
Different direction of RNN - not sharing information
use time to exchange for performance. Squeeze out more capacity (aka reduce redundancy) Inspired by model superposition.

1) Related work: general RNN, CPM, DEQ, we propose a generic RNN mechanism

2) beat CPM, DEQ MDEQ (Done)

3) The method is generic and can be applied at multiple scales. layer (elementary and instructive - Double conv CIFAR10 - simplest model - maybe
3 layers? ), block, or even network.

4) Killer results besides CPM \& MDEQ:
MDEQ
1) tiny model on CIFAR10/100 (done)
2) large model on ImageNet

a) a single layer RESNET18 b)Extend RESNET 18 to deeper model and improve performance.

5) ablation studies

A graph: number of total parameters vs accuracy.
    a) under limited \# parameters, what is the highest accuracy? - capacity
    b) adding more layers - capacity? saturation
c) function of permutation and masking (done)

Advantages:
1) Use the full capacity of all parameters\\
2) Flexible parameters


\begin{table}
\parbox{.32\linewidth}{
\centering
\LARGE
\caption{\small Our SuperResNet models has lower gap between training and validation set and on ImageNet classification higher generalizability. The metric is training accuracy minus validation accuracy. Lower is better. }
\label{tab:gap1}
\resizebox{0.2\textwidth}{!}{\begin{tabular}{>{\columncolor[gray]{0.95}}l|c|c}
\hline
\rowcolor{LightCyan} & ResNet & Ours \\ \hline
18 conv & -0.7   & -2.7        \\ \hline
34 conv & 1.1    & -2.3        \\ \hline
\end{tabular}}
}
\hfill
\parbox{.33\linewidth}{
\centering
\caption{\small Our SuperResNet models has lower gap between training and validation set and on pose estimation higher generalizability. The metric is training accuracy minus validation accuracy. Lower is better.}
\label{tab:gap2}
\resizebox{0.33\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
\rowcolor{LightCyan}  & no shared w & shared w \cite{wei2016convolutional} & ours \\ \hline
2x sub-nets & 1.15       & 1.13    & 0.64      \\ \hline
4x sub-nets & 1.98       & 1.70    & 1.15      \\ \hline
\end{tabular}}
}
\hfill
\parbox{.3\linewidth}{
\centering
\LARGE
\caption{\small Our SuperResNet models have higher performance on out-of-distribution dataset ObjectNet \cite{barbu2019objectnet}. The model is trained on ImageNet only and directly evaluated on ObjectNet.}
\label{tab:object}
\resizebox{0.3\textwidth}{!}{\begin{tabular}{>{\columncolor[gray]{0.95}}l|c|c|c}
\hline
\rowcolor{LightCyan} & R18 & R34-rpg & R34 \\ \hline
\# Params & 11M   & 11M        & 21M   \\ \hline
Acc. (\%) & 13.4  & 16.5       & 16.0  \\ \hline
\end{tabular}}
}

\end{table}



\begin{table}
\parbox{\linewidth}{
\centering
\LARGE
\caption{\small Our SuperResNet models have higher performance on out-of-distribution dataset ObjectNet \cite{barbu2019objectnet}. The model is trained on ImageNet only and directly evaluated on ObjectNet.}
\label{tab:object}
\resizebox{0.4\textwidth}{!}{\begin{tabular}{>{\columncolor[gray]{0.95}}l|c|c|c}
\hline
\rowcolor{LightCyan} & Res18 & Our SuperRes34 & Res34 \\ \hline
\# Params & 11M   & 11M        & 21M   \\ \hline
Acc. (\%) & 13.4  & 16.5       & 16.0  \\ \hline
\end{tabular}}
}

\end{table}


\iffalse
\begin{figure}
\centering
\begin{minipage}{.3\textwidth}
  \centering
 \includegraphics[width=\columnwidth]{figures/subnet_multi.pdf}
   \caption{\small \textcolor{red}{place holder figure for orthogonal} Multi-task regression  with (sub-)network superposition. 
   An input image is fed to an initial network $G$ and $N$ stacked network $F_i$. Each network outputs depth and normal maps, which are penalized by corresponding loss.
   We use multiple model rings that are shared at corresponding building blocks of network $F_i$.
   Note that network $G$ and $F_i$ do not share parameters as they take different inputs.}  %\captionof{figure}{A figure}
  \label{fig:multitask}
\end{minipage}%
\hfill
\begin{minipage}{.68\textwidth}
  \centering
    \includegraphics[width=\columnwidth]{figures/subnet_pose.pdf}
   \caption{\small Pose estimation  with (sub-)network superposition.
   An input image is fed to an initial convolutional block and $N$ stacked pose estimation networks. Each network predicts the pose that is penalized by corresponding loss. We use one model ring
   }
  \label{fig:pose}
\end{minipage}
\end{figure}
\fi


\begin{figure}
\centering
\begin{minipage}{.62\textwidth}
  \centering
  \vspace{-0.12in}
    \includegraphics[width=\columnwidth]{figures/subnet_pose.pdf}
   \caption{ Pose estimation  with sub-network superposition.
   An input image is fed to an initial convolutional block and $N$ stacked pose estimation networks. Each sub-network predicts the pose that are penalized by corresponding loss. Parameters of each sub-network are generated from a global RPG.
   }
  \label{fig:pose}
\end{minipage}
\hfill
\begin{minipage}{.36\textwidth}
  \centering
 \includegraphics[width=\columnwidth]{figures/similarity.pdf}
   \caption{ Normalized histogram of feature similarity for Res34-RPG with different model parameters. Feature similarity increases as the model size decreases, indicating our RPG networks can be further pruned with methods like \citep{wang2019cop}.}  %\captionof{figure}{A figure}
  \label{fig:featuresim}
\end{minipage}%
\end{figure}

==> 2107 (1)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> 2107 (1)/sections/0abstract.tex <==
\begin{abstract}
Deep learning has achieved tremendous success 
by training increasingly large models, which are then compressed for practical deployment.  We propose a drastically different approach to compact and optimal deep learning:   
 We decouple the Degrees of freedom (DoF) and the actual number of parameters of a model, optimize a small DoF with predefined random linear constraints for a large model of an arbitrary architecture, in one-stage end-to-end learning.
 
Specifically, we create a recurrent parameter generator (RPG), which repeatedly fetches parameters from a ring  and unpacks them onto a large model with random permutation and sign flipping to promote parameter decorrelation.  We show that gradient descent can automatically find the best model under constraints with in fact faster convergence.

Our extensive experimentation reveals a log-linear relationship between model DoF and accuracy.  Our
 RPG demonstrates remarkable DoF reduction, 
and can be further pruned and quantized for additional  run-time performance gain.
For example, in terms of top-1 accuracy on ImageNet,
RPG achieves 96\% of ResNet18's performance with only 18\% DoF (the equivalent of one convolutional layer) and 52\% of ResNet34's performance with only 0.25\% DoF!
Our work shows significant potential of constrained neural optimization in compact and optimal deep learning.
\end{abstract}

==> 2107 (1)/sections/1intro.tex <==

\def\figModelRing#1{
\begin{figure}[#1]\centering
\vspace{-1.5em}
\includegraphics[width=0.92\columnwidth]{figures/modelRing.pdf}
\caption{ \small We propose a recurrent parameter generator (RPG) that shares a fixed set of parameters in a ring and use them to generate parameters of different parts of a neural network, %simply by permutations and sign flipping, 
whereas in the standard neural network, all the parameters are independent of each other, so the model gets bigger as it gets deeper. \textbf{Left}: The \textcolor{orange}{third} section of the model starts to overlap with the \textcolor{red}{first} section in the model ring, and all later layers 
 share generating parameters for possibly multiple times.
 \textbf{Right:} Employing the Recurrent Parameter Generator (RPG) for ResNet could reduce the model parameters to any size. Specifically, with only half ResNet34 backbone parameters, we achieve the same ImageNet top-1 accuracy. 
 We also outperform model compression methods such as Knapsack \cite{aflalo2020knapsack}.% and PruneNet \cite{khetan2020prunenet}.
}
\vspace{-1.5em}
\label{fig:modelRing}
\end{figure}
}

\def\figtasks#1{
\vspace{-1.5em}
\begin{figure*}[#1]\centering
\includegraphics[width=0.9\textwidth]{figures/tasks_v2.pdf}
\vspace{-1em}
\caption{ \small  We demonstrate the effectiveness of RPG on various applications including image classification (\textbf{Left}), human pose estimation (\textbf{Middle}), and multitask regression (\textbf{Right}). RPGs are shared at multiple scales: a network can either have a global RPG or multiple local RPGs that are shared within blocks or sub-networks.
}
\vspace{-1.5em}
\label{fig:tasks}
\end{figure*}
}

\section{Introduction}

\begin{figure}[t]
    \centering
 \includegraphics[width=\columnwidth]{figures/teaser.pdf}
   \caption{ \small 
   We propose a novel approach to compact and optimal deep learning by decoupling model DoF and model parameters.
   {\bf a}) Existing methods first finds the optimal in a large model space and then compress it for practical deployment.  
   {\bf b})  We propose to start with a small (DoF) model of free parameters, use 
   recurrent parameter generator (RPG) to unpack them onto a large model with predefined random linear projections. 
   {\bf c}) Gradient descent finds the optimal model of a small DoF under these linear constraints with faster converge than training the large unpacked model itself (Fig.\ref{fig:combo2}{\bf b}). 
   If the DoF is too small, the optimal large model may fall out of the constrained subpsace.  However, at a sufficiently large DoF,  RPG gets rid of redundancy and often finds a model with little loss in accuracy. 
    {\bf d}) RPG reveals a log-linear relationship between model DoF and accuracy.
   {\bf e}) RPG achieves the same ImageNet accuracy with half of the ResNet-vanilla DoF. RPG also outperforms other state-of-the-art compression approaches.
   }  
  \label{fig:teaser}
  \vspace{-1.5em}
\end{figure}

Deep neural networks as general optimization tools have achieved great success with increasingly more training data, deeper and larger neural networks:  A recently developed NLP model, GPT-3 \cite{brown2020language}, has astonishing 175 billion parameters!  
While the model performance generally scales with the number of parameters \cite{henighan2020scaling}, with parameters outnumbering training data, the model is significantly over-parameterized. 

Many approaches have been proposed to remove redundancy in trained large models: neural network pruning \cite{lecun1990optimal, han2015deep, liu2018rethinking}, efficient network design spaces \cite{howard2017mobilenets, iandola2016squeezenet, sandler2018mobilenetv2}, parameter regularization \cite{wan2013regularization, wang2020orthogonal, srivastava2014dropout, NowlanH92simplifying}, model quantization \cite{hubara2017quantized, rastegari2016xnor, louizos2018relaxed}, neural architecture search \cite{zoph2016neural, cai2018proxylessnas, wan2020fbnetv2}, recurrent models \cite{bai2019deep, bai2020multiscale, wei2016convolutional}, multi-task feature encoding \cite{ramamonjisoa2019sharpnet, hao2020multi}, etc. 
Pruning-based model compression dates back to the late 80s \cite{mozer1989using, lecun1990optimal} and has enjoyed recent resurgence \cite{han2015deep, blalock2020state}. They remove unimportant parameters from a pre-trained model and can achieve significant model compression.


 \begin{figure}[t]
    \centering
 \includegraphics[width=\columnwidth]{figures/genweight.pdf}
   \vspace{-1em}
   \caption{ \small
   {\bf Upper:} Networks are optimized with a linear constraint $\hat{\mathbf{W}} = \boldsymbol{G} \mathbf{W}$, where the constrained parameter $\hat{\mathbf{W}}$ of each network layer was generated by the generating matrix $\boldsymbol{G}$ from the free parameter $\mathbf{W}$, which is directly optimized. $\hat{\mathbf{W}}$ is unpacked large model parameter while the size of $\mathbf{W}$ is the model DoF.
   {\bf Lower:} This paper discusses a specific format of parameter generation, 
  recurrent parameter generator (RPG).
   RPG shares a fixed set of parameters in a ring and uses them to generate parameters of different parts of a neural network,
whereas in the standard neural network, all the parameters are independent of each other, so the model gets bigger as it gets deeper. The \textcolor{orange}{third} section of the model starts to overlap with the \textcolor{red}{first} section in the model ring, and all later layers 
 share generating parameters for possibly multiple times.
   }  %\captionof{figure}{A figure}
  \label{fig:modelring_}
  \vspace{-1.5em}
\end{figure}

Our work is a departure from mainstream approaches towards model optimization and parameter reduction: rather than compressing a large model, we directly optimize a lean model with a small set of free parameters (number of free parameters equal to degree of freedom of the model, or DoF), which can be linearly unpacked to a large model. Training the large model can be viewed as solving a neural optimization with a set of predefined linear constraints. One benefit of constrained neural optimization we observe is that it leads to a faster convergence rate (Section \ref{sec:general}).
Specifically, we define different layers in a neural network based on a fixed amount of DoF, which we call \textit{recurrent parameter generator} (RPG).
That is, we differentiate the number of model parameters and DoF.
Traditionally, model parameters are treated independently of each other; the total number of parameters equals DoF. However, by tapping into how a core set of free parameters can be assigned to the neural network model, we can develop a large model of many parameters, which are linearly constrained by the small set of free parameters.

There is excess capacity in neural networks independent of how and where the parameters are used in the network, even at the level of individual scalar values.
Surprisingly, backpropagation training of a deep network is able to cope with that the same parameter can be assigned to multiple random locations in the network without significantly impacting model performance. Our extensive experiments show that a large neural network does not need to be over-parameterized to achieve competitive performance. Particularly, a ResNet18 can be implemented with DoF equivalent to one convolution layer in a ResNet18-vanilla ($4.72\times$ DoF reduction) and still achieves $67.2\%$ ImageNet top-1 accuracy. The proposed method is also extremely flexible in reducing model DoF. In some sense, the proposed RPG method can be viewed as an automatic model DoF reduction technique, which explores the optimal accuracy-parameter trade-off. When we reduce the model DoF, RPG demonstrates graceful performance degradation, and its compression results are frequently on par with the SOTA pruning methods besides the flexibility. Even if we reduce the Res18 backbone DoF to $36$K, which is about $300\times$ reduction, ResNet18 can still achieve $40\%$ ImageNet top-1 accuracy. Further, we show RPG can be quantized and pruned to improve FLOPs and runtime with relatively
mild accuracy drops. 

To summarize, we make three contributions:
%\vspace{-0.5em}
\begin{enumerate*}
%\setlength{\itemsep}{-0em}
    \item We provide a new perspective towards automatic model size reduction: we define a neural network with certain DoF with random linear constraints. We discover that gradient descent can automatically solve constrained optimization for the best model with a faster convergence rate. This constrained neural optimization perspective is likely to benefit many other applications. % under the desired constraint.
    
    \item We propose the recurrent parameter generator (RPG), which decouples the network architecture and the network DoF. We can flexibly choose any desired DoF to construct the network given a specific neural network architecture. 

    \item By separating network architectures from parameters, RPG becomes a tool to understand the relationship between the model DoF and the network performance.  We observe an empirical log-linear DoF-Accuracy relationship.
\end{enumerate*}
\figtasks{t}


==> 2107 (1)/sections/2relatedworks.tex <==
\vspace{-0.5em}
\section{Related Work}
\vspace{-0.5em}
Many works study model DoF reduction or compression.
We discuss each one and its relationship to our work.

\noindent \textbf{Model Pruning, Neural Architecture Search, and Quantization.}
Model pruning seeks to remove unimportant parameters in a trained model. Recently, it's proposed to use neural architecture search as coarse-grained model pruning \cite{yu2018slimmable, dong2019network}. Another related effort is  network quantization \cite{hubara2017quantized, rastegari2016xnor, louizos2018relaxed}, which seeks to reduce the bits used for each parameter and can frequently reduce the model size by $4\times$ with minimal accuracy drop. More recently, \cite{dollar2021fast} presents a framework for analyzing model scaling strategies that consider network properties such as FLOPs and activations.

\noindent \textbf{Parameter Regularization and Priors}. 
Regularization has been widely used to reduce model redundancy \cite{krogh1992simple, NowlanH92simplifying}, alleviate overfitting \cite{srivastava2014dropout, wan2013regularization}, and ensure desired mathematical regularity \cite{wang2020orthogonal}. RPG can be viewed as a parameter regularization in the sense that weight sharing poses many equality constraints to  weights and regularizes  weights to a low-dimensional space. HyperNeat \cite{stanley2009hypercube} and CPPNs \cite{stanley2007compositional} use networks to determine the weight between two neurons as a function of their positions. \cite{karaletsos2018probabilistic, KaraletsosB20} introduced a similar idea by providing a hierarchical prior for network parameters.




\noindent \textbf{Recurrent Networks and Deep Equilibrium Models.} Recurrence and feedback have been shown in psychology and neuroscience to act as modulators or competitive inhibitors to aid feature grouping \cite{gilbert2007brain}, figure-ground segregation \cite{hupe1998cortical} and object recognition \cite{wyatte2012limits}. Recurrence-inspired mechanisms also achieve success in feed-forward models. There are two main types of employing recurrence based on if weights are shared across recurrent modules. ResNet \cite{he2016deep}, a representative of reusing similar structures without weight sharing, introduces parallel residual connections and achieves better performance by going deeper in networks. Similarly, some works \cite{szegedy2015going,srivastava2015highway} also suggest iteratively injecting thus-far representations to the feed-forward network useful. Stacked inference methods \cite{ramakrishna2014pose,wolpert1992stacked,weiss2010structured} are also related while they consider each output in isolation. Some find sharing weights across recurrent modules valuable. They demonstrate applications in temporal modelling \cite{weiss2010structured,shi2015convolutional,karpathy2015deep}, spatial attention \cite{mnih2014recurrent,butko2009optimal}, pose estimation \cite{wei2016convolutional,carreira2016human}, and so on \cite{li2016iterative,zamir2017feedback}. Such methods usually shine in modeling long-term dependencies. In this work, we recurrently share weights across different layers of a feedback network to reduce network redundancy. 

Given stacking weight-shared modules improve the performance, researchers consider running even infinite depth of such modules by making the sequential modules converge to a fixed point \cite{lecun1988theoretical,bai2019deep}. Employing such \textit{equilibrium} models to existing networks, they show improved performance in many natural language processing \cite{bai2019deep} and computer vision tasks \cite{bai2020multiscale,wang2020implicit}. One issue with deep equilibrium models is that the forward and backward propagation usually takes much more iterations than explicit feed-forward networks. Some work \cite{fung2021fixed} improves the efficiency by making the backward propagation Jacobian free. Another issue is that \textit{infinite} depth and fixed point may not be necessary or even too strict for some tasks. 
Instead of achieving infinite depth, our model shares parameters to a certain level. We empirically compare with equilibrium models in Section \ref{sec:exp}.


\noindent \textbf{Efficient Network Space and Matrix Factorization.}
Convolution is an efficient and structured matrix-vector multiplication. Arguably, the most fundamental idea in building efficient linear systems is matrix factorization. Given the redundancy in deep convolutional neural network parameters, one can leverage the matrix factorization concept, e.g., factorized convolutions, and design more efficient network classes \cite{howard2017mobilenets, iandola2016squeezenet, tan2019efficientnet, sandler2018mobilenetv2}.


==> 2107 (1)/sections/3methods.tex <==
%\vspace{-0.5em}
\section{Recurrent Parameter Generator}
%\vspace{-0.5em}

\label{sec:method:ls}


\noindent {\bf Linearly Constrained Neural Optimization.} 
% Parameter generator can be considered  as optimizing neural networks with linear constraints.
Consider optimizing a network with input data $\mathbf{X}$, parameters $\hat{\mathbf{W}}$ and loss function $L$. The optimization can be written as: 
\begin{align}
    \min L(\mathbf{X}; \hat{\mathbf{W}} )\ \ \text{s.t.}\  \mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W} (\text{or equally} \ \boldsymbol{R}\mathbf{\hat{\mathbf{W}}} = 0)
\end{align}
where $\mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W}$ refers to a set of linear constraints, where $\boldsymbol{G}\in \Re^{N\times M}$ is a full-rank tall matrix (i.e. $N\ge M$). Here we refer to $\hat{\mathbf{W}}$ as the constrained parameters and $\mathbf{W}$ as the free parameters. This constraint is a change of variable, i.e., the constrained parameter $\hat{\mathbf{W}}$ is linearly generated from the free parameter $\mathbf{W}$ by generating matrix $\boldsymbol{G}$. We can consider $\mathbf{W}$ as a compressed model, which is unpacked into $\hat{\mathbf{W}}$ to construct the large neural network. $\mathbf{W}$ is directly optimized via gradient descent and free to update. In this linearly constrained neural optimization, the model DoF is equivalent to $M$, which is the dimension of $\mathbf{W}$. An equivalent form of the constraint $\mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W}$ is $\boldsymbol{R}\mathbf{\hat{\mathbf{W}}} = 0$, where $\boldsymbol{R}\in\Re^{(N-M)\times N}$ can be derived from SVD of $\boldsymbol{G}$. 



\noindent {\bf Recurrent Parameter Generator.} Let's assume that we construct a deep convolutional neural network containing $L$ different convolution layers. Let $\mathbf{K}_1,\mathbf{K}_2,\dots, \mathbf{K}_L$ be the corresponding $L$ convolutional kernels\footnote{A kernel contains all the filters of one layer. In this paper, we treat each convolutional kernel as a vector. When the kernel is used to do the convolution, it will be reshaped into the corresponding shape.}. 
Rather than using separate sets of parameters for different convolution layers, we create a single set of parameters $\mathbf{W}\in\Re^M$ and use it to generate the corresponding parameters $\hat{\mathbf{W}} = \left[\mathbf{K}_1^T,\mathbf{K}_2^T,\dots, \mathbf{K}_L^T\right]^T \in \Re^N$ for each convolution layer:
\begin{equation}
\mathbf{K}_i = \boldsymbol{G}_i\cdot \mathbf{W}, i \in \{1,\dots,L\}
\label{eq:k}
\end{equation}
where $\boldsymbol{G}_i$ is a fixed predefined generating matrix, which is used to generate $\mathbf{K}_i$ from $\mathbf{W}$.
We call $\boldsymbol{G} = \left[\boldsymbol{G}_1^T,\dots,\boldsymbol{G}_L^T\right]^T$ and $\mathbf{W}$ the \textit{recurrent parameter generator} (RPG). In this work, we always assume that the size of $\mathbf{W}$ is not larger than the total parameters of the model, i.e., $|\mathbf{W}|\leq\sum_{i}{|\mathbf{K}_i|}$. This means an element of $\mathbf{W}$ will generally be used in more than one layer of a neural network. Additionally, the gradient of $\mathbf{W}$ is a linear superposition of the gradients from each convolution layer.
During the neural network training, let's assume convolution kernel $\mathbf{K}_i$ receives gradient $\frac{\partial \ell}{\partial \mathbf{K}_i}$, where $\ell$ is the loss function. Based on the chain rule, it is clear that the gradient of $\mathbf{W}$ is:
\begin{equation}
\frac{\partial \ell}{\partial \mathbf{W}} = \sum_{i=1}^{L}{\boldsymbol{G}^T_i\cdot \frac{\partial \ell}{\partial \mathbf{K}_i}}
\label{eq:grad_w}
\end{equation}
\noindent {\bf Generating Matrices and Destructive Weight Sharing.} There are various ways to create the generating matrices $\{\boldsymbol{G}_i\}$. While in general $\boldsymbol{G}$ can be any full-rank tall matrix, this paper focuses on the destructive generating matrices, which are random orthogonal matrices and could prevent different kernels from sharing the representation during weight sharing. Random generating matrices empirically improve the model capacity when the model DoF is fixed. We provide an intuitive theoretical explanation of how random orthogonal matrices prevent representation sharing as follows.


For easier discussion, let us consider a special case, where all of the convolutional kernels have the same size and are used in the same shape in the corresponding convolution layers. The dimension of $\mathbf{W}$ is equal to that of one convolutional layer kernel. In other words, $\{\boldsymbol{G}_i\}$ are square matrices, and the spatial sizes of all of the convolutional kernels have the same size, $d_{in}\times d_{out}\times w\times h$, and the input channel dimension $d_{in}$ is always equal to the output channel dimension $d_{out}$. In this case, a filter $\mathbf{f}$ in a kernel can be treated as a vector in $\Re^{dwh}$. Further, we choose $\boldsymbol{G}_i$ to be a block-diagonal matrix $\boldsymbol{G}_i=\text{diag}\{\boldsymbol{A}_i,\boldsymbol{A}_i,\dots,\boldsymbol{A}_i\}$, where $\boldsymbol{A}_i\in O(dwh)$ is an orthogonal matrix that generates each filter of the kernel $\mathbf{K}_i$ from $\mathbf{W}$, and $O(\cdot)$ denotes the orthogonal group. Similar to the Proposition~2 in \cite{CheungPSP19}, we show in the Appendix \ref{sec:supp2} that: if $\boldsymbol{A}_i$, $\boldsymbol{A}_j$ are sampled from the $O(dwh)$ Haar distribution and $\mathbf{f}_i$, $\mathbf{f}_j$ are the corresponding filters (generated by $\boldsymbol{G}_i$, $\boldsymbol{G}_j$ respectively from the same set of entries of $\mathbf{W}$) from $\mathbf{K}_i$, $\mathbf{K}_j$ respectively, then we have $\E\left[\langle \mathbf{f}_i,\mathbf{f}_j \rangle\right] = 0$ and $\E \left[\langle \frac{\mathbf{f}_i}{\|\mathbf{f}_i\|},\frac{\mathbf{f}_j}{\|\mathbf{f}_j\|}\rangle^2 \right]=\frac{1}{dwh}$. Since $dwh$ is usually large, the corresponding filters from $\mathbf{K}_i$, $\mathbf{K}_j$ are close to orthogonal and generally dissimilar. This shows that even when $\{\mathbf{K}_i\}$ are generated from the same entries of $\mathbf{W}$, they are prevented from sharing the representation.

Though $\{\boldsymbol{G}_i\}$ are not updated during training, the size of $\boldsymbol{G}_i$ can be quite large in general, which can create additional computation and storage overhead. In practice, we can use permutation and element-wise random sign reflection to construct a subset of the orthogonal group as permutations and sign reflections could be implemented with high simplicity and negligible cost. A simple demonstration of $\{\boldsymbol{G}_i\}$ is demonstrated in Fig.\ref{fig:modelring_}{\bf U}\footnote{Permutations and element-wise random sign reflection conceptually are subgroups from the orthogonal group, but we shall never use them in the matrix form for the obvious efficiency purpose.}. Since pseudo-random numbers are used, it takes only two random seeds to store a random permutation and an element-wise random sign reflection.



\noindent \textbf{Even Parameter Sampling and Model Ring.}
While it is easy to randomly sample elements from $\mathbf{W}$ when generating parameters for each layer, it may not be optimal as some elements in $\mathbf{W}$ may not be evenly used, and some elements in $\mathbf{W}$ used at all due to sampling fluctuation. 
A simple equalization technique can be used to guarantee all elements of $\mathbf{W}$ are evenly sampled.
Suppose the size of $\mathbf{W}$ is $M$, and the size of parameter $\mathbf{\hat{\mathbf{W}}}$  of the model to be generated is $N$, $N>M$. As we mentioned earlier, there are $L$ layers and they require $\{\|K_1\|,\dots,\|K_L\|\}$ parameters respectively. As $N>M$, we can use $W$ as a ring: we first draw the first $\|K_1\|$ parameters from $\mathbf{\hat{\mathbf{W}}}$ followed by a pre-generated random permutation $p_1$ and a  pre-generated random element-wise sign flipping $b_1$ to construct layer-1 kernel $\mathbf{K}_1$. Then we draw the next $\|K_2\|$ parameters from $\mathbf{\hat{\mathbf{W}}}$ followed by pre-generated random permutation $p_2$ and a pre-generated random element-wise sign flipping $b_2$. We continue this process and wrap around when there is not enough entries left from $\mathbf{\hat{\mathbf{W}}}$. We refer to $\mathbf{\hat{\mathbf{W}}}$ together with this sampling strategy as \textit{model rings} since the free parameters are recurrently used in a loop. We illustrate the general parameter generator in Fig.\ref{fig:modelring_}{\bf U} and RPG in Fig.\ref{fig:modelring_}{\bf L}. This For data saving efficiency, we just need to save several random seed numbers instead of saving the pre-generated permutations $\{p_1,\dots,p_L\}$ and sign flipping operations $\{b_1,\dots,b_L\}$.


\noindent \textbf{Batch Normalization.} Model performance is relatively sensitive to the batch normalization parameters. For better performance, each convolution layer needs to have its own batch normalization parameters. In general, however, the size of batch normalization is relatively negligible. Yet when $\mathbf{W}$ is extremely small (e.g., $36$K parameters), the size of batch normalization should be considered.

\iffalse
\begin{figure}[t]
    \centering
 \includegraphics[width=1\columnwidth]{figures/MSparam.pdf}
   \vspace{-1em}
   \caption{ \small Recurrent parameter generators at multiple scales. \textbf{Upper:} A global RPG is used for generating convolution kernels for the entire ResNet18. \textbf{Lower }: Four local RPGs are each responsible for generating convolution kernels within each corresponding building block of the ResNet18.}  %\captionof{figure}{A figure}
  \label{fig:msparam}
  \vspace{-1.5em}
\end{figure}
\fi

 % \vspace{-1em}
\section{RPG at Multiple Scales}
 % \vspace{-1em}

We discuss the general idea of parameter generators where only one RPG is shared globally across all layers previously. 
We could also create several local RPGs, each of which is shared at certain scales, such as blocks and sub-networks. Such RPGs may be useful for certain applications such as recurrent modeling. %Experimental results are reported in Section \ref{sec:cifar_exp}.

\label{sec:extension}
\noindent \textbf{RPGs at Block-Level.}
Many existing network architectures reuse the same design of network blocks multiple times for higher learning capacity, as discussed in the related work. 
Instead of using one global RPG for the entire network, we could alternatively create several RPGs that are shared within certain network blocks.
We take Res18 \cite{he2016deep} as a concrete example.% (Fig.\ref{fig:msparam}). 
Res18 has four building blocks. Every block has 2 residual convolution modules.
We create four local RPGs for Res18.
Each RPG is shared within the corresponding building block, where the size of the RPG is flexible and can be determined by users. Fig.\ref{fig:tasks}{\bf M}) illustrates how RPGs can be shared at the block-level.

\noindent \textbf{RPGs at Sub-Network-Level.} 
Reusing sub-networks, or recurrent networks, has achieved success in many tasks as they iteratively refine and improve the prediction.
Parameters are often shared when reusing the sub-networks.
This may not be optimal as sub-networks at different stages iteratively improve the prediction, and shared parameters may limit the learning capacity at different stages.
However, not sharing parameters at all greatly increases the model size.
RPG can be created for each sub-network. Such design leads to a much smaller DoF, while parameters of different sub-networks are orthogonal by undergoing destructive changes.
We show applications of sub-network-level RPGs for pose estimation and multitask regression (Section \ref{sec:pose} and \ref{sec:multi}). Fig.\ref{fig:tasks}{\bf R}) illustrates sub-network-level RPGs.

==> 2107 (1)/sections/4results.tex <==
%\vspace{-1em}
\section{Experimental Results}

\label{sec:exp}
We evaluate the performance of RPG with various tasks illustrated in Fig.\ref{fig:tasks}. 
For classification, RPG was used for the entire network except for the last fully-connected layer. We discuss performance with regard to \textit{backbone DoF}, the actual number of parameters of the backbone. For example, Res18 has $11$M backbone parameters and $512$K fc parameters, and RPG was applied to reduce $11$M backbone DoF only.

%\vspace{-1em}
\subsection{CIFAR Classification}
%\vspace{-0.5em}

\label{sec:cifar_exp}

\noindent \textbf{Implementation Details}. CIFAR experiments use 128 batch size, 5e-4 weight decay,  initial learning rate of 0.1 with gamma of 0.1 at epoch 60, 120 and 160. We use Kaiming initialization \cite{he2015delving} with adaptive scaling. Shared parameters are initialized with a particular variance and scale the parameters for each layer to make it match the Kaiming initialization.

\begin{table}[b]
\vspace{-1em}
\parbox{\linewidth}{
\vspace{-0.03in}
\caption{ \small RPG compared with multiscale deep equilibrium models (MDEQ) \cite{bai2020multiscale} on CIFAR10 and CIFAR100 classification. At the same number of model DoF, RPG achieves 3\% - 6\% performance gain with 15 - 25x less inference time. Inference time is measured by milliseconds per image.}
\label{tab:cifar-deq}
\centering
%\LARGE
\vspace{-0.7em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
%\rowcolor{LightCyan}
                          &  & \multicolumn{3}{c}{ {\bf Our RPG (same DoF)} }    \\\cline{3-5} 
  \multirow{-2}{*}{ {\bf Accuracy} (\%)}  &   \multirow{-2}{*}{\bf MDEQ}                & {\bf 2x MS blk} & {\bf 3x MS blk} & {\bf 4x MS blk} \\ \hline
{\bf CIFAR10 }   & 85.1                  & 88.5         & 90.1         & \textbf{90.9}         \\ \hline
{\bf CIFAR100}   & 59.8                  & 62.8         & 64.7         & \textbf{65.7}         \\ \hline\hline
{\bf Inference time (ms)} & 3.15                 & \textbf{0.12}         & 0.18         & 0.22         \\ \hline
\end{tabular}}
}
\vfill
\vspace{0.5em}
\parbox{\linewidth}{
\centering
%\LARGE
\caption{  \small ResNet-RPG outperforms existing DoF reduction methods \cite{han2015deep,chen2015compressing,yang2019legonet} on CIFAR100.
Additionally, a global RPG outperforms block-wise local RPGs.
}
\label{tab:cifar-block}
\vspace{-0.7em}
\resizebox{0.7\linewidth}{!}{\begin{tabular}{l|c|c}
\hline  & {\bf DoF} & {\bf Acc. (\%)} \\ \hline
{\bf R18-vanilla}             & 11M               & 77.5      \\ \hline
{\bf R34-RPG.blk} & 11M               & 78.5      \\ \hline
{\bf R34-RPG}            & 11M               & \textbf{78.9}      \\ \hline \hline
{\bf R34-random weight share}& 11M               & 74.9     \\\hline
{\bf R34-DeepCompression} \cite{han2015deep}& 11M               & 72.2    \\\hline
{\bf R34-Hash} \cite{chen2015compressing}& 11M               & 75.6     \\\hline
{\bf R34-Lego} \cite{yang2019legonet}& 11M               & 78.4     \\\hline\hline
{\bf R34-vanilla}              & 21M% 21,258,240 
& \textbf{79.1}      \\ \hline
\end{tabular}
}
}
\end{table}

\noindent \textbf{Compared to Deep Equilibrium Models}. As a representative of implicit models, deep equilibrium models \cite{bai2019deep}  reduce model DoF by finding fix points via additional optimizations. We compare the image classification accuracy on CIFAR10 and CIFAR100, as well as the inference time on CIFAR100 (Table \ref{tab:cifar-deq}). Following the settings of MDEQ \cite{bai2020multiscale}, an image was sequentially fed into the initial convolutional block, the multi-scale deep equilibrium block (dubbed as \textit{MS} block), and the classification head. 
MDEQ \cite{bai2020multiscale} achieves \textit{infinite} MS blocks by finding the fixed point of the MS block.  We reuse the MS block two to four times without increasing the model DoF. RPG achieves 3\% - 6\% gain on CIFAR10 and 3\% - 6\% gain on CIFAR100. RPG inference time is 15 - 25 times smaller than MDEQ since MDEQ needs additional time to solve equilibrium during training.


\begin{figure}
    \centering
   \includegraphics[width=\columnwidth]{figures/combo1.pdf}
    \caption{\small {\bf a)} Large models are known to have high redundancy and low degree of freedom (DoF). They could be pruned to small models, e.g. high filter similarity of different layers in VGG16 is observed. {\bf b)} Ablation studies of permutation and sign reflection of Res34-RPG. Having both matrices gives the highest performance.}
    \label{fig:combo1}
      \vspace{-1.5em}
\end{figure}

\iffalse
\begin{figure*}[t!]
\centering
\resizebox{0.29\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
   % \vspace{-1em}
 \includegraphics[width=0.8\columnwidth]{figures/filter_sim.pdf}
\caption{ \small Large models are known to have high redundancy and low degree of freedom (DoF). They could be pruned to small models, e.g. high filter similarity of different layers in VGG16 is observed.}
\label{fig:filter_sim}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
    \vspace{-1em}
 \includegraphics[width=\columnwidth]{figures/cifar_nparam.pdf}
\caption{ \small Log-linear DoF-accuracy relationship of CIFAR100 accuracy and model DoF on CIFAR100. 
RPG achieves the same accuracy as vanilla ResNet with 50\% DoF.}
\label{fig:cifar-nparam}
\end{minipage}}
\hfill
\resizebox{0.35\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=0.95\columnwidth]{figures/ablation.pdf}
   \caption{  \small Ablation studies of permutation and sign reflection of Res34-RPG. Having both matrices gives the highest performance.}
   \label{fig:ablation}
     \vspace{-2em}

\end{minipage}}
\vspace{-1.2em}
\end{figure*}
\fi

\noindent \textbf{Global RPG with Varying Model DoF.} 
We create one global RPG to generate parameters for convolution layers of ResNet and refer to it as \textit{ResNet-RPG}.
We report CIFAR100 top-1 accuracy of ResNet-RPG18 and ResNet-RPG34 at different model DoF (Table \ref{tab:imagenet} and Fig.\ref{fig:cifar-nparam} in Appendix \ref{sec:cifar_supp}).
Compared to ResNet, ResNet-RPG achieves higher accuracy at the same model DoF. Specifically, we achieve 36\% CIFAR100 accuracy with only 8K backbone DoF. Further, ResNet34-RPG achieves higher accuracy than ResNet18-RPG, indicating increasing time complexity gives performance gain. We observe log-linear DoF-accuracy relationship, with details in \textit{Power Law} of the following subsection.

\noindent \textbf{Local RPGs at the Block-Level}. 
In the previous Res-RPG experiments, we use one global RPG for the entire network.  
We also evaluate the performance when RPGs are shared locally at a block level, as discussed in Section \ref{sec:multi}.
In Table \ref{tab:cifar-block}, compared to plain ResNet18 at the same DoF, our block-level RPG network gives 1.0\% gain. In contrast, our ResNet-RPG (parameters are evenly distributed) gives a 1.4\% gain.
Using one global RPG where parameters of each layer are evenly distributed is 0.4\% higher than multiple RPGs. 

\noindent \textbf{Comparison to Baselines.} Table \ref{tab:cifar-block} compares RPG and other model DoF reduction methods including random weight sharing, weight sharing with the deep compression \cite{han2015deep}, hashing trick \cite{chen2015compressing} and weight sharing with Lego filters \cite{yang2019legonet}. We also compare with HyperNetworks \cite{ha2016hypernetworks} in Appendix \ref{sec:hypernet}. At the same model DoF, RPG outperforms all other baselines, demonstrating the effectiveness of the proposed method. 

\noindent \textbf{RPG for Transformers.} We apply RPG for a vision transformer ViT \cite{dosovitskiy2020image} and report results in %Table \ref{tab:vit} and
Fig.\ref{fig:combo2}{\bf a}. Specifically, the ViT-tiny model with 6 transformer layers, 4 attention heads and 64 embedding dimensions, is used as a baseline. A log-linear relationship is also identified in ViT-RPG.


\subsection{ImageNet Classification}
\vspace{-0.5em}

\noindent \textbf{Implementation Details}. All ImageNet experiments use batchsize of 256, weight decay of 3e-5, and an initial learning rate of 0.3 with gamma of 0.1 every 75 epochs and 225 epochs in total. Our schedule is different from the standard schedule as the weight-sharing mechanism requires different training dynamics. We tried a few settings and found this one to be the best for RPG.

\noindent \textbf{RPG with Varying Model DoF.} We use RPG with different DoF for ResNet and report the top-1 accuracy (Table \ref{tab:imagenet} and Fig.\ref{fig:teaser}\textbf{e})). ResNet-RPGs consistently achieve higher performance than ResNets under the same model DoF. Specifically, ResNet-RPG34 achieves the same accuracy 73.4\% as ResNet34 with only half of ResNet34 backbone DoF. ResNet-RPG18 also achieves the same accuracy as ResNet18 with only half of ResNet18 backbone DoF. Further, RPG networks have higher generalizability (Section \ref{sec:general}).

\begin{table}[t!]
\centering
\LARGE
\caption{ \small ResNet-RPG consistently achieves higher performance at the same model DoF. We report ImageNet and CIFAR100 top-1 accuracy and backbone DoF for ResNet-vanilla and ResNet-RPG. }
\vspace{-0.3em}
\label{tab:imagenet}
%\vspace{0.2in}
\setlength{\tabcolsep}{20pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
         {\bf Acc. (\%)}      & \multicolumn{3}{c|}{ \bf R18-RPG} &  {\bf R18-vanilla} & \multicolumn{3}{c|}{ \bf R34-RPG} & {\bf R34-vanilla} \\ \hline

{\bf ImageNet }            & 40.0             & 67.2 & 70.5   & 70.5          & 41.6       & 69.1      & \textbf{73.4}   & \textbf{73.4}   \\ \hline
{\bf CIFAR100  }        &60.2              & 75.6& 77.6    & 77.6        & 61.7       & 76.5      & \textbf{78.9}   &\textbf{79.1}   \\ \hline\hline
{\bf Model DoF }          & 45K              & 2M        & 5.5M   & 11M    & 45K         & 2M        & 11M    & 21M     \\ \hline 
\end{tabular}}
\vspace{-1.5em}

\end{table}

\noindent \textbf{Power Law.} Empirically, accuracy and model DoF follow a power law, when RPG DoF is lower than 50\% ResNet-vanilla DoF (Fig.\ref{fig:teaser}{\bf d}).
The exponents of the power laws are the same for ResNet18-RPG and ResNet34-RPG on ImageNet.
The scaling law may be useful for estimating the network accuracy without training the network.
Similarly, \cite{henighan2020scaling} also identifies a power law for accuracy and model DoF of transformers.
The proposed RPG enables {\it under-parameterized} models for large-scale datasets such as ImageNet, which may unleash more new studies and findings.



\iffalse
\textbf{ResNet Experiment logs}.

\begin{itemize}
    \item Resnet18 (baseline) IMAGENET: Top1 val acc: $69.80 \%$, Top5 val acc $89.18 \%$:
    \item Resnet34 (baseline) IMAGENET: Top1 val acc: $73.4 \%$, Top5 val acc: $91.4 \%$
    
    \item ResNet-rpg18 (512x512x3x3) IMAGENET: 3E-5 wd, 0.3*0.1**(ep/75.) for 250 epochs learning schedule, new initialization, final accuracy on validation set: Acc@1 67.2\% Acc@5 87.4\%
    
    \item ResNet-rpg34 (512x512x3x3) IMAGENET: ResNet-rpg34, 5E-5 wd, 0.3*0.1**(ep/75.) for 250 epochs learning schedule, final accuracy on validation set:  Acc@1 69.1\% Acc@5 88.7\%
    
    \item ResNet-rpg34 (11.16M, 512x3x3x2422) IMAGENET: Acc@1: 73.4\%, Acc@5 91.2\%
    
\end{itemize}
\fi

\vspace{-0.5em}
\subsection{Pose Estimation}
\vspace{-0.5em}

\label{sec:pose}



\begin{table}[b]
\parbox{\linewidth}{

\centering
\LARGE
\caption{ \small RPG outperforms CPM \cite{wei2016convolutional} at the same DoF. We report pose estimation performance (model DoF) on MPII human pose compared with CPM \cite{wei2016convolutional}. The metric is PCKh@0.5. }
\label{tab:pck}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c|c}
\hline
    {\bf Acc. (DoF)}  & {\bf CPM} \cite{wei2016convolutional}  & {\bf RPG}   & {\bf No shared w.} \\ \hline
{\bf 1x sub-net}  & \multicolumn{3}{c}{84.7 (3.3M)}         \\ \hline
{\bf 2x sub-nets} & 86.1 (3.3M) & 86.5 (3.3M) & 87.1 (6.7M)  \\ \hline
{\bf 4x sub-nets} & 86.5 (3.3M) & 87.3 (3.3M) & 88.0 (13.3M) \\ \hline
\end{tabular}}

}
\vfill
\vspace{0.3em}
\parbox{\linewidth}{
\centering
\LARGE
\caption{ \small RPG achieves the best accuracy without sharing batch normalize parameters and with permutation and sign reflection. We report multitask regression errors on S3DIS with sub-net architecture as  \cite{ramamonjisoa2019sharpnet}. % \cite{armeni2017joint}.
Lower is better. All methods share the same DoF. Sub-net is reused once.}
\label{tab:multitask}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c}
\hline
    {\bf RMSE} (\%) & {\bf Depth} & {\bf Normal} \\ \hline
{\bf Vanilla model} & 25.5     & 41.0      \\ \hline
{\bf RPG with shared BN}                                & 24.7     & 40.3      \\ \hline
{\bf Reuse \& new BN}                           & 24.0     & 39.4     \\ \hline
{\bf Reuse \& new BN \& perm. and reflect.} & \textbf{22.8}     & \textbf{39.1}      \\ \hline
\end{tabular}}
}
\end{table}
\noindent \textbf{Implementation Details.}
We superpose sub-networks for pose estimation with a globally shared RPG. %(Fig.\ref{fig:pose}).
Hourglass networks \cite{newell2016stacked} are used as the backbone.
An input image is first fed to an initial convolution block to obtain a feature map, which is then fed to multiple stacked pose estimation sub-networks. Each sub-network outputs a pose estimation prediction, which is penalized by the pose estimation loss. 
Convolutional pose machine (CPM) \cite{wei2016convolutional} share all sub-networks weights. 
We create one global RPG to generate parameters for each sub-network. Our model size is set to the same as CPM. We also compare with larger models where parameters of sub-networks are not shared.

We evaluate on MPII Human Pose dataset \cite{andriluka20142d}, a benchmark for articulated human pose estimation, which consists of over 28K training samples over 40K people with annotated body joints. We use the hourglass network \cite{newell2016stacked} as backbone and follow all their settings. 

\noindent \textbf{Results and Analysis.} We report the Percentage of Correct Key-points at 50\% threshold (PCK@0.5) of different methods in Table \ref{tab:pck}. 
CPM \cite{wei2016convolutional} share all parameters for different sub-networks. We use one RPG that is shared globally at the same size as CPM. For reference, we also compare with the no-sharing model as the performance ceiling.
Adding the number of recurrences leads to performance gain for all methods. 
At the same model size, RPG achieves higher PCK@0.5 compared to CPM. Increasing the number of parameters by not sharing sub-network parameters also leads to some performance gain.

\iffalse
\begin{figure}[t]\centering
  \vspace{-0.12in}
    \includegraphics[width=0.62\columnwidth]{figures/subnet_pose.pdf}
\caption{ Pose estimation  with sub-network RPG.
   An input image is fed to an initial convolutional block and $N$ stacked pose estimation networks. Each sub-network predicts the pose that are penalized by corresponding loss. Parameters of each sub-network are generated from a global RPG.}
\label{fig:pose}
\end{figure}
\fi

\begin{figure*}
    \centering
   \includegraphics[width=\textwidth]{figures/combo2.pdf}
    \caption{\small {\bf a)} A log-linear DoF-accuracy relationship exists for RPGs applied to vision transformer ViT \cite{dosovitskiy2020image}. {\bf b)} RPG converges faster than the vanilla model. We plot the CIFAR10 accuracy (smoothed by moving average) versus training iterations for Res18-vanilla and Res18-RPG. RPG converges at 1k iterations while the vanilla model converges at 1.7k. {\bf c)} RPG consistently converges faster. The reduction becomes substantial with the increasing batchsize, e.g., at batchsize 1024, RPG takes $41\%$ less iterations to converge. Denote final accuracy as $P_f$, the convergence iteration is defined when current smoothed accuracy (by moving average) is within 5\% range of $P_f$.}
    \label{fig:combo2}
\end{figure*}

\iffalse
\begin{figure*}[t!]
\centering
\resizebox{0.33\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
    \vspace{-1em}
 \includegraphics[width=0.9\columnwidth]{figures/vit_nparam.pdf}
\caption{ \small A log-linear DoF-accuracy relationship exists for RPGs applied on vision transformer ViT \cite{dosovitskiy2020image}.
}
\label{fig:vit}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=\columnwidth]{figures/converge.pdf}
   \caption{  \small RPG converges faster than the vanilla model. We plot the CIFAR10 accuracy (smoothed by moving average) versus training iterations for Res18-vanilla and Res18-RPG. RPG converges at 1k iterations while vanilla model converges at 1.7k.
   }
   \label{fig:converge1}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=\columnwidth]{figures/batchsize.pdf}
   \caption{  \small RPG consistently converges faster than the vanilla R18. The reduction becomes substantial with the increasing batchsize, e.g. at batchsize 1024, RPG takes $41\%$ less iterations to converge. Denote final accuracy as $P_f$, the convergence iteration is defined when current smoothed accuracy (by moving average) is within 5\% range of $P_f$.}
   \label{fig:converge2}
\end{minipage}}
\vspace{-2em}
\end{figure*}
\fi
\vspace{-0.5em}
\subsection{Multi-Task Regression}
\vspace{-0.5em}

\label{sec:multi}

\iffalse
\begin{figure}
    \centering
 \includegraphics[width=\columnwidth]{figures/subnet_multi.pdf}
   \caption{\small Multi-task regression  with (sub-)network RPG. 
   An input image is fed to an initial network $G$ and $N$ stacked network $F_i$. Each network outputs depth and normal maps which are penalized by corresponding loss.
   We use multiple RPGs that are shared at corresponding building blocks of the network $F_i$.
   Note that network $G$ and $F_i$ do not share parameters as they take different inputs.}  %\captionof{figure}{A figure}
  \label{fig:multitask}
\end{figure}
\fi

\noindent \textbf{Implementation Details.} We superpose sub-networks for multi-task regression with multiple RPGs at the building-block level.
We  focus on predicting depth and normal maps from a given image. We stack multiple SharpNet \cite{ramamonjisoa2019sharpnet}, a network for monocular depth and normal estimation. 
Specifically, we create multiple RPGs at the SharpNet building-block level. That is, parameters of corresponding blocks of different sub-networks are generated from the same RPG.

We evaluate the monocular depth and normal prediction performance on a 3D indoor scene dataset \cite{armeni2017joint}, which contains over 70K images with corresponding depths and normals covering over 6,000 $\text{m}^2$ indoor area.
We follow all settings of SharpNet \cite{ramamonjisoa2019sharpnet}, a SOTA monocular depth and normal estimation method.

\noindent \textbf{Results and Analysis.} We report the mean square errors for depth and normal estimation in Table \ref{tab:multitask}. Compared to one-time inference without recurrence, our RPG network gives 3\% and 2\% gain for depth and normal estimation, respectively. Directly sharing weights but using new batch normalization layers decrease the performance by 1.2\% and 0.3\% for depth and normal. Sharing weights and normalization layers further decrease the performance by 0.7\% and 0.9\% for depth and normal.

\vspace{-0.5em}
\subsection{Pruning RPG}
\vspace{-0.5em}


\begin{table}[t]
\parbox{\linewidth}{
\vspace{-0.03in}
\caption{ \small RPG achieves higher post-pruning CIFAR10 accuracy and similar post-pruning accuracy drops as SOTA fine-grained pruning approach IMP \cite{frankle2019stabilizing}. Fine-grained pruning is used for reducing DoF.
}
\label{tab:fprune}
\centering
\LARGE
\vspace{-0.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline

                           & {\bf acc before} & {\bf acc after ↓ DoF} & {\bf acc drop} & {\bf model DoF} \\ \hline
{\bf R18-IMP} \cite{frankle2019stabilizing} & 92.3       & 90.5               & 1.8      & 274k      \\ \hline
{\bf R18-RPG} & 95.0       & 93.0               & 2.0      & 274k      \\ \hline
\end{tabular}}
}
\vfill
\vspace{0.5em}
\parbox{\linewidth}{
\centering
\LARGE
\caption{ \small RPG achieves similar post-pruning ImageNet performance as SOTA coarse-grained apporach Knapsack \cite{aflalo2020knapsack} at the same FLOPs. Coarse-grained pruning is used for reducing RPG FLOPs.
%Comparison with coarse-grained pruning for reducing FLOPs and inference speed.RPG achieves similar performance as Knapsack \cite{aflalo2020knapsack} on ImageNet classification.
}
\label{tab:cprune}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c|c} \hline
   & {\bf DoF before pruning} & {\bf Pruned acc.} & {\bf FLOPs}  \\ \hline
{\bf R18-Knapsack}   & 11.2M                    & 69.35\%     & 1.09e9 \\ \hline
{\bf Pruned R18-RPG} & 5.6M                     & 69.10\%     & 1.09e9 \\ \hline
\end{tabular}
}
}
\vspace{-1em}
\end{table}

\noindent \textbf{Fine-Grained Pruning}. 
Fine-grained pruning methods aim to reduce the model DoF by sparsifying weight matrices.
Such methods usually do not reduce the inference speed, although custom algorithms \cite{sgk_sc2020} may improve the speed.
%Fine-grained pruning methods aim at reducing the model parameters, and generally cannot reduce the inference speed in practice. 
%RPG models can be directly compared to such methods as they share the same goal of reducing the number of parameters. 
At the same model DoF, RPG outperforms state-of-the-art fine-grained pruning method IMP \cite{frankle2019stabilizing}. Accuracy drops of RPG and IMP are similar, both around 2\% (Table \ref{tab:fprune}).
It is worth noting that although IMP has no run time improvement in regular settings,
it could save inference time with customized sparse GPU kernels \cite{sgk_sc2020}.

\noindent \textbf{Coarse-Grained Pruning}. While RPG is not designed to reduce FLOPs, it can be combined with coarse-grained pruning to reduce FLOPs. We prune RPG filters with the lowest $\ell_1$ norms. Table \ref{tab:cprune} shows that the pruned RPG achieves on-par performance as state-of-the-art coarse-grained pruning method Knapsack \cite{aflalo2020knapsack} at the same FLOPs.



\vspace{-0.5em}
\subsection{Analysis} 
\vspace{-0.5em}

\label{sec:general}


\begin{table*}[t]
%\vspace{-1em}
    \caption{ \small RPG increases the model generalizability. \textbf{(a)} ResNet-RPG has lower training-validation accuracy gap on ImageNet classification. The metric is training accuracy minus validation accuracy. Lower is better. \textbf{(b)} Using RPG for pose estimation also decreases the training and validation performance GAP.  The metric is training PCK@0.5 minus validation PCK@0.5. Lower is better. \textbf{(c)} ResNet with RPG has higher performance on out-of-distribution dataset ObjectNet \cite{barbu2019objectnet}. The model is trained on ImageNet only and directly evaluated on ObjectNet. }
        \vspace{-1em}

\label{tab:general}
    \begin{subtable}{.24\linewidth}
      \centering
        \caption{IN train-val gap}
\resizebox{\textwidth}{!}{\begin{tabular}{l|c|c}
\hline
{\bf Acc gap (\%)} & {\bf vanilla} & {\bf RPG} \\ \hline
{\bf R18} & -0.7   & {\bf -2.7}        \\ \hline
{\bf R34} & 1.1    & {\bf -2.3}        \\ \hline
\end{tabular}}
    \end{subtable}%
    \hfill
    \begin{subtable}{.38\linewidth}
      \centering
        \caption{Pose train-val gap}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
{\bf Acc gap (\%)} & {\bf no shared w} & {\bf shared w}  & {\bf RPG} \\ \hline
{\bf 2x sub-nets} & 1.15       & 1.13    & {\bf 0.64}      \\ \hline
{\bf 4x sub-nets} & 1.98       & 1.70    & {\bf 1.15}      \\ \hline
\end{tabular}}
    \end{subtable} 
    \hfill
    \begin{subtable}{.3\linewidth}
      \centering
        \caption{OOD on ObjectNet}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
 & {\bf R18} & {\bf R34-RPG} & {\bf R34} \\ \hline
{\bf DoF} & 11M   & 11M        & 21M   \\ \hline
{\bf Acc.} (\%) & 13.4  & {\bf 16.5}       & 16.0  \\ \hline
\end{tabular}}
    \end{subtable}
    \vspace{-1em}
\end{table*}


\noindent \textbf{Convergence rate.} Compared with the vanilla model, RPG optimizes in a parameter subspace $\hat{\mathbf{W}} =\boldsymbol{G} \mathbf{W}$ with fewer DoF. Would such constrained optimization lead to a faster convergence rate? We analyze the convergence rate of Res18-vanilla and Res18-RPG (DoF is 5.5M, 50\% of the vanilla model) with different batchsizes. All models are trained with multi-step SGD optimizer and they all reach $>94.1\%$ final CIFAR10 accuracy. For simplicity, we analyze the first optimization stage where learning rate has not decayed.

Fig.\ref{fig:combo2}{\bf b} plots the accuracy (smoothed with moving averages) v.s. training iterations with batchsize 1024. RPG has a faster convergence rate than vanilla models. We also analyze the smoothed accuracy and identify the convergence iteration versus batchsize in Fig.\ref{fig:combo2}{\bf c}. RPG consistently converges faster than the vanilla model, and the reduction becomes substantial with the increasing batchsize.

\noindent \textbf{Comparison to Model Compression Methods}. 
 We report ResNet-RPG performance with different model DoF and existing compression methods on ImageNet (Fig.\ref{fig:teaser}\textbf{e}).
  RPG networks outperform SOTA methods such as \cite{aflalo2020knapsack,dong2019network,he2019filter,he2018soft,dong2017more,khetan2020prunenet}. For example, at the same model DoF, our RPG network has 0.6\% gain over the knapsack pruning \cite{aflalo2020knapsack}, a SOTA method of ImageNet pruning. 


\noindent \textbf{Storage.} RPG models only need to save the effective parameter $\mathbf{W}$, which has the size of the model DoF, since the generation matrix $G$ is saved as a random seed at no cost. The storage space of the model file can be diminished to satisfy a smaller storage limit for inference and a faster model file transfer. Empirically on PyTorch platform, ResNet18-vanilla model file is 45MB. With no accuracy loss, ResNet18-RPG model save file size is 23MB ($ \downarrow  49\%$). With 2 percentage point accuracy loss, RPG save file size is 9.5MB  ($ \downarrow  79\%$).

\noindent \textbf{Generalizability}. 
We report the performance gap between training and validation set on ImageNet (Table \ref{tab:general}(a)) and MPII pose estimation (Table \ref{tab:general}(b)). CPM \cite{wei2016convolutional} serves as the baseline pose estimation method. RPG models consistently achieve lower gaps between training and validation sets, indicating the RPG model suffers less from over-fitting.

We also report the out-of-distribution performance of RPG models. ObjectNet \cite{barbu2019objectnet} contains 50k images with 113 classes overlapping with ImageNet. Existing models are reported to have a large performance drop on ObjectNet. 
We directly evaluate the performance of ImageNet-trained model on ObjectNet without any fine-tuning (Table \ref{tab:general}(c)).
With the same backbone DoF, R18-RPG achieves a 3\% gain compared to R18-vanilla.
With the same network architecture design, R34-RPG achieves 0.5\% gain compared to R34.
This indicates RPG networks have higher out-of-distribution performance even with smaller model DoF.


\iffalse
\textbf{Feature Similarity}. 
RPG networks are small in DoF, are they still possible to prune?
Some work \cite{wang2019cop} achieves satisfactory pruning results by calculating the correlation matrix of a feature map from the network, and prune channels with high correlations. 
Following their settings, we report feature similarity of ResNet34-RPG after residual building block 3 (Fig.\ref{fig:featuresim}). From our small ResNet34-RPG with 45k backbone DoF to plain ResNet34 with 21M backbone DoF, the feature similarity gradually increases. 
This indicates our RPG networks can still be pruned, and the FLOPs and run time can be further reduced. We provide empirical pruning results in Appendix \ref{sec:supp1}.
\fi

\noindent \textbf{Quantization.} Network quantization can reduce model size with minimal accuracy drop. It is of interest to study if RPG models, whose parameters have been shrunk, can be quantized. After 8-bit quantization, the accuracy of ResNet18-RPG (5.6M DoF) only drop 0.1 percentage point on ImageNet, indicating RPG can be quantized for further model size reduction. Details are in Appendix \ref{sec:quantize}. 

\noindent \textbf{Security}. Permutation matrices generated by the random seed can be considered as security keys to decode the model. Further, only random seeds to generate generating matrix $G$ need to be saved and transferred at negligible cost.%, which is efficient in terms of size.

%\vspace{-1em}
\subsection{Ablation Studies}
\vspace{-0.5em}

\label{sec:ablation}
We conduct ablation studies on CIFAR100 to analyze functions of permutation and reflection matrices (Fig.\ref{fig:combo1}{\bf b}. 
We evaluate ResNet-RPG34 with 2M backbone DoF. Permutation and sign reflection together achieves 76.5\% accuracy, while permutation only achieves 75.8\%, and sign reflection only achieves 71.1\%. Training with neither permutation nor reflection matrices achieves 70.7\%. This suggests permutation and sign reflection matrices increase RPG performance.


==> 2107 (1)/sections/5summary.tex <==
%\vspace{-1em}

\section{Discussion}
\vspace{-0.5em}

 The common practice in neural network compression is to prune weights from a trained large model with many parameters or degrees of freedom (DoF).
 Our key insight is that a direct and drastically different approach might work faster and better: We start from a lean model with a small DoF, which can be linearly unpacked into a large model with many parameters. Then we can let the gradient descent automatically find the best model under the linear constraints. Our work is a departure from mainstream approaches towards model optimization and parameter reduction. We show how the model DoF and actual parameter size can be decoupled: we can define an arbitrary network of an arbitrary DoF.
 
We limit our scope to optimization with random linear constraints, termed destructive weight sharing.
However, in general, there might also exist nonlinear RPGs and efficient nonlinear generation functions to create convolutional kernels from a shared model ring $\mathbf{W}$. 
Further, although RPG focuses on reducing model DoF, it can be quantized and pruned to further reduce the FLOPs and runtime.

To sum up, we develop an efficient approach to build an arbitrarily complex neural network with any amount of DoF via a recurrent parameter generator.
On a wide range of applications, including classification, pose estimation and multitask regression, we show RPG consistently achieves higher performance at the same model DoF. Further, we show  such networks converge faster, are less likely to overfit and have higher performance on out-of-distribution data.

RPG can be added to any existing network flexibly with any amount of DoF at the user's discretion. It provides new perspectives for recurrent models, equilibrium models, and model compression. It also serves as a tool for understanding relationships between network properties and network DoF by factoring out the network architecture.

==> Recurrent layers/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Recurrent layers/sections/0abstract.tex <==
\begin{abstract}
Deep learning has achieved tremendous success 
by training increasingly large models, which are then compressed for practical deployment.  We propose a drastically different approach to compact and optimal deep learning:   
 We decouple the Degrees of freedom (DoF) and the actual number of parameters of a model, optimize a small DoF with predefined random linear constraints for a large model of an arbitrary architecture, in one-stage end-to-end learning.
 
Specifically, we create a recurrent parameter generator (RPG), which repeatedly fetches parameters from a ring  and unpacks them onto a large model with random permutation and sign flipping to promote parameter decorrelation.  We show that gradient descent can automatically find the best model under constraints with in fact faster convergence.

Our extensive experimentation reveals a log-linear relationship between model DoF and accuracy.  Our
 RPG demonstrates remarkable DoF reduction, 
and can be further pruned and quantized for additional  run-time performance gain.
For example, in terms of top-1 accuracy on ImageNet,
RPG achieves 96\% of ResNet18's performance with only 18\% DoF (the equivalent of one convolutional layer) and 52\% of ResNet34's performance with only 0.25\% DoF!
Our work shows significant potential of constrained neural optimization in compact and optimal deep learning.
\end{abstract}

==> Recurrent layers/sections/1intro.tex <==
%\textcolor{red}{To add: RPG is similar to weight clustering. Model file can be diminished - thus, there is smaller storage space and faster transfer rate.}

\def\figModelRing#1{
\begin{figure}[#1]\centering
\vspace{-1.5em}
\includegraphics[width=0.92\columnwidth]{figures/modelRing.pdf}
\caption{ \small We propose a recurrent parameter generator (RPG) that shares a fixed set of parameters in a ring and use them to generate parameters of different parts of a neural network, %simply by permutations and sign flipping, 
whereas in the standard neural network, all the parameters are independent of each other, so the model gets bigger as it gets deeper. \textbf{Left}: The \textcolor{orange}{third} section of the model starts to overlap with the \textcolor{red}{first} section in the model ring, and all later layers 
 share generating parameters for possibly multiple times.
 \textbf{Right:} Employing the Recurrent Parameter Generator (RPG) for ResNet could reduce the model parameters to any size. Specifically, with only half ResNet34 backbone parameters, we achieve the same ImageNet top-1 accuracy. 
 We also outperform model compression methods such as Knapsack \cite{aflalo2020knapsack}.% and PruneNet \cite{khetan2020prunenet}.
}
\vspace{-1.5em}
\label{fig:modelRing}
\end{figure}
}

\def\figtasks#1{
\vspace{-1.5em}
\begin{figure*}[#1]\centering
\includegraphics[width=0.9\textwidth]{figures/tasks_v2.pdf}
\vspace{-1em}
\caption{ \small  We demonstrate the effectiveness of RPG on various applications including image classification (\textbf{Left}), human pose estimation (\textbf{Middle}), and multitask regression (\textbf{Right}). RPGs are shared at multiple scales: a network can either have a global RPG or multiple local RPGs that are shared within blocks or sub-networks.
}
\vspace{-1.5em}
\label{fig:tasks}
\end{figure*}
}

\section{Introduction}

\begin{figure}[t]
    \centering
 \includegraphics[width=\columnwidth]{figures/teaser.pdf}
   \caption{ \small 
   We propose a novel approach to compact and optimal deep learning by decoupling model DoF and model parameters.
   {\bf a}) Existing methods first finds the optimal in a large model space and then compress it for practical deployment.  
   {\bf b})  We propose to start with a small (DoF) model of free parameters, use 
   recurrent parameter generator (RPG) to unpack them onto a large model with predefined random linear projections. 
   {\bf c}) Gradient descent finds the optimal model of a small DoF under these linear constraints with faster converge than training the large unpacked model itself (Fig.\ref{fig:combo2}{\bf b}). 
   If the DoF is too small, the optimal large model may fall out of the constrained subpsace.  However, at a sufficiently large DoF,  RPG gets rid of redundancy and often finds a model with little loss in accuracy. 
   %Large models are known to have high redundancy and low degree of freedom (DoF), for which they could be pruned to small models, e.g. high filter similarity of different layers in VGG16 is observed ({\bf c}).
    {\bf d}) RPG reveals a log-linear relationship between model DoF and accuracy.
   {\bf e}) RPG achieves the same ImageNet accuracy with half of the ResNet-vanilla DoF. RPG also outperforms other state-of-the-art compression approaches.
   }  %\captionof{figure}{A figure}
  \label{fig:teaser}
  \vspace{-1.5em}
\end{figure}

%TODO: (on reduce redundancy) Cite OCNN, lean block;
% Mention we do not compress FLOPs

% points: 1) decouple; 2) DoF; 3) practical use (reduce flops)

Deep neural networks as general optimization tools have achieved great success with increasingly more training data, deeper and larger neural networks:  A recently developed NLP model, GPT-3 \cite{brown2020language}, has astonishing 175 billion parameters!  
While the model performance generally scales with the number of parameters \cite{henighan2020scaling}, with parameters outnumbering training data, the model is significantly over-parameterized. 

%(Fig.\ref{fig:combo1}{\bf a}), 
Many approaches have been proposed to remove redundancy in trained large models: neural network pruning \cite{lecun1990optimal, han2015deep, liu2018rethinking}, efficient network design spaces \cite{howard2017mobilenets, iandola2016squeezenet, sandler2018mobilenetv2}, parameter regularization \cite{wan2013regularization, wang2020orthogonal, srivastava2014dropout, NowlanH92simplifying}, model quantization \cite{hubara2017quantized, rastegari2016xnor, louizos2018relaxed}, neural architecture search \cite{zoph2016neural, cai2018proxylessnas, wan2020fbnetv2}, recurrent models \cite{bai2019deep, bai2020multiscale, wei2016convolutional}, multi-task feature encoding \cite{ramamonjisoa2019sharpnet, hao2020multi}, etc. 
Pruning-based model compression dates back to the late 80s \cite{mozer1989using, lecun1990optimal} and has enjoyed recent resurgence \cite{han2015deep, blalock2020state}. They remove unimportant parameters from a pre-trained model and can achieve significant model compression.


 %\figModelRing{tp}
 \begin{figure}[t]
    \centering
 \includegraphics[width=\columnwidth]{figures/genweight.pdf}
   \vspace{-1em}
   \caption{ \small
   {\bf Upper:} Networks are optimized with a linear constraint $\hat{\mathbf{W}} = \boldsymbol{G} \mathbf{W}$, where the constrained parameter $\hat{\mathbf{W}}$ of each network layer was generated by the generating matrix $\boldsymbol{G}$ from the free parameter $\mathbf{W}$, which is directly optimized. $\hat{\mathbf{W}}$ is unpacked large model parameter while the size of $\mathbf{W}$ is the model DoF.
   {\bf Lower:} This paper discusses a specific format of parameter generation, 
  recurrent parameter generator (RPG).
   RPG shares a fixed set of parameters in a ring and uses them to generate parameters of different parts of a neural network,
whereas in the standard neural network, all the parameters are independent of each other, so the model gets bigger as it gets deeper. The \textcolor{orange}{third} section of the model starts to overlap with the \textcolor{red}{first} section in the model ring, and all later layers 
 share generating parameters for possibly multiple times.
   }  %\captionof{figure}{A figure}
  \label{fig:modelring_}
  \vspace{-1.5em}
\end{figure}

%Though sharing a similar motivation to reduce the parameter redundancy, 
Our work is a departure from mainstream approaches towards model optimization and parameter reduction: rather than compressing a large model, we directly optimize a lean model with a small set of free parameters (number of free parameters equal to degree of freedom of the model, or DoF), which can be linearly unpacked to a large model. Training the large model can be viewed as solving a neural optimization with a set of predefined linear constraints. One benefit of constrained neural optimization we observe is that it leads to a faster convergence rate (Section \ref{sec:general}).
% The optimization parameters of the large model are linearly constrained by the small DoF.
%We explore an entirely different territory of model DoF reduction: rather than compressing a large model, we define an arbitrarily large model based on a fixed set of parameters to maximize the model capacity. 
Specifically, we define different layers in a neural network based on a fixed amount of DoF, which we call \textit{recurrent parameter generator} (RPG).
That is, we differentiate the number of model parameters and DoF.
Traditionally, model parameters are treated independently of each other; the total number of parameters equals DoF. However, by tapping into how a core set of free parameters can be assigned to the neural network model, we can develop a large model of many parameters, which are linearly constrained by the small set of free parameters.
%We show that the excess parameter capacity can be exploited with almost no assumptions of how the parameters are assigned to the neural network architecture.

There is excess capacity in neural networks independent of how and where the parameters are used in the network, even at the level of individual scalar values.
% , parameters can be reused in another arbitrary location of the deep network architecture without significantly impacting model performance.
Surprisingly, backpropagation training of a deep network is able to cope with that the same parameter can be assigned to multiple random locations in the network without significantly impacting model performance. Our extensive experiments show that a large neural network does not need to be over-parameterized to achieve competitive performance. Particularly, a ResNet18 can be implemented with DoF equivalent to one convolution layer in a ResNet18-vanilla ($4.72\times$ DoF reduction) and still achieves $67.2\%$ ImageNet top-1 accuracy. The proposed method is also extremely flexible in reducing model DoF. In some sense, the proposed RPG method can be viewed as an automatic model DoF reduction technique, which explores the optimal accuracy-parameter trade-off. When we reduce the model DoF, RPG demonstrates graceful performance degradation, and its compression results are frequently on par with the SOTA pruning methods besides the flexibility. Even if we reduce the Res18 backbone DoF to $36$K, which is about $300\times$ reduction, ResNet18 can still achieve $40\%$ ImageNet top-1 accuracy. Further, we show RPG can be quantized and pruned to improve FLOPs and runtime with relatively
mild accuracy drops. 

To summarize, we make three contributions:
%\vspace{-0.5em}
\begin{enumerate*}
%\setlength{\itemsep}{-0em}
    \item We provide a new perspective towards automatic model size reduction: we define a neural network with certain DoF with random linear constraints. We discover that gradient descent can automatically solve constrained optimization for the best model with a faster convergence rate. This constrained neural optimization perspective is likely to benefit many other applications. % under the desired constraint.
    
    \item We propose the recurrent parameter generator (RPG), which decouples the network architecture and the network DoF. We can flexibly choose any desired DoF to construct the network given a specific neural network architecture. 

    \item By separating network architectures from parameters, RPG becomes a tool to understand the relationship between the model DoF and the network performance.  We observe an empirical log-linear DoF-Accuracy relationship.
    %\textcolor{red}{By factoring out network architecture, RPG could be considered as a tool to understand relationships between parameter size and network performance. We show a log-linear relationship between them.} %Given a compression ratio, RPG achieves on-par performance compared to the state-of-the-art model pruning methods. This may provide an entirely new perspective for model compression.
    
    %\item With destructive weight sharing, RPG achieves competitive performance compared to several recurrent weight-sharing models. This makes RPG a strong baseline for probing the representation sharing for recurrent models.
\end{enumerate*}
\figtasks{t}

% This makes RPG a strong and practical baseline for probing whether there is nontrivial representation sharing within any recurrent network.

%\textcolor{red}{This needs to be moved to later part of the paper.} Notably, we choose a destructive parameter sharing method \cite{CheungPSP19} for RPG in this work, which discourages potential representation sharing from layer to layer. Compared to other weight-sharing methods, e.g., convolutional pose machine (CPM) and multi-scale deep equilibrium models (MDEQ), our method achieves competitive  performance on various benchmarks. 


% A more relevant result was shown in model superposition \cite{cheung2019superposition} that many different models based on the same neural network can be stored into one set of parameters with minimal performance interference to each other. Inspired by the result, we generalize the concept and propose to define many different layer in a deep neural network based on a fixed amount of parameters. we show that the excess capacity can be exploited with almost no assumptions of how the parameters are assigned into architecture of the neural network. In other words, there is excess capacity in neural network models independent of how and where the parameters are used in the network. Even at the level of individual scalar values, parameters can be reused in another arbitrary location of the deep network architecture without significantly impacting model performance. Surprisingly, back propagation training of a deep network is able to cope with that the same parameter can be assigned to multiple random locations in the network without significantly impacting model performance. Through thorough experiments, we show that a large neural network does not need to be over overparameterized to achieve competitive performance. Particularly, a Resnet18 model can be implemented with the number of weights equivalent to one convolution layer in a conventional Resnet ($4.72\times$ parameter reduction) and still achieve $67.2\%$ ImageNet top-1 accuracy. The propose method is also extremely flexible in reducing the model parameters. Even if we reduce the backbone parameters to $36K$, which is about $300\times$ reduction, Resnet18 can still achieve $40.0\%$ ImageNet top-1 accuracy.

% Notably, a destructive parameter sharing method is used in this work, which discourages any potential representation sharing from layer to layer. Compared to other recurrent weight-sharing methods, e.g. convolutional pose machine (CPM) or multi-scale deep equilibrium models (MDEQ), our method achieves competitive or even better performance on a variety benchmarks. This makes our work a strong baseline for probing whether there is nontrivial representation sharing within any recurrent network.




% The number of parameters in deep networks often outnumber the datapoints they are trained on indicating that these models are significantly overparameterized. 
% This has led to many types of network compression algorithms and pruning methods to reduce the redundancies after training. But what is the source of this excess capacity?


%\textcolor{red}{ Call it ``parameter generator ring'', dub as parameter ring.}
% Contributions:
% \begin{itemize}
% \item Generic method to construct an arbitrarily convolutional neural network with a fixed set of parameters. Show competitive performance.
% \item Strong baseline for probing if there is any representation sharing in recurrent models.
% \end{itemize}


  


==> Recurrent layers/sections/2relatedworks.tex <==
\vspace{-0.5em}
\section{Related Work}
\vspace{-0.5em}
%There are many important efforts to compress  neural networks or to reduce the redundancy in neural network parameters.
Many works study model DoF reduction or compression.
We discuss each one and its relationship to our work.

\noindent \textbf{Model Pruning, Neural Architecture Search, and Quantization.}
%As we discussed earlier, 
Model pruning seeks to remove unimportant parameters in a trained model. Recently, it's proposed to use neural architecture search as coarse-grained model pruning \cite{yu2018slimmable, dong2019network}. Another related effort is  network quantization \cite{hubara2017quantized, rastegari2016xnor, louizos2018relaxed}, which seeks to reduce the bits used for each parameter and can frequently reduce the model size by $4\times$ with minimal accuracy drop. More recently, \cite{dollar2021fast} presents a framework for analyzing model scaling strategies that consider network properties such as FLOPs and activations.

\noindent \textbf{Parameter Regularization and Priors}. 
%Another highly related direction is parameter regularization.  %Another highly related direction to this work is parameter regularization. 
Regularization has been widely used to reduce model redundancy \cite{krogh1992simple, NowlanH92simplifying}, alleviate overfitting \cite{srivastava2014dropout, wan2013regularization}, and ensure desired mathematical regularity \cite{wang2020orthogonal}. RPG can be viewed as a parameter regularization in the sense that weight sharing poses many equality constraints to  weights and regularizes  weights to a low-dimensional space. HyperNeat \cite{stanley2009hypercube} and CPPNs \cite{stanley2007compositional} use networks to determine the weight between two neurons as a function of their positions. \cite{karaletsos2018probabilistic, KaraletsosB20} introduced a similar idea by providing a hierarchical prior for network parameters.

% Given a network design, another way to improve performance and model capacity is via a regularizer on model parameters. Regularizers include weight decay \cite{krogh1992simple}, dropout\cite{srivastava2014dropout}, and orthogonal regularizer \cite{wang2020orthogonal}.
% %Weight decay. OCNN \cite{wang2020orthogonal}, dropout\cite{srivastava2014dropout}, DropConnect\cite{wan2013regularization}
% %Researchers \cite{wang2020orthogonal} demonstrate adding additional regularizer improves model capacity.

% \textbf{Recurrent Models.}
%add Convolutional Sparse Coding.

%ResNext use group convolution as efficient processing. A related work?


\noindent \textbf{Recurrent Networks and Deep Equilibrium Models.} Recurrence and feedback have been shown in psychology and neuroscience to act as modulators or competitive inhibitors to aid feature grouping \cite{gilbert2007brain}, figure-ground segregation \cite{hupe1998cortical} and object recognition \cite{wyatte2012limits}. Recurrence-inspired mechanisms also achieve success in feed-forward models. There are two main types of employing recurrence based on if weights are shared across recurrent modules. ResNet \cite{he2016deep}, a representative of reusing similar structures without weight sharing, introduces parallel residual connections and achieves better performance by going deeper in networks. Similarly, some works \cite{szegedy2015going,srivastava2015highway} also suggest iteratively injecting thus-far representations to the feed-forward network useful. Stacked inference methods \cite{ramakrishna2014pose,wolpert1992stacked,weiss2010structured} are also related while they consider each output in isolation. Some find sharing weights across recurrent modules valuable. They demonstrate applications in temporal modelling \cite{weiss2010structured,shi2015convolutional,karpathy2015deep}, spatial attention \cite{mnih2014recurrent,butko2009optimal}, pose estimation \cite{wei2016convolutional,carreira2016human}, and so on \cite{li2016iterative,zamir2017feedback}. Such methods usually shine in modeling long-term dependencies. In this work, we recurrently share weights across different layers of a feedback network to reduce network redundancy. 

% \textbf{Deep Equilibrium Models.}
%DEQ, MDEQ. Application in detection.
%Improve efficiency: Fixed Point Networks:
%Implicit Depth Models with Jacobian-Free Backprop
Given stacking weight-shared modules improve the performance, researchers consider running even infinite depth of such modules by making the sequential modules converge to a fixed point \cite{lecun1988theoretical,bai2019deep}. Employing such \textit{equilibrium} models to existing networks, they show improved performance in many natural language processing \cite{bai2019deep} and computer vision tasks \cite{bai2020multiscale,wang2020implicit}. One issue with deep equilibrium models is that the forward and backward propagation usually takes much more iterations than explicit feed-forward networks. Some work \cite{fung2021fixed} improves the efficiency by making the backward propagation Jacobian free. Another issue is that \textit{infinite} depth and fixed point may not be necessary or even too strict for some tasks. 
Instead of achieving infinite depth, our model shares parameters to a certain level. We empirically compare with equilibrium models in Section \ref{sec:exp}.


\noindent \textbf{Efficient Network Space and Matrix Factorization.}
Convolution is an efficient and structured matrix-vector multiplication. Arguably, the most fundamental idea in building efficient linear systems is matrix factorization. Given the redundancy in deep convolutional neural network parameters, one can leverage the matrix factorization concept, e.g., factorized convolutions, and design more efficient network classes \cite{howard2017mobilenets, iandola2016squeezenet, tan2019efficientnet, sandler2018mobilenetv2}.


% \textbf{Deep Network Redundancy.}
% %+ Review once-for-all (arxiv 1908.09791)
% Deep neural networks are over-parameterized and have significant redundancy \cite{jaderberg2014speeding}. Towards reduce network redundancy and efficient deep learning, different works propose solutions including model compression \cite{han2015deep,han2015learning},  efficient network structures \cite{iandola2016squeezenet,sandler2018mobilenetv2}, training techniques \cite{wang2020orthogonal}, and hardware-aware neural architecture search \cite{wu2019fbnet,tan2019mnasnet}. These works demonstrate reduced network redundancy and improved efficiency for a specific tasks. Recent works \cite{cai2019once,cheung2019superposition} further show that parameters of a base model can be shared and used for multiple tasks, which further improves the model efficiency. We explore sharing parameters across different layers of a model.

==> Recurrent layers/sections/3methods.tex <==
%\vspace{-0.5em}
\section{Recurrent Parameter Generator}
%\vspace{-0.5em}

\label{sec:method:ls}

%\textcolor{red}{To add: linear constraint theory}
%\textcolor{red}{matrix from the general orthogonal group also leads to similar results but this implementation has better efficiency.}

\noindent {\bf Linearly Constrained Neural Optimization.} 
% Parameter generator can be considered  as optimizing neural networks with linear constraints.
Consider optimizing a network with input data $\mathbf{X}$, parameters $\hat{\mathbf{W}}$ and loss function $L$. The optimization can be written as: 
\begin{align}
    \min L(\mathbf{X}; \hat{\mathbf{W}} )\ \ \text{s.t.}\  \mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W} (\text{or equally} \ \boldsymbol{R}\mathbf{\hat{\mathbf{W}}} = 0)
\end{align}
where $\mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W}$ refers to a set of linear constraints, where $\boldsymbol{G}\in \Re^{N\times M}$ is a full-rank tall matrix (i.e. $N\ge M$). Here we refer to $\hat{\mathbf{W}}$ as the constrained parameters and $\mathbf{W}$ as the free parameters. This constraint is a change of variable, i.e., the constrained parameter $\hat{\mathbf{W}}$ is linearly generated from the free parameter $\mathbf{W}$ by generating matrix $\boldsymbol{G}$. We can consider $\mathbf{W}$ as a compressed model, which is unpacked into $\hat{\mathbf{W}}$ to construct the large neural network. $\mathbf{W}$ is directly optimized via gradient descent and free to update. In this linearly constrained neural optimization, the model DoF is equivalent to $M$, which is the dimension of $\mathbf{W}$. An equivalent form of the constraint $\mathbf{\hat{\mathbf{W}}} = \boldsymbol{G} \mathbf{W}$ is $\boldsymbol{R}\mathbf{\hat{\mathbf{W}}} = 0$, where $\boldsymbol{R}\in\Re^{(N-M)\times N}$ can be derived from SVD of $\boldsymbol{G}$. 

% We also discuss the even sampling and batch normalization technique that are beneficial for training with RPG.


\noindent {\bf Recurrent Parameter Generator.} Let's assume that we construct a deep convolutional neural network containing $L$ different convolution layers. Let $\mathbf{K}_1,\mathbf{K}_2,\dots, \mathbf{K}_L$ be the corresponding $L$ convolutional kernels\footnote{A kernel contains all the filters of one layer. In this paper, we treat each convolutional kernel as a vector. When the kernel is used to do the convolution, it will be reshaped into the corresponding shape.}. 
Rather than using separate sets of parameters for different convolution layers, we create a single set of parameters $\mathbf{W}\in\Re^M$ and use it to generate the corresponding parameters $\hat{\mathbf{W}} = \left[\mathbf{K}_1^T,\mathbf{K}_2^T,\dots, \mathbf{K}_L^T\right]^T \in \Re^N$ for each convolution layer:
%Rather than using a different set of parameters for each different layer, we reuse a single set of parameters $W\in\Re^N$ in the following fashion:
\begin{equation}
\mathbf{K}_i = \boldsymbol{G}_i\cdot \mathbf{W}, i \in \{1,\dots,L\}
\label{eq:k}
\end{equation}
where $\boldsymbol{G}_i$ is a fixed predefined generating matrix, which is used to generate $\mathbf{K}_i$ from $\mathbf{W}$.
We call $\boldsymbol{G} = \left[\boldsymbol{G}_1^T,\dots,\boldsymbol{G}_L^T\right]^T$ and $\mathbf{W}$ the \textit{recurrent parameter generator} (RPG). In this work, we always assume that the size of $\mathbf{W}$ is not larger than the total parameters of the model, i.e., $|\mathbf{W}|\leq\sum_{i}{|\mathbf{K}_i|}$. This means an element of $\mathbf{W}$ will generally be used in more than one layer of a neural network. Additionally, the gradient of $\mathbf{W}$ is a linear superposition of the gradients from each convolution layer.
During the neural network training, let's assume convolution kernel $\mathbf{K}_i$ receives gradient $\frac{\partial \ell}{\partial \mathbf{K}_i}$, where $\ell$ is the loss function. Based on the chain rule, it is clear that the gradient of $\mathbf{W}$ is:
\begin{equation}
\frac{\partial \ell}{\partial \mathbf{W}} = \sum_{i=1}^{L}{\boldsymbol{G}^T_i\cdot \frac{\partial \ell}{\partial \mathbf{K}_i}}
\label{eq:grad_w}
\end{equation}
% {\bf Recurrent Parameter Generator.} We focus on a special case where $W$ is reused when generating convolutional kernels. In this case, the size of $W$ is smaller than the total parameters of the model, and elements of $W$ are recurrently used. $\{R_i\}$ and $W$ together is considered as a \textit{recurrent parameter generator}. Additionally, the gradient of $W$ is a linear superposition of the gradients from each convolution layer.
%{\bf Model Rings.} As we can see, the gradient of $W$ is a linear superposition of the gradients from each convolution layer. We call $W$ as the \emph{model ring} since it can be effectively seen as a superposition of many different convolutional kernels.
\noindent {\bf Generating Matrices and Destructive Weight Sharing.} There are various ways to create the generating matrices $\{\boldsymbol{G}_i\}$. While in general $\boldsymbol{G}$ can be any full-rank tall matrix, this paper focuses on the destructive generating matrices, which are random orthogonal matrices and could prevent different kernels from sharing the representation during weight sharing. Random generating matrices empirically improve the model capacity when the model DoF is fixed. We provide an intuitive theoretical explanation of how random orthogonal matrices prevent representation sharing as follows.

% Let's assume $\{\boldsymbol{G}_i\}$ are random orthogonal matrices and $\boldsymbol{G}_i = \left[A_1,\dots,A_\right]$

For easier discussion, let us consider a special case, where all of the convolutional kernels have the same size and are used in the same shape in the corresponding convolution layers. The dimension of $\mathbf{W}$ is equal to that of one convolutional layer kernel. In other words, $\{\boldsymbol{G}_i\}$ are square matrices, and the spatial sizes of all of the convolutional kernels have the same size, $d_{in}\times d_{out}\times w\times h$, and the input channel dimension $d_{in}$ is always equal to the output channel dimension $d_{out}$. In this case, a filter $\mathbf{f}$ in a kernel can be treated as a vector in $\Re^{dwh}$. Further, we choose $\boldsymbol{G}_i$ to be a block-diagonal matrix $\boldsymbol{G}_i=\text{diag}\{\boldsymbol{A}_i,\boldsymbol{A}_i,\dots,\boldsymbol{A}_i\}$, where $\boldsymbol{A}_i\in O(dwh)$ is an orthogonal matrix that generates each filter of the kernel $\mathbf{K}_i$ from $\mathbf{W}$, and $O(\cdot)$ denotes the orthogonal group. Similar to the Proposition~2 in \cite{CheungPSP19}, we show in the Appendix \ref{sec:supp2} that: if $\boldsymbol{A}_i$, $\boldsymbol{A}_j$ are sampled from the $O(dwh)$ Haar distribution and $\mathbf{f}_i$, $\mathbf{f}_j$ are the corresponding filters (generated by $\boldsymbol{G}_i$, $\boldsymbol{G}_j$ respectively from the same set of entries of $\mathbf{W}$) from $\mathbf{K}_i$, $\mathbf{K}_j$ respectively, then we have $\E\left[\langle \mathbf{f}_i,\mathbf{f}_j \rangle\right] = 0$ and $\E \left[\langle \frac{\mathbf{f}_i}{\|\mathbf{f}_i\|},\frac{\mathbf{f}_j}{\|\mathbf{f}_j\|}\rangle^2 \right]=\frac{1}{dwh}$. Since $dwh$ is usually large, the corresponding filters from $\mathbf{K}_i$, $\mathbf{K}_j$ are close to orthogonal and generally dissimilar. This shows that even when $\{\mathbf{K}_i\}$ are generated from the same entries of $\mathbf{W}$, they are prevented from sharing the representation.

Though $\{\boldsymbol{G}_i\}$ are not updated during training, the size of $\boldsymbol{G}_i$ can be quite large in general, which can create additional computation and storage overhead. In practice, we can use permutation and element-wise random sign reflection to construct a subset of the orthogonal group as permutations and sign reflections could be implemented with high simplicity and negligible cost. A simple demonstration of $\{\boldsymbol{G}_i\}$ is demonstrated in Fig.\ref{fig:modelring_}{\bf U}\footnote{Permutations and element-wise random sign reflection conceptually are subgroups from the orthogonal group, but we shall never use them in the matrix form for the obvious efficiency purpose.}. Since pseudo-random numbers are used, it takes only two random seeds to store a random permutation and an element-wise random sign reflection.


% In practice, we can use permutation $p\in P(M)$ and element-wise random sign reflection $b\in B(M)$ to construct a subset of the orthogonal group $O(M)$, i.e. we choose $\boldsymbol{A}_i \in \{b\circ p|\ b\in B(M), p\in P(M)\}$.\footnote{Permutations and element-wise random sign reflection conceptually are subgroups from the orthogonal group, but we shall never use them in the matrix form for the obvious efficiency purpose.} Since pseudo-random numbers are used, it takes only two random seeds to store a random permutation and an element-wise random sign reflection. 

% This paper requires that $R$ can only have three values $1, 0, -1$. In general, $R$ is a random matrix, but we show that this implementation has better efficiency.



% In this work, we generalize the usage of $\boldsymbol{G}_i$ beyond the block-diagonal generating matrices described above. $\{\mathbf{K}_i\}$ may have different sizes, which can be chosen even larger than the size of $\mathbf{W}$. When $\mathbf{K}_i\in \Re^{N_i}$ is larger than $\mathbf{W}\in\Re^{N}$, the corresponding generating matrix $\boldsymbol{G}_i$ is a tall matrix. There are many ways to efficiently create the generating matrices. We use random permutations $P(N_i)$ and element-wise random sign reflections $B(N_i)$ to create $\boldsymbol{G}_i$:
% \begin{equation}
% \label{eq:generating_matrix}
% \boldsymbol{G}_i\in \{b\circ p|\ b\in B(N_i), p\in P(N_i)\},\ i = 1,\dots,L
% \end{equation}
% $\{\boldsymbol{G}_i\}$ tend to lead to destructive weight sharing and lead to better utilization of the parameter capacity. Permutations and sign reflections could be implemented with high simplicity and negligible cost.

% The opposite of destructive generating matrices would be the identity matrix.




% Add destructive proposition.

%\textbf{Super-Parameter.}

% \textbf{Permutation and Random Rotation.}

\noindent \textbf{Even Parameter Sampling and Model Ring.}
% For better parameter capacity, we introduce an even sampling strategy. We illustrate the general parameter generator in Fig.\ref{fig:modelring_}{\bf L} and RPG in Fig.\ref{fig:modelring_}{\bf R}.
While it is easy to randomly sample elements from $\mathbf{W}$ when generating parameters for each layer, it may not be optimal as some elements in $\mathbf{W}$ may not be evenly used, and some elements in $\mathbf{W}$ used at all due to sampling fluctuation. 
A simple equalization technique can be used to guarantee all elements of $\mathbf{W}$ are evenly sampled.
Suppose the size of $\mathbf{W}$ is $M$, and the size of parameter $\mathbf{\hat{\mathbf{W}}}$  of the model to be generated is $N$, $N>M$. As we mentioned earlier, there are $L$ layers and they require $\{\|K_1\|,\dots,\|K_L\|\}$ parameters respectively. As $N>M$, we can use $W$ as a ring: we first draw the first $\|K_1\|$ parameters from $\mathbf{\hat{\mathbf{W}}}$ followed by a pre-generated random permutation $p_1$ and a  pre-generated random element-wise sign flipping $b_1$ to construct layer-1 kernel $\mathbf{K}_1$. Then we draw the next $\|K_2\|$ parameters from $\mathbf{\hat{\mathbf{W}}}$ followed by pre-generated random permutation $p_2$ and a pre-generated random element-wise sign flipping $b_2$. We continue this process and wrap around when there is not enough entries left from $\mathbf{\hat{\mathbf{W}}}$. We refer to $\mathbf{\hat{\mathbf{W}}}$ together with this sampling strategy as \textit{model rings} since the free parameters are recurrently used in a loop. We illustrate the general parameter generator in Fig.\ref{fig:modelring_}{\bf U} and RPG in Fig.\ref{fig:modelring_}{\bf L}. This For data saving efficiency, we just need to save several random seed numbers instead of saving the pre-generated permutations $\{p_1,\dots,p_L\}$ and sign flipping operations $\{b_1,\dots,b_L\}$.


% We first generate $\floor{\frac{N}{M} }$ arrays $\{x|x=1,..,M\}$ and concatenate them with $(N \mod M)$ elements randomly sampled from array $\{x|x=1,..,M\}$. We call the concatenated array index array $u \in \Re^N$.
% When initializing each layer's parameter, we sequentially get indices of chosen elements $u_i$ from $u$, and randomly shuffle $u_i$.
%In this way, each layer's parameters are randomly and evenly sampled from $\mathbf{W}$.
% We refer to $\mathbf{W}$ as \textit{model rings} since elements are recurrently used in a loop.
% For data saving efficiency, we just need to save two random seed numbers (one for sampling $(M \mod N)$ elements and one for shuffling) instead of saving the large index array $u$.

\noindent \textbf{Batch Normalization.} Model performance is relatively sensitive to the batch normalization parameters. For better performance, each convolution layer needs to have its own batch normalization parameters. In general, however, the size of batch normalization is relatively negligible. Yet when $\mathbf{W}$ is extremely small (e.g., $36$K parameters), the size of batch normalization should be considered.

\iffalse
\begin{figure}[t]
    \centering
 \includegraphics[width=1\columnwidth]{figures/MSparam.pdf}
   \vspace{-1em}
   \caption{ \small Recurrent parameter generators at multiple scales. \textbf{Upper:} A global RPG is used for generating convolution kernels for the entire ResNet18. \textbf{Lower }: Four local RPGs are each responsible for generating convolution kernels within each corresponding building block of the ResNet18.}  %\captionof{figure}{A figure}
  \label{fig:msparam}
  \vspace{-1.5em}
\end{figure}
\fi

 % \vspace{-1em}
\section{RPG at Multiple Scales}
 % \vspace{-1em}

We discuss the general idea of parameter generators where only one RPG is shared globally across all layers previously. 
We could also create several local RPGs, each of which is shared at certain scales, such as blocks and sub-networks. Such RPGs may be useful for certain applications such as recurrent modeling. %Experimental results are reported in Section \ref{sec:cifar_exp}.

\label{sec:extension}
\noindent \textbf{RPGs at Block-Level.}
Many existing network architectures reuse the same design of network blocks multiple times for higher learning capacity, as discussed in the related work. 
Instead of using one global RPG for the entire network, we could alternatively create several RPGs that are shared within certain network blocks.
We take Res18 \cite{he2016deep} as a concrete example.% (Fig.\ref{fig:msparam}). 
Res18 has four building blocks. Every block has 2 residual convolution modules. %Each block has multiple residual convolution modules and outputs feature maps at different spatial sizes. 
%Specifically, ResNet18 has $2,2,2,2$ residual modules for each building block, while ResNet34 has  $3,4,6,3$ residual modules for each building block.
%To superpose ResNet18 at block scale, 
We create four local RPGs for Res18.
Each RPG is shared within the corresponding building block, where the size of the RPG is flexible and can be determined by users. Fig.\ref{fig:tasks}{\bf M}) illustrates how RPGs can be shared at the block-level.

\noindent \textbf{RPGs at Sub-Network-Level.} 
Reusing sub-networks, or recurrent networks, has achieved success in many tasks as they iteratively refine and improve the prediction.
Parameters are often shared when reusing the sub-networks.
This may not be optimal as sub-networks at different stages iteratively improve the prediction, and shared parameters may limit the learning capacity at different stages.
However, not sharing parameters at all greatly increases the model size.
RPG can be created for each sub-network. Such design leads to a much smaller DoF, while parameters of different sub-networks are orthogonal by undergoing destructive changes.% instead of directly copy-paste.
%We superpose different sub-networks with one or more RPGs. Superposition sub-networks could have a much smaller model size, while parameters for different sub-networks undergo destructive changes instead of directly copy-paste.
%We show we can also create model rings that are used for recurrent networks. At each recurrence, the weights for recurrent networks are under destructive changes. 
We show applications of sub-network-level RPGs for pose estimation and multitask regression (Section \ref{sec:pose} and \ref{sec:multi}). Fig.\ref{fig:tasks}{\bf R}) illustrates sub-network-level RPGs.% with two different ways of network superposition.


==> Recurrent layers/sections/4results.tex <==
%\vspace{-1em}
\section{Experimental Results}

\label{sec:exp}
We evaluate the performance of RPG with various tasks illustrated in Fig.\ref{fig:tasks}. %\textcolor{red}{ We refer to model DoF as \textit{number of parameters} or \textit{parameter size} for convenience, although their differences have been discussed in Introduction.}
For classification, RPG was used for the entire network except for the last fully-connected layer. We discuss performance with regard to \textit{backbone DoF}, the actual number of parameters of the backbone. For example, Res18 has $11$M backbone parameters and $512$K fc parameters, and RPG was applied to reduce $11$M backbone DoF only.
%We conduct 3 sets of experiments to evaluate the proposed superposition method (with tasks illustrated in Fig.\ref{fig:tasks}). The first set benchmarks the performance of RPG networks on image classification datasets including CIFAR100 and ImageNet. %Specifically, 
%We compare with deep equilibrium models, a strong baseline on exploiting model capacity with limited model size. 
%The second set benchmarks the performance of RPG at block and sub-network level on human pose estimation and multi-task regression datasets. We compare with recurrent models as baselines.
%The last set provide additional analysis and ablation studies of RPG networks.
%Experiments are conducted on NVIDIA GeForce GTX 2080Ti GPUs.

%\vspace{-1em}
\subsection{CIFAR Classification}
%\vspace{-0.5em}

\label{sec:cifar_exp}
%We benchmark the performance of the proposed RPG network on CIFAR10 and CIFAR100 datasets. 

\noindent \textbf{Implementation Details}. CIFAR experiments use 128 batch size, 5e-4 weight decay,  initial learning rate of 0.1 with gamma of 0.1 at epoch 60, 120 and 160. We use Kaiming initialization \cite{he2015delving} with adaptive scaling. Shared parameters are initialized with a particular variance and scale the parameters for each layer to make it match the Kaiming initialization.

\begin{table}[b]
\vspace{-1em}
\parbox{\linewidth}{
\vspace{-0.03in}
\caption{ \small RPG compared with multiscale deep equilibrium models (MDEQ) \cite{bai2020multiscale} on CIFAR10 and CIFAR100 classification. At the same number of model DoF, RPG achieves 3\% - 6\% performance gain with 15 - 25x less inference time. Inference time is measured by milliseconds per image.}
\label{tab:cifar-deq}
\centering
%\LARGE
\vspace{-0.7em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline
%\rowcolor{LightCyan}
                          &  & \multicolumn{3}{c}{ {\bf Our RPG (same DoF)} }    \\\cline{3-5} 
  \multirow{-2}{*}{ {\bf Accuracy} (\%)}  &   \multirow{-2}{*}{\bf MDEQ}                & {\bf 2x MS blk} & {\bf 3x MS blk} & {\bf 4x MS blk} \\ \hline
{\bf CIFAR10 }   & 85.1                  & 88.5         & 90.1         & \textbf{90.9}         \\ \hline
{\bf CIFAR100}   & 59.8                  & 62.8         & 64.7         & \textbf{65.7}         \\ \hline\hline
{\bf Inference time (ms)} & 3.15                 & \textbf{0.12}         & 0.18         & 0.22         \\ \hline
\end{tabular}}
}
\vfill
\vspace{0.5em}
\parbox{\linewidth}{
\centering
%\LARGE
\caption{  \small ResNet-RPG outperforms existing DoF reduction methods \cite{han2015deep,chen2015compressing,yang2019legonet} on CIFAR100.
Additionally, a global RPG outperforms block-wise local RPGs.
%At the same number of backbone DoF on CIFAR100, using local RPGs at block-level improves accuracy. Using a global RPG further improves the accuracy. RPG also outperforms baseline methods.
}
\label{tab:cifar-block}
\vspace{-0.7em}
\resizebox{0.7\linewidth}{!}{\begin{tabular}{l|c|c}
\hline  & {\bf DoF} & {\bf Acc. (\%)} \\ \hline
{\bf R18-vanilla}             & 11M               & 77.5      \\ \hline
{\bf R34-RPG.blk} & 11M               & 78.5      \\ \hline
{\bf R34-RPG}            & 11M               & \textbf{78.9}      \\ \hline \hline
{\bf R34-random weight share}& 11M               & 74.9     \\\hline
{\bf R34-DeepCompression} \cite{han2015deep}& 11M               & 72.2    \\\hline
{\bf R34-Hash} \cite{chen2015compressing}& 11M               & 75.6     \\\hline
{\bf R34-Lego} \cite{yang2019legonet}& 11M               & 78.4     \\\hline\hline
{\bf R34-vanilla}              & 21M% 21,258,240 
& \textbf{79.1}      \\ \hline
\end{tabular}
}
}
\end{table}

\noindent \textbf{Compared to Deep Equilibrium Models}. As a representative of implicit models, deep equilibrium models \cite{bai2019deep}  reduce model DoF by finding fix points via additional optimizations. We compare the image classification accuracy on CIFAR10 and CIFAR100, as well as the inference time on CIFAR100 (Table \ref{tab:cifar-deq}). Following the settings of MDEQ \cite{bai2020multiscale}, an image was sequentially fed into the initial convolutional block, the multi-scale deep equilibrium block (dubbed as \textit{MS} block), and the classification head. 
MDEQ \cite{bai2020multiscale} achieves \textit{infinite} MS blocks by finding the fixed point of the MS block.  We reuse the MS block two to four times without increasing the model DoF. RPG achieves 3\% - 6\% gain on CIFAR10 and 3\% - 6\% gain on CIFAR100. RPG inference time is 15 - 25 times smaller than MDEQ since MDEQ needs additional time to solve equilibrium during training.

%CIFAR10: MDEQ 85.1\%; ours loop twice 88.53\%, loop 3 times 90.1\%, loop 4 times 90.87\%.

%CIFAR100: MDEQ 59.75\%; ours loop twice 62.83\%, loop 3 times 64.74\%, loop 4 times 65.74\%.

%%Time (ms/per image): MDEQ: 804.7504425048828/128; ours loop twice 14.95671272277832/128, loop 3 times 22.687673568725586/128, loop 4 times 28.149127960205078/128.
%Time (ms/per image): MDEQ: 6.29; ours loop twice 0.12, loop 3 times 0.18, loop 4 times 0.22


\begin{figure}
    \centering
   \includegraphics[width=\columnwidth]{figures/combo1.pdf}
    \caption{\small {\bf a)} Large models are known to have high redundancy and low degree of freedom (DoF). They could be pruned to small models, e.g. high filter similarity of different layers in VGG16 is observed. {\bf b)} Ablation studies of permutation and sign reflection of Res34-RPG. Having both matrices gives the highest performance.}
    \label{fig:combo1}
      \vspace{-1.5em}
\end{figure}

\iffalse
\begin{figure*}[t!]
\centering
\resizebox{0.29\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
   % \vspace{-1em}
 \includegraphics[width=0.8\columnwidth]{figures/filter_sim.pdf}
\caption{ \small Large models are known to have high redundancy and low degree of freedom (DoF). They could be pruned to small models, e.g. high filter similarity of different layers in VGG16 is observed.}
\label{fig:filter_sim}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
    \vspace{-1em}
 \includegraphics[width=\columnwidth]{figures/cifar_nparam.pdf}
\caption{ \small Log-linear DoF-accuracy relationship of CIFAR100 accuracy and model DoF on CIFAR100. 
%CIFAR100 accuracy versus the backbone DoF for ResNet-vanilla and RPG.
RPG achieves the same accuracy as vanilla ResNet with 50\% DoF.}
\label{fig:cifar-nparam}
\end{minipage}}
\hfill
\resizebox{0.35\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=0.95\columnwidth]{figures/ablation.pdf}
   \caption{  \small Ablation studies of permutation and sign reflection of Res34-RPG. Having both matrices gives the highest performance.}
   \label{fig:ablation}
     \vspace{-2em}

\end{minipage}}
\vspace{-1.2em}
\end{figure*}
\fi

\noindent \textbf{Global RPG with Varying Model DoF.} 
We create one global RPG to generate parameters for convolution layers of ResNet and refer to it as \textit{ResNet-RPG}.
We report CIFAR100 top-1 accuracy of ResNet-RPG18 and ResNet-RPG34 at different model DoF (Table \ref{tab:imagenet} and Fig.\ref{fig:cifar-nparam} in Appendix \ref{sec:cifar_supp}).
Compared to ResNet, ResNet-RPG achieves higher accuracy at the same model DoF. Specifically, we achieve 36\% CIFAR100 accuracy with only 8K backbone DoF. Further, ResNet34-RPG achieves higher accuracy than ResNet18-RPG, indicating increasing time complexity gives performance gain. We observe log-linear DoF-accuracy relationship, with details in \textit{Power Law} of the following subsection.

\noindent \textbf{Local RPGs at the Block-Level}. 
In the previous Res-RPG experiments, we use one global RPG for the entire network. %(Fig.\ref{fig:msparam}-\textbf{Upper}).%the equalization technique (mentioned in Section \ref{sec:method:ls}) so that parameters of different convolutional layers are evenly sampled from the model ring. 
We also evaluate the performance when RPGs are shared locally at a block level, as discussed in Section \ref{sec:multi}.
In Table \ref{tab:cifar-block}, compared to plain ResNet18 at the same DoF, our block-level RPG network gives 1.0\% gain. In contrast, our ResNet-RPG (parameters are evenly distributed) gives a 1.4\% gain.
Using one global RPG where parameters of each layer are evenly distributed is 0.4\% higher than multiple RPGs. %The gain comes from the equalization technique.
%We compare using one model ring shared by all layers versus parameters shared by corresponding blocks (Table \ref{tab:cifar-block}). Using a model ring shared by all layers leads to 0.4\% higher accuracy.
%CIFAR10: resnet18 baseline: 95.49\%, resnet18 extend to 34: 95.52\%, resnet34 baseline: 95.57\%

%%% CIFAR100: resnet18 baseline: 77.57\%, resnet18 extend to 34 (block reuse): 78.2\%, resnet18 extend to 34 (superparam): 78.6\% , resnet34 baseline: 79.10\%.

\noindent \textbf{Comparison to Baselines.} Table \ref{tab:cifar-block} compares RPG and other model DoF reduction methods including random weight sharing, weight sharing with the deep compression \cite{han2015deep}, hashing trick \cite{chen2015compressing} and weight sharing with Lego filters \cite{yang2019legonet}. We also compare with HyperNetworks \cite{ha2016hypernetworks} in Appendix \ref{sec:hypernet}. At the same model DoF, RPG outperforms all other baselines, demonstrating the effectiveness of the proposed method. 

\noindent \textbf{RPG for Transformers.} We apply RPG for a vision transformer ViT \cite{dosovitskiy2020image} and report results in %Table \ref{tab:vit} and
Fig.\ref{fig:combo2}{\bf a}. Specifically, the ViT-tiny model with 6 transformer layers, 4 attention heads and 64 embedding dimensions, is used as a baseline. A log-linear relationship is also identified in ViT-RPG.


\subsection{ImageNet Classification}
\vspace{-0.5em}

\noindent \textbf{Implementation Details}. All ImageNet experiments use batchsize of 256, weight decay of 3e-5, and an initial learning rate of 0.3 with gamma of 0.1 every 75 epochs and 225 epochs in total. Our schedule is different from the standard schedule as the weight-sharing mechanism requires different training dynamics. We tried a few settings and found this one to be the best for RPG.

\noindent \textbf{RPG with Varying Model DoF.} We use RPG with different DoF for ResNet and report the top-1 accuracy (Table \ref{tab:imagenet} and Fig.\ref{fig:teaser}\textbf{e})). ResNet-RPGs consistently achieve higher performance than ResNets under the same model DoF. Specifically, ResNet-RPG34 achieves the same accuracy 73.4\% as ResNet34 with only half of ResNet34 backbone DoF. ResNet-RPG18 also achieves the same accuracy as ResNet18 with only half of ResNet18 backbone DoF. Further, RPG networks have higher generalizability (Section \ref{sec:general}).

\begin{table}[t!]
\centering
\LARGE
\caption{ \small ResNet-RPG consistently achieves higher performance at the same model DoF. We report ImageNet and CIFAR100 top-1 accuracy and backbone DoF for ResNet-vanilla and ResNet-RPG. }
\vspace{-0.3em}
\label{tab:imagenet}
%\vspace{0.2in}
\setlength{\tabcolsep}{20pt}
\resizebox{\columnwidth}{!}{\begin{tabular}{l|c|c|c|c|c|c|c|c}
\hline
         {\bf Acc. (\%)}      & \multicolumn{3}{c|}{ \bf R18-RPG} &  {\bf R18-vanilla} & \multicolumn{3}{c|}{ \bf R34-RPG} & {\bf R34-vanilla} \\ \hline

{\bf ImageNet }            & 40.0             & 67.2 & 70.5   & 70.5          & 41.6       & 69.1      & \textbf{73.4}   & \textbf{73.4}   \\ \hline
{\bf CIFAR100  }        &60.2              & 75.6& 77.6    & 77.6        & 61.7       & 76.5      & \textbf{78.9}   &\textbf{79.1}   \\ \hline\hline
{\bf Model DoF }          & 45K              & 2M        & 5.5M   & 11M    & 45K         & 2M        & 11M    & 21M     \\ \hline 
\end{tabular}}
\vspace{-1.5em}

\end{table}

\noindent \textbf{Power Law.} Empirically, accuracy and model DoF follow a power law, when RPG DoF is lower than 50\% ResNet-vanilla DoF (Fig.\ref{fig:teaser}{\bf d}).
The exponents of the power laws are the same for ResNet18-RPG and ResNet34-RPG on ImageNet.
The scaling law may be useful for estimating the network accuracy without training the network.
Similarly, \cite{henighan2020scaling} also identifies a power law for accuracy and model DoF of transformers.
The proposed RPG enables {\it under-parameterized} models for large-scale datasets such as ImageNet, which may unleash more new studies and findings.

%\textbf{Compared to MDEQ}. MDEQ \cite{bai2020multiscale} achieves 75.2\% top-1 accuracy on ImageNet. We use our model ring at the same number of model parameters and lower inference time and achieves \textcolor{red}{XXX}.
%MDEQ baseline: 75.2\%. ours: 74.3\%.


\iffalse
\textbf{ResNet Experiment logs}.

\begin{itemize}
    % \item Resnet18 (modified to 34) IMAGENET: Top1 val acc: $70.94 \%$ , Top5 val acc: $90.00 \%$
    \item Resnet18 (baseline) IMAGENET: Top1 val acc: $69.80 \%$, Top5 val acc $89.18 \%$:
    \item Resnet34 (baseline) IMAGENET: Top1 val acc: $73.4 \%$, Top5 val acc: $91.4 \%$
    
    \item ResNet-rpg18 (512x512x3x3) IMAGENET: 3E-5 wd, 0.3*0.1**(ep/75.) for 250 epochs learning schedule, new initialization, final accuracy on validation set: Acc@1 67.2\% Acc@5 87.4\%
    
    \item ResNet-rpg34 (512x512x3x3) IMAGENET: ResNet-rpg34, 5E-5 wd, 0.3*0.1**(ep/75.) for 250 epochs learning schedule, final accuracy on validation set:  Acc@1 69.1\% Acc@5 88.7\%
    
    \item ResNet-rpg34 (11.16M, 512x3x3x2422) IMAGENET: Acc@1: 73.4\%, Acc@5 91.2\%
    
\end{itemize}
\fi

\vspace{-0.5em}
\subsection{Pose Estimation}
\vspace{-0.5em}

\label{sec:pose}



\begin{table}[b]
\parbox{\linewidth}{

\centering
\LARGE
\caption{ \small RPG outperforms CPM \cite{wei2016convolutional} at the same DoF. We report pose estimation performance (model DoF) on MPII human pose compared with CPM \cite{wei2016convolutional}. The metric is PCKh@0.5. }
\label{tab:pck}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c|c}
\hline
    {\bf Acc. (DoF)}  & {\bf CPM} \cite{wei2016convolutional}  & {\bf RPG}   & {\bf No shared w.} \\ \hline
{\bf 1x sub-net}  & \multicolumn{3}{c}{84.7 (3.3M)}         \\ \hline
{\bf 2x sub-nets} & 86.1 (3.3M) & 86.5 (3.3M) & 87.1 (6.7M)  \\ \hline
{\bf 4x sub-nets} & 86.5 (3.3M) & 87.3 (3.3M) & 88.0 (13.3M) \\ \hline
\end{tabular}}

}
\vfill
\vspace{0.3em}
\parbox{\linewidth}{
\centering
\LARGE
\caption{ \small RPG achieves the best accuracy without sharing batch normalize parameters and with permutation and sign reflection. We report multitask regression errors on S3DIS with sub-net architecture as  \cite{ramamonjisoa2019sharpnet}. % \cite{armeni2017joint}.
Lower is better. All methods share the same DoF. Sub-net is reused once.}
\label{tab:multitask}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c}
\hline
    {\bf RMSE} (\%) & {\bf Depth} & {\bf Normal} \\ \hline
{\bf Vanilla model} & 25.5     & 41.0      \\ \hline
{\bf RPG with shared BN}                                & 24.7     & 40.3      \\ \hline
{\bf Reuse \& new BN}                           & 24.0     & 39.4     \\ \hline
{\bf Reuse \& new BN \& perm. and reflect.} & \textbf{22.8}     & \textbf{39.1}      \\ \hline
\end{tabular}}
}
\end{table}
\noindent \textbf{Implementation Details.}
We superpose sub-networks for pose estimation with a globally shared RPG. %(Fig.\ref{fig:pose}).
Hourglass networks \cite{newell2016stacked} are used as the backbone.
An input image is first fed to an initial convolution block to obtain a feature map, which is then fed to multiple stacked pose estimation sub-networks. Each sub-network outputs a pose estimation prediction, which is penalized by the pose estimation loss. 
Convolutional pose machine (CPM) \cite{wei2016convolutional} share all sub-networks weights. 
We create one global RPG to generate parameters for each sub-network. Our model size is set to the same as CPM. We also compare with larger models where parameters of sub-networks are not shared.

We evaluate on MPII Human Pose dataset \cite{andriluka20142d}, a benchmark for articulated human pose estimation, which consists of over 28K training samples over 40K people with annotated body joints. We use the hourglass network \cite{newell2016stacked} as backbone and follow all their settings. 

\noindent \textbf{Results and Analysis.} We report the Percentage of Correct Key-points at 50\% threshold (PCK@0.5) of different methods in Table \ref{tab:pck}. 
CPM \cite{wei2016convolutional} share all parameters for different sub-networks. We use one RPG that is shared globally at the same size as CPM. For reference, we also compare with the no-sharing model as the performance ceiling.
Adding the number of recurrences leads to performance gain for all methods. 
At the same model size, RPG achieves higher PCK@0.5 compared to CPM. Increasing the number of parameters by not sharing sub-network parameters also leads to some performance gain.

%metric: PCKh@0.5\\
%- 1 model (3.3M) 84.7\\
%- 2 models: cpm (3.3M) 86.1, our super (3.3M) 86.5, different weight (6.7M) 87.1\\
%- 4 models: cpm (3.3M) 86.5, our super (3.3M) 87.3, different weight (13.3M) 88.0
\iffalse
\begin{figure}[t]\centering
  \vspace{-0.12in}
    \includegraphics[width=0.62\columnwidth]{figures/subnet_pose.pdf}
\caption{ Pose estimation  with sub-network RPG.
   An input image is fed to an initial convolutional block and $N$ stacked pose estimation networks. Each sub-network predicts the pose that are penalized by corresponding loss. Parameters of each sub-network are generated from a global RPG.}
\label{fig:pose}
\end{figure}
\fi

\begin{figure*}
    \centering
   \includegraphics[width=\textwidth]{figures/combo2.pdf}
    \caption{\small {\bf a)} A log-linear DoF-accuracy relationship exists for RPGs applied to vision transformer ViT \cite{dosovitskiy2020image}. {\bf b)} RPG converges faster than the vanilla model. We plot the CIFAR10 accuracy (smoothed by moving average) versus training iterations for Res18-vanilla and Res18-RPG. RPG converges at 1k iterations while the vanilla model converges at 1.7k. {\bf c)} RPG consistently converges faster. The reduction becomes substantial with the increasing batchsize, e.g., at batchsize 1024, RPG takes $41\%$ less iterations to converge. Denote final accuracy as $P_f$, the convergence iteration is defined when current smoothed accuracy (by moving average) is within 5\% range of $P_f$.}
    \label{fig:combo2}
\end{figure*}

\iffalse
\begin{figure*}[t!]
\centering
\resizebox{0.33\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
    \vspace{-1em}
 \includegraphics[width=0.9\columnwidth]{figures/vit_nparam.pdf}
\caption{ \small A log-linear DoF-accuracy relationship exists for RPGs applied on vision transformer ViT \cite{dosovitskiy2020image}.
%The model accuracy and DoF plot of ViT-RPGs. The accuracy-DoF relationship also follows a log-linear relationship.
}
\label{fig:vit}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=\columnwidth]{figures/converge.pdf}
   \caption{  \small RPG converges faster than the vanilla model. We plot the CIFAR10 accuracy (smoothed by moving average) versus training iterations for Res18-vanilla and Res18-RPG. RPG converges at 1k iterations while vanilla model converges at 1.7k.
   }
   \label{fig:converge1}
\end{minipage}}
\hfill
\resizebox{0.32\textwidth}{!}{\begin{minipage}{.5\textwidth}
  \centering
  \vspace{-0.2in}
    \vspace{-1em}
    \includegraphics[width=\columnwidth]{figures/batchsize.pdf}
   \caption{  \small RPG consistently converges faster than the vanilla R18. The reduction becomes substantial with the increasing batchsize, e.g. at batchsize 1024, RPG takes $41\%$ less iterations to converge. Denote final accuracy as $P_f$, the convergence iteration is defined when current smoothed accuracy (by moving average) is within 5\% range of $P_f$.}
   \label{fig:converge2}
\end{minipage}}
\vspace{-2em}
\end{figure*}
\fi
\vspace{-0.5em}
\subsection{Multi-Task Regression}
\vspace{-0.5em}

\label{sec:multi}

\iffalse
\begin{figure}
    \centering
 \includegraphics[width=\columnwidth]{figures/subnet_multi.pdf}
   \caption{\small Multi-task regression  with (sub-)network RPG. 
   An input image is fed to an initial network $G$ and $N$ stacked network $F_i$. Each network outputs depth and normal maps which are penalized by corresponding loss.
   We use multiple RPGs that are shared at corresponding building blocks of the network $F_i$.
   Note that network $G$ and $F_i$ do not share parameters as they take different inputs.}  %\captionof{figure}{A figure}
  \label{fig:multitask}
\end{figure}
\fi

\noindent \textbf{Implementation Details.} We superpose sub-networks for multi-task regression with multiple RPGs at the building-block level.
We  focus on predicting depth and normal maps from a given image. We stack multiple SharpNet \cite{ramamonjisoa2019sharpnet}, a network for monocular depth and normal estimation. 
Specifically, we create multiple RPGs at the SharpNet building-block level. That is, parameters of corresponding blocks of different sub-networks are generated from the same RPG.

We evaluate the monocular depth and normal prediction performance on a 3D indoor scene dataset \cite{armeni2017joint}, which contains over 70K images with corresponding depths and normals covering over 6,000 $\text{m}^2$ indoor area.
We follow all settings of SharpNet \cite{ramamonjisoa2019sharpnet}, a SOTA monocular depth and normal estimation method.

\noindent \textbf{Results and Analysis.} We report the mean square errors for depth and normal estimation in Table \ref{tab:multitask}. Compared to one-time inference without recurrence, our RPG network gives 3\% and 2\% gain for depth and normal estimation, respectively. Directly sharing weights but using new batch normalization layers decrease the performance by 1.2\% and 0.3\% for depth and normal. Sharing weights and normalization layers further decrease the performance by 0.7\% and 0.9\% for depth and normal.

%	Depth RMSE,	Normal RMSE\\
%shared \& mask\& change BN,	22.79\%,	39.05\%\\
%shared \& no mask nor permute\& change BN,	24.0\%,	39.4\%\\
%shared \& no mask nor permute\& no change BN,	24.7\%,	40.3\%\\
%one time baseline, 25.5\%,	41.0\%

%\textcolor{red}{Figure: visualizations of different methods}
\vspace{-0.5em}
\subsection{Pruning RPG}
\vspace{-0.5em}


\begin{table}[t]
\parbox{\linewidth}{
\vspace{-0.03in}
\caption{ \small RPG achieves higher post-pruning CIFAR10 accuracy and similar post-pruning accuracy drops as SOTA fine-grained pruning approach IMP \cite{frankle2019stabilizing}. Fine-grained pruning is used for reducing DoF.
%Comparison with fine-grained pruning for reducing model size. Compared with IMP \cite{frankle2019stabilizing} on CIFAR10, RPG achieves higher pruned accuracy and similar accuracy drops.
}
\label{tab:fprune}
\centering
\LARGE
\vspace{-0.5em}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c|c}
\hline

                           & {\bf acc before} & {\bf acc after ↓ DoF} & {\bf acc drop} & {\bf model DoF} \\ \hline
{\bf R18-IMP} \cite{frankle2019stabilizing} & 92.3       & 90.5               & 1.8      & 274k      \\ \hline
{\bf R18-RPG} & 95.0       & 93.0               & 2.0      & 274k      \\ \hline
\end{tabular}}
}
\vfill
\vspace{0.5em}
\parbox{\linewidth}{
\centering
\LARGE
\caption{ \small RPG achieves similar post-pruning ImageNet performance as SOTA coarse-grained apporach Knapsack \cite{aflalo2020knapsack} at the same FLOPs. Coarse-grained pruning is used for reducing RPG FLOPs.
%Comparison with coarse-grained pruning for reducing FLOPs and inference speed.RPG achieves similar performance as Knapsack \cite{aflalo2020knapsack} on ImageNet classification.
}
\label{tab:cprune}
\vspace{-0.5em}
\resizebox{\linewidth}{!}{\begin{tabular}{l|c|c|c} \hline
   & {\bf DoF before pruning} & {\bf Pruned acc.} & {\bf FLOPs}  \\ \hline
{\bf R18-Knapsack}   & 11.2M                    & 69.35\%     & 1.09e9 \\ \hline
{\bf Pruned R18-RPG} & 5.6M                     & 69.10\%     & 1.09e9 \\ \hline
\end{tabular}
}
}
\vspace{-1em}
\end{table}

\noindent \textbf{Fine-Grained Pruning}. 
Fine-grained pruning methods aim to reduce the model DoF by sparsifying weight matrices.
Such methods usually do not reduce the inference speed, although custom algorithms \cite{sgk_sc2020} may improve the speed.
%Fine-grained pruning methods aim at reducing the model parameters, and generally cannot reduce the inference speed in practice. 
%RPG models can be directly compared to such methods as they share the same goal of reducing the number of parameters. 
At the same model DoF, RPG outperforms state-of-the-art fine-grained pruning method IMP \cite{frankle2019stabilizing}. Accuracy drops of RPG and IMP are similar, both around 2\% (Table \ref{tab:fprune}).
It is worth noting that although IMP has no run time improvement in regular settings,
it could save inference time with customized sparse GPU kernels \cite{sgk_sc2020}.

\noindent \textbf{Coarse-Grained Pruning}. While RPG is not designed to reduce FLOPs, it can be combined with coarse-grained pruning to reduce FLOPs. We prune RPG filters with the lowest $\ell_1$ norms. Table \ref{tab:cprune} shows that the pruned RPG achieves on-par performance as state-of-the-art coarse-grained pruning method Knapsack \cite{aflalo2020knapsack} at the same FLOPs.



\vspace{-0.5em}
\subsection{Analysis} 
\vspace{-0.5em}

\label{sec:general}


\begin{table*}[t]
%\vspace{-1em}
    \caption{ \small RPG increases the model generalizability. \textbf{(a)} ResNet-RPG has lower training-validation accuracy gap on ImageNet classification. The metric is training accuracy minus validation accuracy. Lower is better. \textbf{(b)} Using RPG for pose estimation also decreases the training and validation performance GAP.  The metric is training PCK@0.5 minus validation PCK@0.5. Lower is better. \textbf{(c)} ResNet with RPG has higher performance on out-of-distribution dataset ObjectNet \cite{barbu2019objectnet}. The model is trained on ImageNet only and directly evaluated on ObjectNet. }
        \vspace{-1em}

\label{tab:general}
    \begin{subtable}{.24\linewidth}
      \centering
        \caption{IN train-val gap}
\resizebox{\textwidth}{!}{\begin{tabular}{l|c|c}
\hline
{\bf Acc gap (\%)} & {\bf vanilla} & {\bf RPG} \\ \hline
{\bf R18} & -0.7   & {\bf -2.7}        \\ \hline
{\bf R34} & 1.1    & {\bf -2.3}        \\ \hline
\end{tabular}}
    \end{subtable}%
    \hfill
    \begin{subtable}{.38\linewidth}
      \centering
        \caption{Pose train-val gap}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
{\bf Acc gap (\%)} & {\bf no shared w} & {\bf shared w}  & {\bf RPG} \\ \hline
{\bf 2x sub-nets} & 1.15       & 1.13    & {\bf 0.64}      \\ \hline
{\bf 4x sub-nets} & 1.98       & 1.70    & {\bf 1.15}      \\ \hline
\end{tabular}}
    \end{subtable} 
    \hfill
    \begin{subtable}{.3\linewidth}
      \centering
        \caption{OOD on ObjectNet}
\resizebox{\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
 & {\bf R18} & {\bf R34-RPG} & {\bf R34} \\ \hline
{\bf DoF} & 11M   & 11M        & 21M   \\ \hline
{\bf Acc.} (\%) & 13.4  & {\bf 16.5}       & 16.0  \\ \hline
\end{tabular}}
    \end{subtable}
    \vspace{-1em}
\end{table*}


\noindent \textbf{Convergence rate.} Compared with the vanilla model, RPG optimizes in a parameter subspace $\hat{\mathbf{W}} =\boldsymbol{G} \mathbf{W}$ with fewer DoF. Would such constrained optimization lead to a faster convergence rate? We analyze the convergence rate of Res18-vanilla and Res18-RPG (DoF is 5.5M, 50\% of the vanilla model) with different batchsizes. All models are trained with multi-step SGD optimizer and they all reach $>94.1\%$ final CIFAR10 accuracy. For simplicity, we analyze the first optimization stage where learning rate has not decayed.

Fig.\ref{fig:combo2}{\bf b} plots the accuracy (smoothed with moving averages) v.s. training iterations with batchsize 1024. RPG has a faster convergence rate than vanilla models. We also analyze the smoothed accuracy and identify the convergence iteration versus batchsize in Fig.\ref{fig:combo2}{\bf c}. RPG consistently converges faster than the vanilla model, and the reduction becomes substantial with the increasing batchsize. %RPG consistently has lower convergence iteration than the vanilla model, and the gap is larger beyond batchsize 256. As RPG optimizes in small model space, batchsize needs to be large enough to ensure the model updates in a correct direction every iteration for a fast convergence.


\noindent \textbf{Comparison to Model Compression Methods}. 
 We report ResNet-RPG performance with different model DoF and existing compression methods on ImageNet (Fig.\ref{fig:teaser}\textbf{e}).
  RPG networks outperform SOTA methods such as \cite{aflalo2020knapsack,dong2019network,he2019filter,he2018soft,dong2017more,khetan2020prunenet}. For example, at the same model DoF, our RPG network has 0.6\% gain over the knapsack pruning \cite{aflalo2020knapsack}, a SOTA method of ImageNet pruning. 


\noindent \textbf{Storage.} RPG models only need to save the effective parameter $\mathbf{W}$, which has the size of the model DoF, since the generation matrix $G$ is saved as a random seed at no cost. The storage space of the model file can be diminished to satisfy a smaller storage limit for inference and a faster model file transfer. Empirically on PyTorch platform, ResNet18-vanilla model file is 45MB. With no accuracy loss, ResNet18-RPG model save file size is 23MB ($ \downarrow  49\%$). With 2 percentage point accuracy loss, RPG save file size is 9.5MB  ($ \downarrow  79\%$).
%Empirically on PyTorch platform for ResNet18, RPG model file achieves 

\noindent \textbf{Generalizability}. 
%To understand generalizability of proposed RPG networks, 
We report the performance gap between training and validation set on ImageNet (Table \ref{tab:general}(a)) and MPII pose estimation (Table \ref{tab:general}(b)). CPM \cite{wei2016convolutional} serves as the baseline pose estimation method. RPG models consistently achieve lower gaps between training and validation sets, indicating the RPG model suffers less from over-fitting.

We also report the out-of-distribution performance of RPG models. ObjectNet \cite{barbu2019objectnet} contains 50k images with 113 classes overlapping with ImageNet. Existing models are reported to have a large performance drop on ObjectNet. 
We directly evaluate the performance of ImageNet-trained model on ObjectNet without any fine-tuning (Table \ref{tab:general}(c)).
With the same backbone DoF, R18-RPG achieves a 3\% gain compared to R18-vanilla.
With the same network architecture design, R34-RPG achieves 0.5\% gain compared to R34.
This indicates RPG networks have higher out-of-distribution performance even with smaller model DoF.

%\textbf{Filter Similarity}.
%\textcolor{red}{TODO}

%\textbf{Filters Visualization}.
%\textcolor{red}{TODO}

\iffalse
\textbf{Feature Similarity}. 
RPG networks are small in DoF, are they still possible to prune?
Some work \cite{wang2019cop} achieves satisfactory pruning results by calculating the correlation matrix of a feature map from the network, and prune channels with high correlations. 
Following their settings, we report feature similarity of ResNet34-RPG after residual building block 3 (Fig.\ref{fig:featuresim}). From our small ResNet34-RPG with 45k backbone DoF to plain ResNet34 with 21M backbone DoF, the feature similarity gradually increases. 
This indicates our RPG networks can still be pruned, and the FLOPs and run time can be further reduced. We provide empirical pruning results in Appendix \ref{sec:supp1}.
\fi

\noindent \textbf{Quantization.} Network quantization can reduce model size with minimal accuracy drop. It is of interest to study if RPG models, whose parameters have been shrunk, can be quantized. After 8-bit quantization, the accuracy of ResNet18-RPG (5.6M DoF) only drop 0.1 percentage point on ImageNet, indicating RPG can be quantized for further model size reduction. Details are in Appendix \ref{sec:quantize}. 

\noindent \textbf{Security}. Permutation matrices generated by the random seed can be considered as security keys to decode the model. Further, only random seeds to generate generating matrix $G$ need to be saved and transferred at negligible cost.%, which is efficient in terms of size.

%\vspace{-1em}
\subsection{Ablation Studies}
\vspace{-0.5em}

\label{sec:ablation}
We conduct ablation studies on CIFAR100 to analyze functions of permutation and reflection matrices (Fig.\ref{fig:combo1}{\bf b}. 
We evaluate ResNet-RPG34 with 2M backbone DoF. Permutation and sign reflection together achieves 76.5\% accuracy, while permutation only achieves 75.8\%, and sign reflection only achieves 71.1\%. Training with neither permutation nor reflection matrices achieves 70.7\%. This suggests permutation and sign reflection matrices increase RPG performance.

%\textbf{Functions of Permutation and Reflection Matrices.}


%CIFAR100, resnet34, 2M: no perm nor mask: 70.7 \% ;no perm: 71.1\%; no mask: 75.8\%; with perm and mask: 76.5\%.
%CIFAR100, resnet18: no perm nor mask: 77.8\% ;no perm: 77.8\%; no mask: 78.3\%; with perm and mask: 78.2\%.
%\textbf{Number Parameters vs Accuracy}

==> Recurrent layers/sections/5summary.tex <==
%\vspace{-1em}

\section{Discussion}
\vspace{-0.5em}

 The common practice in neural network compression is to prune weights from a trained large model with many parameters or degrees of freedom (DoF).
 Our key insight is that a direct and drastically different approach might work faster and better: We start from a lean model with a small DoF, which can be linearly unpacked into a large model with many parameters. Then we can let the gradient descent automatically find the best model under the linear constraints. Our work is a departure from mainstream approaches towards model optimization and parameter reduction. We show how the model DoF and actual parameter size can be decoupled: we can define an arbitrary network of an arbitrary DoF.% (number of parameters). 

%Our RPG achieves on-par performance with SOTA fine-grained pruning methods. Another interesting finding is that the model accuracy shows a log-linear dependency on DoF (Section A of the supplementary). In other words, as the DoF is reduced by a factor of 2, the accuracy drop is only linear. RPG also provides a very strong baseline for parameter sharing methods.

We limit our scope to optimization with random linear constraints, termed destructive weight sharing. %for different convolutional layers. 
However, in general, there might also exist nonlinear RPGs and efficient nonlinear generation functions to create convolutional kernels from a shared model ring $\mathbf{W}$. 
Further, although RPG focuses on reducing model DoF, it can be quantized and pruned to further reduce the FLOPs and runtime.
%Additionally, although we focus on reducing model parameters, results in Fig.\ref{fig:featuresim} indicate RPG networks are compressible, and it is possible to further reduce the FLOPs and run time.

%(filter similarity: it is possible to compress other runtime efficient networks)

To sum up, we develop an efficient approach to build an arbitrarily complex neural network with any amount of DoF via a recurrent parameter generator.
On a wide range of applications, including classification, pose estimation and multitask regression, we show RPG consistently achieves higher performance at the same model DoF. Further, we show  such networks converge faster, are less likely to overfit and have higher performance on out-of-distribution data.

RPG can be added to any existing network flexibly with any amount of DoF at the user's discretion. It provides new perspectives for recurrent models, equilibrium models, and model compression. It also serves as a tool for understanding relationships between network properties and network DoF by factoring out the network architecture.
%The superposition method is general and can be applied to any given convolutional neural network for limiting model size for lower model redundancy.
%The model size is flexible and can be tailored at the user's discretion.

%{\small  \textbf{Reproducibility:} We provide our code in the supplementary.}

==> Recurrent layers/sections/old0abstract.tex <==
\begin{abstract}
Deep neural networks have achieved tremendous success as general optimization tools. To achieve higher accuracy, one has to frequently use a larger model with more parameters or degrees of freedom (DoF). A common practice of neural network compression is to prune weights from a trained large model. In this work, we explore a drastically different way of model DoF reduction. We start from a lean model with a small DoF, which can be linearly unpacked into a large model with many parameters. This can be viewed as constrained neural optimization, where the parameters have many predefined random linear constraints. We show that gradient descent can automatically find the best model under constraints with a faster convergence rate.
% The common practice in machine learning is to search for the best model in large model space with many parameters or degrees of freedom (DoF), and then shrink the optimal model for deployment. We start from a lean model with a small DoF, which can be unpacked into a large model with many parameters. We can then let the gradient descent automatically find the best model under the DoF constraint.
%The size of deep network parameters has been growing rapidly for higher performance, yet the relationship between network degree of freedom (DoF) and performance has been rarely studied. Model architecture becomes a factor for the study as it is coupled with DoF and hard to factorize. 
%We present a generic method for recurrently using the same parameters for  different layers of a deep network that decouples model architecture and DoF. 
Specifically, we create a recurrent parameter generator (RPG), from which the parameters of each layer are linearly generated. We demonstrate how to build a one-layer-size neural network to achieve similar performance as existing CNNs on various applications. For example, ResNet18 achieves $70\%$ ImageNet accuracy, while the RPG network built for it with the number of weights equivalent to one convolutional layer (or $18\%$ of the vanilla model size) achieves $67\%$ ImageNet top-1 accuracy. 
% We achieve significant performance gain compared to existing works. 
%Though using recurrent models to build a deep convolutional neural network (CNN) is not entirely new, our method achieves significant performance gain compared to the existing works. 
% We demonstrate how to build a one-layer-size neural network to achieve similar performance as other traditional CNNs on various applications.% and datasets.
%Furthermore, we demonstrate the RPG can be applied at different scales, such as layers, blocks, or even sub-networks. 
%Additionally, 
% For example, our RPG network built for ResNet18 with the number of weights equivalent to one convolutional layer of a vanilla ResNet achieves $67.2\%$ ImageNet top-1 accuracy. 
%We use the RPG to build a ResNet18 network with the number of weights equivalent to one convolutional layer of a conventional ResNet and show this model can achieve $67.2\%$ ImageNet top-1 accuracy. 
RPG allows us to build an arbitrarily complex neural network with any amount of parameters. For example, we build a ResNet34 with model DoF reduced by more than $400$ times, which still achieves $42\%$ ImageNet top-1 accuracy.
Furthermore, RPG can be further pruned and quantized for better run-time performance in addition to reducing DoF.
We provide a new tool to study the degree of freedom of a neural network and identify a log-linear relationship between model DoF and accuracy. Arguably most importantly, the discovery, supported by extensive experimental results, shows that constrained neural optimization has a significant potential for many applications.
% We also provide a new perspective for model compression.
% Rather than shrinking parameters from a large model, RPG sets a certain parameter-size constraint and 
% uses the gradient descent algorithm to automatically find the best model under the constraint. Extensive experimental results demonstrate the power of RPG.

%\keywords{ constrained neural optimization, parameter generator, degree of freedom, convergence rate}


%   The abstract paragraph should be indented \nicefrac{1}{2}~inch (3~picas) on
%   both the left- and right-hand margins. Use 10~point type, with a vertical
%   spacing (leading) of 11~points.  The word \textbf{Abstract} must be centered,
%   bold, and in point size 12. Two line spaces precede the abstract. The abstract
%   must be limited to one paragraph.
\end{abstract}

==> Recurrent layers/sections/scratch_points.tex <==
\begin{table}[ht]
\begin{minipage}[b]{0.5\columnwidth}
\centering
\resizebox{0.55\textwidth}{!}{\begin{tabular}{>{\columncolor[gray]{0.95}}l|c|c}
\hline \rowcolor{LightCyan} & DoF  & Acc. (\%) \\ \hline
ViT-vanilla & 590k & 89.1          \\ \hline
ViT-1/2     & 295k & 89.0          \\ \hline
ViT-1/4     & 148k & 88.4          \\ \hline
ViT-1/8     & 74k  & 86.0          \\ \hline
ViT-1/16    & 37k  & 83.1          \\ \hline
ViT-1/32    & 18k  & 80.0          \\ \hline
ViT-1/64    & 9k   & 76.5          \\ \hline
\end{tabular}}
    \caption{\small ViT with RPG to achieve different model DoF and CIFAR10 classification accuracy.}
       \label{tab:vit}
    \label{table:student}
\end{minipage}\hfill
\begin{minipage}[b]{0.48\linewidth}
\centering
   \includegraphics[width=\columnwidth]{figures/vit_nparam.pdf}
\captionof{figure}{\small The model accuracy and DoF plot of ViT-RPGs. The accuracy-DoF relationship also follows a log-linear relationship. }
   \label{fig:vit}
\label{fig:image}
\end{minipage}
\end{table}

\textbf{Points to make}   
   
Limit model redundancy.
0) Inverse to model compression. 
Different direction of RNN - not sharing information
use time to exchange for performance. Squeeze out more capacity (aka reduce redundancy) Inspired by model superposition.

1) Related work: general RNN, CPM, DEQ, we propose a generic RNN mechanism

2) beat CPM, DEQ MDEQ (Done)

3) The method is generic and can be applied at multiple scales. layer (elementary and instructive - Double conv CIFAR10 - simplest model - maybe
3 layers? ), block, or even network.

4) Killer results besides CPM \& MDEQ:
MDEQ
1) tiny model on CIFAR10/100 (done)
2) large model on ImageNet

a) a single layer RESNET18 b)Extend RESNET 18 to deeper model and improve performance.

5) ablation studies

A graph: number of total parameters vs accuracy.
    a) under limited \# parameters, what is the highest accuracy? - capacity
    b) adding more layers - capacity? saturation
c) function of permutation and masking (done)

Advantages:
1) Use the full capacity of all parameters\\
2) Flexible parameters


\begin{table}
\parbox{.32\linewidth}{
\centering
\LARGE
\caption{\small Our SuperResNet models has lower gap between training and validation set and on ImageNet classification higher generalizability. The metric is training accuracy minus validation accuracy. Lower is better. }
\label{tab:gap1}
\resizebox{0.2\textwidth}{!}{\begin{tabular}{>{\columncolor[gray]{0.95}}l|c|c}
\hline
\rowcolor{LightCyan} & ResNet & Ours \\ \hline
18 conv & -0.7   & -2.7        \\ \hline
34 conv & 1.1    & -2.3        \\ \hline
\end{tabular}}
}
\hfill
\parbox{.33\linewidth}{
\centering
\caption{\small Our SuperResNet models has lower gap between training and validation set and on pose estimation higher generalizability. The metric is training accuracy minus validation accuracy. Lower is better.}
\label{tab:gap2}
\resizebox{0.33\textwidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
\rowcolor{LightCyan}  & no shared w & shared w \cite{wei2016convolutional} & ours \\ \hline
2x sub-nets & 1.15       & 1.13    & 0.64      \\ \hline
4x sub-nets & 1.98       & 1.70    & 1.15      \\ \hline
\end{tabular}}
}
\hfill
\parbox{.3\linewidth}{
\centering
\LARGE
\caption{\small Our SuperResNet models have higher performance on out-of-distribution dataset ObjectNet \cite{barbu2019objectnet}. The model is trained on ImageNet only and directly evaluated on ObjectNet.}
\label{tab:object}
\resizebox{0.3\textwidth}{!}{\begin{tabular}{>{\columncolor[gray]{0.95}}l|c|c|c}
\hline
\rowcolor{LightCyan} & R18 & R34-rpg & R34 \\ \hline
\# Params & 11M   & 11M        & 21M   \\ \hline
Acc. (\%) & 13.4  & 16.5       & 16.0  \\ \hline
\end{tabular}}
}

\end{table}



\begin{table}
\parbox{\linewidth}{
\centering
\LARGE
\caption{\small Our SuperResNet models have higher performance on out-of-distribution dataset ObjectNet \cite{barbu2019objectnet}. The model is trained on ImageNet only and directly evaluated on ObjectNet.}
\label{tab:object}
\resizebox{0.4\textwidth}{!}{\begin{tabular}{>{\columncolor[gray]{0.95}}l|c|c|c}
\hline
\rowcolor{LightCyan} & Res18 & Our SuperRes34 & Res34 \\ \hline
\# Params & 11M   & 11M        & 21M   \\ \hline
Acc. (\%) & 13.4  & 16.5       & 16.0  \\ \hline
\end{tabular}}
}

\end{table}


\iffalse
\begin{figure}
\centering
\begin{minipage}{.3\textwidth}
  \centering
 \includegraphics[width=\columnwidth]{figures/subnet_multi.pdf}
   \caption{\small \textcolor{red}{place holder figure for orthogonal} Multi-task regression  with (sub-)network superposition. 
   An input image is fed to an initial network $G$ and $N$ stacked network $F_i$. Each network outputs depth and normal maps, which are penalized by corresponding loss.
   We use multiple model rings that are shared at corresponding building blocks of network $F_i$.
   Note that network $G$ and $F_i$ do not share parameters as they take different inputs.}  %\captionof{figure}{A figure}
  \label{fig:multitask}
\end{minipage}%
\hfill
\begin{minipage}{.68\textwidth}
  \centering
    \includegraphics[width=\columnwidth]{figures/subnet_pose.pdf}
   \caption{\small Pose estimation  with (sub-)network superposition.
   An input image is fed to an initial convolutional block and $N$ stacked pose estimation networks. Each network predicts the pose that is penalized by corresponding loss. We use one model ring
   }
  \label{fig:pose}
\end{minipage}
\end{figure}
\fi


\begin{figure}
\centering
\begin{minipage}{.62\textwidth}
  \centering
  \vspace{-0.12in}
    \includegraphics[width=\columnwidth]{figures/subnet_pose.pdf}
   \caption{ Pose estimation  with sub-network superposition.
   An input image is fed to an initial convolutional block and $N$ stacked pose estimation networks. Each sub-network predicts the pose that are penalized by corresponding loss. Parameters of each sub-network are generated from a global RPG.
   }
  \label{fig:pose}
\end{minipage}
\hfill
\begin{minipage}{.36\textwidth}
  \centering
 \includegraphics[width=\columnwidth]{figures/similarity.pdf}
   \caption{ Normalized histogram of feature similarity for Res34-RPG with different model parameters. Feature similarity increases as the model size decreases, indicating our RPG networks can be further pruned with methods like \citep{wang2019cop}.}  %\captionof{figure}{A figure}
  \label{fig:featuresim}
\end{minipage}%
\end{figure}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

